Range Estimation of a Moving Target Using Ultrasound Differential Zadoff-Chu Codes

High accuracy range estimation is an essential tool required in many modern applications and technologies. However, continuous range estimation of a moving target is a challenging task, especially under Doppler effects. This paper presents a novel signal design, which we name differential Zadoff-Chu (DZC). Under Doppler effects, DZC sequences improve the performance of the maximum likelihood (ML)-based range estimation compared to its performance when using regular ZC sequences. Moreover, a reduced-complexity ranging algorithm is proposed utilizing DZC sequences and is shown to outperform the regular ZC ML-based range estimation. The proposed system is evaluated in a typical indoor environment, using low-cost ultrasound hardware. Under a low signal to noise ratio (-10 dB SNR), more than 90% of the range estimates are in less than 1.6 mm error, with a movement range from $0.2$ m to 2.2 m and a maximum velocity of 0.5 m/s. For the same movement range, the system provides range estimates with a root mean square error (RMSE) less than 0.76 mm in a high SNR scenario (10 dB), and an MSE less than 0.85 mm in a low SNR scenario (-10 dB). For a larger movement range from 1.8 m to 4.2 m with a maximum velocity of 1.91 m/s, the proposed system provides range estimates with RMSE less than 7.70 mm at 10 dB SNR.

==> IEEEfull.tex <==

IEEEfull.bib
V1.12 (2007/01/11)
Copyright (c) 2002-2007 by Michael Shell
See: http://www.michaelshell.org/
for current contact information.

BibTeX bibliography string definitions of the FULL titles of
IEEE journals and magazines and online publications.

This file is designed for bibliography styles that require 
full-length titles and is not for use in bibliographies that
abbreviate titles.

Support sites:
http://www.michaelshell.org/tex/ieeetran/
http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
and/or
http://www.ieee.org/

Special thanks to Laura Hyslop and ken Rawson of IEEE for their help
in obtaining the information needed to compile this file. Also,
Volker Kuhlmann and Moritz Borgmann kindly provided some corrections
and additions.

*************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEabrv.bib, IEEEfull.bib, IEEEexample.bib,
                   IEEEtran.bst, IEEEtranS.bst, IEEEtranSA.bst,
                   IEEEtranN.bst, IEEEtranSN.bst, IEEEtran_bst_HOWTO.pdf
*************************************************************************


USAGE:

\bibliographystyle{mybstfile}
\bibliography{IEEEfull,mybibfile}

where the IEEE titles in the .bib database entries use the strings
defined here. e.g.,


   journal = IEEE_J_AC,


to yield "{IEEE} Transactions on Automatic Control"


WARNING: IEEE uses abbreviated journal titles in their bibliographies!
Because this file provides the full titles, you should NOT use this file
for work that is to be submitted to the IEEE.

For IEEE work, you should use the abbreviated titles provided in the
companion file, IEEEabrv.bib.


** NOTES **

 1. Journals have been grouped according to subject in order to make it
    easier to locate and extract the definitions for related journals - 
    as most works use references that are confined to a single topic.
    Magazines are listed in straight alphabetical order.

 2. String names are closely based on IEEE's own internal acronyms.

 3. Older, out-of-print IEEE titles are included (but not including titles
    dating prior to IEEE's formation from the IRE and AIEE in 1963).






IEEE Journals 



aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Transactions on Aerospace and Electronic Systems"}
@STRING{IEEE_J_ANE        = "{IEEE} Transactions on Aerospace and Navigational Electronics"}
@STRING{IEEE_J_ANNE       = "{IEEE} Transactions on Aeronautical and Navigational Electronics"}
@STRING{IEEE_J_AS         = "{IEEE} Transactions on Aerospace"}
@STRING{IEEE_J_AIRE       = "{IEEE} Transactions on Airborne Electronics"}
@STRING{IEEE_J_MIL        = "{IEEE} Transactions on Military Electronics"}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Transactions on Intelligent Transportation Systems"}
@STRING{IEEE_J_VT         = "{IEEE} Transactions on Vehicular Technology"}
@STRING{IEEE_J_VC         = "{IEEE} Transactions on Vehicular Communications"}



circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Letters"}
@STRING{IEEE_J_ASSP       = "{IEEE} Transactions on Acoustics, Speech, and Signal Processing"}
@STRING{IEEE_J_AU         = "{IEEE} Transactions on Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Transactions on Audio and Electroacoustics"}
@STRING{IEEE_J_AC         = "{IEEE} Transactions on Automatic Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Transactions on Circuits and Systems"}
@STRING{IEEE_J_CASVT      = "{IEEE} Transactions on Circuits and Systems for Video Technology"}
@STRING{IEEE_J_CASI       = "{IEEE} Transactions on Circuits and Systems---Part {I}: Fundamental Theory and Applications"}
@STRING{IEEE_J_CASII      = "{IEEE} Transactions on Circuits and Systems---Part {II}: Analog and Digital Signal Processing"}
in 2004 CASI and CASII renamed part title to CASI_RP and CASII_EB, respectively.
@STRING{IEEE_J_CASI_RP    = "{IEEE} Transactions on Circuits and Systems---Part {I}: Regular Papers"}
@STRING{IEEE_J_CASII_EB   = "{IEEE} Transactions on Circuits and Systems---Part {II}: Express Briefs"}
@STRING{IEEE_J_CT         = "{IEEE} Transactions on Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Transactions on Control Systems Technology"}
@STRING{IEEE_J_SP         = "{IEEE} Transactions on Signal Processing"}
@STRING{IEEE_J_SU         = "{IEEE} Transactions on Sonics and Ultrasonics"}
@STRING{IEEE_J_SAP        = "{IEEE} Transactions on Speech and Audio Processing"}
@STRING{IEEE_J_UE         = "{IEEE} Transactions on Ultrasonics Engineering"}
@STRING{IEEE_J_UFFC       = "{IEEE} Transactions on Ultrasonics, Ferroelectrics, and Frequency Control"}



communications
@STRING{IEEE_J_COML       = "{IEEE} Communications Letters"}
@STRING{IEEE_J_JSAC       = "{IEEE} Journal on Selected Areas in Communications"}
@STRING{IEEE_J_COM        = "{IEEE} Transactions on Communications"}
@STRING{IEEE_J_COMT       = "{IEEE} Transactions on Communication Technology"}
@STRING{IEEE_J_WCOM       = "{IEEE} Transactions on Wireless Communications"}



components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Transactions on Advanced Packaging"}
@STRING{IEEE_J_CHMT       = "{IEEE} Transactions on Components, Hybrids and Manufacturing Technology"}
@STRING{IEEE_J_CPMTA      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {B}: Advanced Packaging"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {C}: Manufacturing"}
@STRING{IEEE_J_CAPT       = "{IEEE} Transactions on Components and Packaging Technology"}
@STRING{IEEE_J_CAPTS      = "{IEEE} Transactions on Components and Packaging Technologies"}
@STRING{IEEE_J_CPART      = "{IEEE} Transactions on Component Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Transactions on Electronics Packaging Manufacturing"}
@STRING{IEEE_J_MFT        = "{IEEE} Transactions on Manufacturing Technology"}
@STRING{IEEE_J_PHP        = "{IEEE} Transactions on Parts, Hybrids and Packaging"}
@STRING{IEEE_J_PMP        = "{IEEE} Transactions on Parts, Materials and Packaging"}



CAD
@STRING{IEEE_J_TCAD       = "{IEEE} Journal on Technology in Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Transactions on Computer-Aided Design of Integrated Circuits and Systems"}



coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Transactions on Information Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Transactions on Knowledge and Data Engineering"}



computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Transactions on Computers"}
@STRING{IEEE_J_CAL        = "{IEEE} Computer Architecture Letters"}
@STRING{IEEE_J_DSC        = "{IEEE} Transactions on Dependable and Secure Computing"}
@STRING{IEEE_J_ECOMP      = "{IEEE} Transactions on Electronic Computers"}
@STRING{IEEE_J_EVC        = "{IEEE} Transactions on Evolutionary Computation"}
@STRING{IEEE_J_FUZZ       = "{IEEE} Transactions on Fuzzy Systems"}
@STRING{IEEE_J_IFS        = "{IEEE} Transactions on Information Forensics and Security"}
@STRING{IEEE_J_MC         = "{IEEE} Transactions on Mobile Computing"}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Transactions on Networking"}
@STRING{IEEE_J_NN         = "{IEEE} Transactions on Neural Networks"}
@STRING{IEEE_J_PDS        = "{IEEE} Transactions on Parallel and Distributed Systems"}
@STRING{IEEE_J_SE         = "{IEEE} Transactions on Software Engineering"}



computer graphics, imaging, and multimedia
@STRING{IEEE_J_JDT        = "{IEEE/OSA} Journal of Display Technology"}
@STRING{IEEE_J_IP         = "{IEEE} Transactions on Image Processing"}
@STRING{IEEE_J_MM         = "{IEEE} Transactions on Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Transactions on Visualization and Computer Graphics"}



cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_ASE        = "{IEEE} Transactions on Automation Science and Engineering"}
@STRING{IEEE_J_JRA        = "{IEEE} Journal of Robotics and Automation"}
@STRING{IEEE_J_HFE        = "{IEEE} Transactions on Human Factors in Electronics"}
@STRING{IEEE_J_MMS        = "{IEEE} Transactions on Man-Machine Systems"}
@STRING{IEEE_J_PAMI       = "{IEEE} Transactions on Pattern Analysis and Machine Intelligence"}
in 1989 JRA became RA
in August 2004, RA split into ASE and RO
@STRING{IEEE_J_RA         = "{IEEE} Transactions on Robotics and Automation"}
@STRING{IEEE_J_RO         = "{IEEE} Transactions on Robotics"}
@STRING{IEEE_J_SMC        = "{IEEE} Transactions on Systems, Man, and Cybernetics"}
@STRING{IEEE_J_SMCA       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {A}: Systems and Humans"}
@STRING{IEEE_J_SMCB       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {B}: Cybernetics"}
@STRING{IEEE_J_SMCC       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {C}: Applications and Reviews"}
@STRING{IEEE_J_SSC        = "{IEEE} Transactions on Systems Science and Cybernetics"}



earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Transactions on Geoscience Electronics"}
@STRING{IEEE_J_GRS        = "{IEEE} Transactions on Geoscience and Remote Sensing"}
@STRING{IEEE_J_GRSL       = "{IEEE} Geoscience and Remote Sensing Letters"}
@STRING{IEEE_J_OE         = "{IEEE} Journal of Oceanic Engineering"}



education, engineering, history, IEEE, professional
@STRING{IEEE_J_CJECE      = "Canadian Journal of Electrical and Computer Engineering"}
@STRING{IEEE_J_PROC       = "Proceedings of the {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Transactions on Education"}
@STRING{IEEE_J_EM         = "{IEEE} Transactions on Engineering Management"}
@STRING{IEEE_J_EWS        = "{IEEE} Transactions on Engineering Writing and Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Transactions on Professional Communication"}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas and Wireless Propagation Letters"}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave and Guided Wave Letters"}
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave and Wireless Components Letters"}
@STRING{IEEE_J_AP         = "{IEEE} Transactions on Antennas and Propagation"}
@STRING{IEEE_J_EMC        = "{IEEE} Transactions on Electromagnetic Compatibility"}
@STRING{IEEE_J_MAG        = "{IEEE} Transactions on Magnetics"}
@STRING{IEEE_J_MTT        = "{IEEE} Transactions on Microwave Theory and Techniques"}
@STRING{IEEE_J_RFI        = "{IEEE} Transactions on Radio Frequency Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Translation Journal on Magnetics in Japan"}



energy and power
@STRING{IEEE_J_EC         = "{IEEE} Transactions on Energy Conversion"}
@STRING{IEEE_J_PEL        = "{IEEE} Power Electronics Letters"}
@STRING{IEEE_J_PWRAS      = "{IEEE} Transactions on Power Apparatus and Systems"}
@STRING{IEEE_J_PWRD       = "{IEEE} Transactions on Power Delivery"}
@STRING{IEEE_J_PWRE       = "{IEEE} Transactions on Power Electronics"}
@STRING{IEEE_J_PWRS       = "{IEEE} Transactions on Power Systems"}



industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Transactions on Applications and Industry"}
@STRING{IEEE_J_BC         = "{IEEE} Transactions on Broadcasting"}
@STRING{IEEE_J_BCTV       = "{IEEE} Transactions on Broadcast and Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Transactions on Consumer Electronics"}
@STRING{IEEE_J_IE         = "{IEEE} Transactions on Industrial Electronics"}
@STRING{IEEE_J_IECI       = "{IEEE} Transactions on Industrial Electronics and Control Instrumentation"}
@STRING{IEEE_J_IA         = "{IEEE} Transactions on Industry Applications"}
@STRING{IEEE_J_IGA        = "{IEEE} Transactions on Industry and General Applications"}
@STRING{IEEE_J_IINF       = "{IEEE} Transactions on Industrial Informatics"}
@STRING{IEEE_J_PSE        = "{IEEE} Journal of Product Safety Engineering"}



instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Transactions on Instrumentation and Measurement"}



insulation and materials
@STRING{IEEE_J_JEM        = "{IEEE/TMS} Journal of Electronic Materials"}
@STRING{IEEE_J_DEI        = "{IEEE} Transactions on Dielectrics and Electrical Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Transactions on Electrical Insulation"}



mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Transactions on Mechatronics"}
@STRING{IEEE_J_MEMS       = "{IEEE/ASME} Journal of Microelectromechanical Systems"}



medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Transactions on Biomedical Engineering"}
Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Transactions on Bio-Medical Engineering"}
@STRING{IEEE_J_BMELC      = "{IEEE} Transactions on Bio-Medical Electronics"}
@STRING{IEEE_J_CBB        = "{IEEE/ACM} Transactions on Computational Biology and Bioinformatics"}
@STRING{IEEE_J_ITBM       = "{IEEE} Transactions on Information Technology in Biomedicine"}
@STRING{IEEE_J_ME         = "{IEEE} Transactions on Medical Electronics"}
@STRING{IEEE_J_MI         = "{IEEE} Transactions on Medical Imaging"}
@STRING{IEEE_J_NB         = "{IEEE} Transactions on NanoBioscience"}
@STRING{IEEE_J_NSRE       = "{IEEE} Transactions on Neural Systems and Rehabilitation Engineering"}
@STRING{IEEE_J_RE         = "{IEEE} Transactions on Rehabilitation Engineering"}



optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photonics Technology Letters"}
@STRING{IEEE_J_JLT        = "{IEEE/OSA} Journal of Lightwave Technology"}



physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Letters"}
@STRING{IEEE_J_JQE        = "{IEEE} Journal of Quantum Electronics"}
@STRING{IEEE_J_JSTQE      = "{IEEE} Journal of Selected Topics in Quantum Electronics"}
@STRING{IEEE_J_ED         = "{IEEE} Transactions on Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Transactions on Nanotechnology"}
@STRING{IEEE_J_NS         = "{IEEE} Transactions on Nuclear Science"}
@STRING{IEEE_J_PS         = "{IEEE} Transactions on Plasma Science"}



reliability
@STRING{IEEE_J_DMR        = "{IEEE} Transactions on Device and Materials Reliability"}
@STRING{IEEE_J_R          = "{IEEE} Transactions on Reliability"}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical and Solid-State Letters"}
@STRING{IEEE_J_JSSC       = "{IEEE} Journal of Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Transactions on Applied Superconductivity"}
@STRING{IEEE_J_SM         = "{IEEE} Transactions on Semiconductor Manufacturing"}



sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors Journal"}



VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Transactions on Very Large Scale Integration ({VLSI}) Systems"}






IEEE Magazines



@STRING{IEEE_M_AES        = "{IEEE} Aerospace and Electronics Systems Magazine"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals of the History of Computing"}
@STRING{IEEE_M_AP         = "{IEEE} Antennas and Propagation Magazine"}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Magazine"}
@STRING{IEEE_M_CD         = "{IEEE} Circuits and Devices Magazine"}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits and Systems Magazine"}
@STRING{IEEE_M_COM        = "{IEEE} Communications Magazine"}
@STRING{IEEE_M_COMSOC     = "{IEEE} Communications Society Magazine"}
@STRING{IEEE_M_CIM        = "{IEEE} Computational Intelligence Magazine"}
CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Computing in Science and Engineering"}
@STRING{IEEE_M_CSEM       = "{IEEE} Computational Science and Engineering Magazine"}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Computer Applications in Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Computer Graphics and Applications"}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Systems Magazine"}
@STRING{IEEE_M_DTC        = "{IEEE} Design and Test of Computers"}
@STRING{IEEE_M_EI         = "{IEEE} Electrical Insulation Magazine"}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnology Review"}
@STRING{IEEE_M_EMB        = "{IEEE} Engineering in Medicine and Biology Magazine"}
@STRING{IEEE_M_EMR        = "{IEEE} Engineering Management Review"}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Industry Applications Magazine"}
@STRING{IEEE_M_IM         = "{IEEE} Instrumentation and Measurement Magazine"}
@STRING{IEEE_M_IS         = "{IEEE} Intelligent Systems"}
@STRING{IEEE_M_IC         = "{IEEE} Internet Computing"}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Professional"}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave Magazine"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Communications Magazine"}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power and Energy Magazine"}
@STRING{IEEE_M_PER        = "{IEEE} Power Engineering Review"}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Computing"}
@STRING{IEEE_M_RA         = "{IEEE} Robotics and Automation Magazine"}
@STRING{IEEE_M_SAP        = "{IEEE} Security and Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Magazine"}
@STRING{IEEE_M_S          = "{IEEE} Software"}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectrum"}
@STRING{IEEE_M_TS         = "{IEEE} Technology and Society Magazine"}
@STRING{IEEE_M_VT         = "{IEEE} Vehicular Technology Magazine"}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Communications Magazine"}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}






IEEE Online Publications 



@STRING{IEEE_O_CSTO        = "{IEEE} Communications Surveys and Tutorials"}
@STRING{IEEE_O_DSO         = "{IEEE} Distributed Systems Online"}





--
EOF

%%%%%%%%%%%%%%%%%% Intro Ref %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@online{Gest2015Market,
  author = "marketsandmarkets.com",
  title = "Gesture Recognition \& Touchless Sensing Market by Technology (Touch-based \& Touchless), Application (Consumer Electronics, Automotive, \& Others), Product (Biometric \& Sanitary Equipment) \& by Geography - Global Forecast to 2020",
  year = 2015,
  url = "http://www.marketsandmarkets.com/Market-Reports/touchless-sensing-gesturing-market-369.html?gclid=CM68vN790csCFfUV0wodX64INQ",
  urldate = "2016-03-19"
}

@article{rautaray2015vision,
  title="Vision based hand gesture recognition for human computer interaction: a survey",
  author="Rautaray, Siddharth S and Agrawal, Anupam",
  journal="Artificial Intelligence Review",
  volume="43",
  number="1",
  pages="1--54",
  year="2015",
  publisher="Springer"
}

@online{lynx2015studio,
  author = {http://www.lynxstudio.com/},
  title = {New Lynx E44, E22 PCI Express Cards},
  year = 2016,
  url = {http://www.lynxstudio.com/news_press_detail.asp?i=152},
  urldate = {2016-03-19}
}

@inproceedings{gupta2012soundwave,
  title="Soundwave: using the doppler effect to sense gestures",
  author="Gupta, Sidhant and Morris, Daniel and Patel, Shwetak and Tan, Desney",
  booktitle="Proceedings of the SIGCHI Conference on Human Factors in Computing Systems",
  pages="1911--1914",
  year="2012",
  organization="ACM"
}

@inproceedings{kalgaonkar2009one,
  title={One-handed gesture recognition using ultrasonic Doppler sonar},
  author={Kalgaonkar, Kaustubh and Raj, Bhiksha},
  booktitle={Acoustics, Speech and Signal Processing, 2009. ICASSP 2009. IEEE International Conference on},
  pages={1889--1892},
  year={2009},
  organization={IEEE}
}

@inproceedings{tarzia2009sonar,
  title={Sonar-based measurement of user presence and attention},
  author={Tarzia, Stephen P and Dick, Robert P and Dinda, Peter A and Memik, Gokhan},
  booktitle={Proceedings of the 11th international conference on Ubiquitous computing},
  pages={89--92},
  year={2009},
  organization={ACM}
}

@inproceedings{qifan2014dolphin,
  title={Dolphin: Ultrasonic-based gesture recognition on smartphone platform},
  author={Qifan, Yang and Hao, Tang and Xuebing, Zhao and Yin, Li and Sanfeng, Zhang},
  booktitle={Computational Science and Engineering (CSE), 2014 IEEE 17th International Conference on},
  pages={1461--1468},
  year={2014},
  organization={IEEE}
}

@article{frank1962phase,
  title={Phase shift pulse codes with good periodic correlation properties (corresp.)},
  author={Frank, R and Zadoff, S and Heimiller, R},
  journal={IRE Transactions on Information Theory},
  volume={8},
  number={6},
  pages={381--382},
  year={1962},
  publisher={IEEE}
}

@article{chu1972polyphase,
  title={Polyphase codes with good periodic correlation properties (corresp.)},
  author={Chu, David},
  journal={IEEE Transactions on Information Theory},
  volume={18},
  number={4},
  pages={531--532},
  year={1972},
  publisher={IEEE}
}

@InProceedings{C2,
  author = 	 "Jones, C.D. and Smith, A.B. and Roberts, E.F.",
  title =        "Article Title",
  booktitle =        "Proceedings Title",
  organization = "IEEE",
  year = 	 "2003",
  volume = 	 "II",
  pages = 	 "803-806"
}






@incollection{shan2010gesture,
  title= "Gesture control for consumer electronics",
  author= "Shan, Caifeng",
  booktitle= "Multimedia Interaction and Intelligent User Interfaces",
  pages= "107--128",
  year= "2010",
  publisher= "Springer"
}


@article{sharif2000computationally,
  title={A computationally efficient Doppler compensation system for underwater acoustic communications},
  author={Sharif, Bayan S and Neasham, Jeff and Hinton, Oliver R and Adams, Alan E},
  journal={IEEE Journal of oceanic engineering},
  volume={25},
  number={1},
  pages={52--61},
  year={2000},
  publisher={IEEE}
}

@inproceedings{kushwaha2005sensor,
  title={Sensor node localization using mobile acoustic beacons},
  author={Kushwaha, Manish and Moln{\'a}r, K{\'a}roly and Sallai, J{\'a}nos and Volgyesi, Peter and Mar{\'o}ti, Mikl{\'o}s and L{\'e}deczi, Akos},
  booktitle={IEEE International Conference on Mobile Adhoc and Sensor Systems Conference},
  pages={9--17},
  year={2005}
}

@inproceedings{girod2001robust,
  title={Robust range estimation using acoustic and multimodal sensing},
  author={Girod, Lewis and Estrin, Deborah},
  booktitle={Proceedings of Intelligent Robots and Systems, 2001. 2001 IEEE/RSJ International Conference on},
  volume={3},
  pages={1312--1320},
  year={2001},
  organization={IEEE}
}


@article{hightower2001survey,
  title={A survey and taxonomy of location systems for ubiquitous computing},
  author={Hightower, Jeffrey and Borriello, Gaetano},
  journal={IEEE computer},
  volume={34},
  number={8},
  pages={57--66},
  year={2001}
}

@article{whitehouse2007practical,
  title={A practical evaluation of radio signal strength for ranging-based localization},
  author={Whitehouse, Kamin and Karlof, Chris and Culler, David},
  journal={ACM SIGMOBILE Mobile Computing and Communications Review},
  volume={11},
  number={1},
  pages={41--52},
  year={2007},
  publisher={ACM}
}

@article{yuzbacsiouglu2005improved,
  title={Improved range estimation using simple infrared sensors without prior knowledge of surface characteristics},
  author={Y{\"u}zba{\c{s}}io{\u{g}}lu, {\c{C}}a{\u{g}}ri and Barshan, Billur},
  journal={Measurement Science and Technology},
  volume={16},
  number={7},
  pages={1395},
  year={2005},
  publisher={IOP Publishing}
}


@article{amann2001laser,
  title={Laser ranging: a critical review of usual techniques for distance measurement},
  author={Amann, Markus-Christian and Bosch, Thierry and Lescure, Marc and Myllyla, Risto and Rioux, Marc},
  journal={Optical engineering},
  volume={40},
  number={1},
  pages={10--19},
  year={2001},
  publisher={International Society for Optics and Photonics}
}


@article{figueroa1991ultrasonic,
  title={An ultrasonic ranging system for structural vibration measurements},
  author={Figueroa, Fernando and Barbieri, Enrique},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={40},
  number={4},
  pages={764--769},
  year={1991},
  publisher={IEEE}
}


@article{huang2009multiple,
  title={Multiple-frequency ultrasonic distance measurement using direct digital frequency synthesizers},
  author={Huang, Ke-Nung and Huang, Yu-Pei},
  journal={Sensors and Actuators A: Physical},
  volume={149},
  number={1},
  pages={42--50},
  year={2009},
  publisher={Elsevier}
}


@article{huang2002high,
  title={A high accuracy ultrasonic distance measurement system using binary frequency shift-keyed signal and phase detection},
  author={Huang, SS and Huang, CF and Huang, KN and Young, Ming-Shing},
  journal={Review of Scientific Instruments},
  volume={73},
  number={10},
  pages={3671--3677},
  year={2002},
  publisher={AIP Publishing}
}

@article{huang1999multiple,
  title={Multiple-frequency continuous wave ultrasonic system for accurate distance measurement},
  author={Huang, CF and Young, MS and Li, YC},
  journal={Review of scientific instruments},
  volume={70},
  number={2},
  pages={1452--1458},
  year={1999},
  publisher={AIP Publishing}
}

@article{hua2002low,
  title={A low-cost dynamic range-finding device based on amplitude-modulated continuous ultrasonic wave},
  author={Hua, Hong and Wang, Yongtian and Yan, Dayuan},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={51},
  number={2},
  pages={362--367},
  year={2002},
  publisher={IEEE}
}

@article{sasaki2009air,
  title={Air-coupled ultrasonic time-of-flight measurement system using amplitude-modulated and phase inverted driving signal for accurate distance measurements},
  author={Sasaki, Katsuhiro and Tsuritani, Hiroyuki and Tsukamoto, Yoshitoshi and Iwatsubo, Satoshi},
  journal={IEICE Electronics Express},
  volume={6},
  number={21},
  pages={1516--1521},
  year={2009},
  publisher={The Institute of Electronics, Information and Communication Engineers}
}

@article{hazas2002novel,
  title={A novel broadband ultrasonic location system},
  author={Hazas, Mike and Ward, Andy},
  booktitle={International Conference on Ubiquitous Computing},
  pages={264--280},
  year={2002},
  organization={Springer}
}

@article{saad2011robust,
  title={Robust high-accuracy ultrasonic range measurement system},
  author={Saad, Mohamed M and Bleakley, Chris J and Dobson, Simon},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={60},
  number={10},
  pages={3334--3341},
  year={2011},
  publisher={IEEE}
}

@online{ART,
  author = {http://www.ar-tracking.com/products/tracking-systems/systems-overview/},
  title = {ARTTRACK system overview},
  year = 2017,
  url = {http://www.ar-tracking.com/products/tracking-systems/systems-overview/},
  urldate = {2017-03-06}
}

@article{narayanan2000doppler,
  title={Doppler estimation using a coherent ultrawide-band random noise radar},
  author={Narayanan, Ram M and Dawood, Muhammad},
  journal={IEEE Transactions on Antennas and Propagation},
  volume={48},
  number={6},
  pages={868--878},
  year={2000},
  publisher={IEEE}
}

@inproceedings{cypriani2009open,
  title={Open wireless positioning system: A wi-fi-based indoor positioning system},
  author={Cypriani, Matteo and Lassabe, Fr{\'e}d{\'e}ric and Canalda, Philippe and Spies, Fran{\c{c}}ois},
  booktitle={Vehicular Technology Conference Fall (VTC 2009-Fall), IEEE 70th},
  pages={1--5},
  year={2009}
}

@article{alvarez2017cdma,
  title={CDMA-based acoustic local positioning system for portable devices with multipath cancellation},
  author={{\'A}lvarez, Fernando J and Aguilera, Teodoro and L{\'o}pez-Valcarce, Roberto},
  journal={Digital Signal Processing},
  volume={62},
  pages={38--51},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{najjar2009new,
  title={A New scheme for preamble detection and frequency acquisition in OFDM systems},
  author={Najjar, Le{\"\i}la and Siala, Mohamed},
  booktitle={Electronics, Circuits, and Systems, 2009. ICECS 2009. 16th IEEE International Conference on},
  pages={1008--1011},
  year={2009},
  organization={IEEE}
}

@book{abramowitz1965handbook,
  title={Handbook of mathematical functions: with formulas, graphs, and mathematical tables},
  author={Abramowitz, Milton and Stegun, Irene A},
  volume={55},
  year={1965},
  publisher={Courier Corporation}
}

@book{zagzebski1996essentials,
  title={Essentials of ultrasound physics},
  author={Zagzebski, James A},
  year={1996},
  publisher={Mosby}
}

@online{Pozyx,
	author = {https://www.pozyx.io/},
	title = {Pozyx System Overview},
	year = 2020,
	url = {https://www.pozyx.io/},
	urldate = {2020-12-23}
}

@online{Marvel,
	author = {https://marvelmind.com/},
	title = {Marvel Mind System Overview},
	year = 2020,
	url = {https://marvelmind.com/},
	urldate = {2020-12-23}
}

==> circuitikz/doc/changelog.tex <==
%DO NOT EDIT THIS AUTOMATICALLY GENERATED FILE, run "make changelog" at toplevel!!!
The major changes among the different circuitikz versions are listed
here. See \url{https://github.com/circuitikz/circuitikz/commits} for a
full list of changes.

\begin{itemize}
\tightlist
\item
  Version 0.8.3 (2017-05-28)

  \begin{itemize}
  \tightlist
  \item
    Removed unwanted lines at to-paths if the starting point is a node
    without a explicit anchor.
  \item
    Fixed scaling option, now all parts are scaled by bipoles/length
  \item
    Surge arrester appears no more if a to path is used without
    {[}{]}-options
  \item
    Fixed current placement now possible with paths at an angle of
    around 280°
  \item
    Fixed voltage placement now possible with paths at an angle of
    around 280°
  \item
    Fixed label and annotation placement (at some angles position not
    changable)
  \item
    Adjustable default distance for straight-voltages:
    `bipoles/voltage/straight label distance'
  \item
    Added Symbol for bandstop filter
  \item
    New annotation type to show flows using f=\ldots{} like currents,
    can be used for thermal, power or current flows
  \end{itemize}
\item
  Version 0.8.2 (2017-05-01)

  \begin{itemize}
  \tightlist
  \item
    Fixes pgfkeys error using alternatively specified mixed colors(see
    pgfplots manual section ``4.7.5 Colors'')
  \item
    Added new switches ``ncs'' and ``nos''
  \item
    Reworked arrows at spst-switches
  \item
    Fixed direction of controlled american voltage source
  \item
    ``v\textless{}='' and ``i\textless{}='' do not rotate the sources
    anymore(see them as ``counting direction indication'', this can be
    different then the shape orientation); Use the option ``invert'' to
    change the direction of the source/apperance of the shape.
  \item
    current label ``i='' can now be used independent of the regular
    label ``l='' at current sources
  \item
    rewrite of current arrow placement. Current arrows can now also be
    rotated on zero-length paths
  \item
    New DIN/EN compliant operational amplifier symbol ``en amp''
  \end{itemize}
\item
  Version 0.8.1 (2017-03-25)

  \begin{itemize}
  \tightlist
  \item
    Fixed unwanted line through components if target coordinate is a
    name of a node
  \item
    Fixed position of labels with subscript letters.
  \item
    Absolute distance calculation in terms of ex at rotated labels
  \item
    Fixed label for transistor paths (no label drawn)
  \end{itemize}
\item
  Version 0.8 (2017-03-08)

  \begin{itemize}
  \tightlist
  \item
    Allow use of voltage label at a {[}short{]}
  \item
    Correct line joins between path components (to{[}\ldots{}{]})
  \item
    New Pole-shape .-. to fill perpendicular joins
  \item
    Fixed direction of controlled american current source
  \item
    Fixed incorrect scaling of magnetron
  \item
    Fixed: Number of american inductor coils not adjustable
  \item
    Fixed Battery Symbols and added new battery2 symbol
  \item
    Added non-inverting Schmitttrigger
  \end{itemize}
\item
  Version 0.7 (2016-09-08)

  \begin{itemize}
  \tightlist
  \item
    Added second annotation label, showing, e.g., the value of an
    component
  \item
    Added new symbol: magnetron
  \item
    Fixed name conflict of diamond shape with tikz.shapes package
  \item
    Fixed varcap symbol at small scalings
  \item
    New packet-option ``straightvoltages, to draw straight(no curved)
    voltage arrows
  \item
    New option ``invert'' to revert the node direction at paths
  \item
    Fixed american voltage label at special sources and battery
  \item
    Fixed/rotated battery symbol(longer lines by default positive
    voltage)
  \item
    New symbol Schmitttrigger
  \end{itemize}
\item
  Version 0.6 (2016-06-06)

  \begin{itemize}
  \tightlist
  \item
    Added Mechanical Symbols (damper,mass,spring)
  \item
    Added new connection style diamond, use (d-d)
  \item
    Added new sources voosource and ioosource (double zero-style)
  \item
    All diode can now drawn in a stroked way, just use globel option
    ``strokediode'' or stroke instead of full/empty, or D-. Use this
    option for compliance with DIN standard EN-60617
  \item
    Improved Shape of Diodes:tunnel diode, Zener diode, schottky diode
    (bit longer lines at cathode)
  \item
    Reworked igbt: New anchors G,gate and new L-shaped form Lnigbt,
    Lpigbt
  \item
    Improved shape of all fet-transistors and mirrored p-chan fets as
    default, as pnp, pmos, pfet are already. This means a
    backward-incompatibility, but smaller code, because p-channels
    mosfet are by default in the correct direction(source at top). Just
    remove the `yscale=-1' from your p-chan fets at old pictures.
  \end{itemize}
\item
  Version 0.5 (2016-04-24)

  \begin{itemize}
  \tightlist
  \item
    new option boxed and dashed for hf-symbols
  \item
    new option solderdot to enable/disable solderdot at source port of
    some fets
  \item
    new parts: photovoltaic source, piezo crystal, electrolytic
    capacitor, electromechanical device(motor, generator)
  \item
    corrected voltage and current direction(option to use old behaviour)
  \item
    option to show body diode at fet transistors
  \end{itemize}
\item
  Version 0.4

  \begin{itemize}
  \tightlist
  \item
    minor improvements to documentation
  \item
    comply with TDS
  \item
    merge high frequency symbols by Stefan Erhardt
  \item
    added switch (not opening nor closing)
  \item
    added solder dot in some transistors
  \item
    improved ConTeXt compatibility
  \end{itemize}
\item
  Version 0.3.1

  \begin{itemize}
  \tightlist
  \item
    different management of color\ldots{}
  \item
    fixed typo in documentation
  \item
    fixed an error in the angle computation in voltage and current
    routines
  \item
    fixed problem with label size when scaling a tikz picture
  \item
    added gas filled surge arrester
  \item
    added compatibility option to work with Tikz's own circuit library
  \item
    fixed infinite in arctan computation
  \end{itemize}
\item
  Version 0.3.0

  \begin{itemize}
  \tightlist
  \item
    fixed gate node for a few transistors
  \item
    added mixer
  \item
    added fully differential op amp (by Kristofer M. Monisit)
  \item
    now general settings for the drawing of voltage can be overridden
    for specific components
  \item
    made arrows more homogeneous (either the current one, or latex' bt
    pgf)
  \item
    added the single battery cell
  \item
    added fuse and asymmetric fuse
  \item
    added toggle switch
  \item
    added varistor, photoresistor, thermocouple, push button
  \item
    added thermistor, thermistor ptc, thermistor ptc
  \item
    fixed misalignment of voltage label in vertical bipoles with names
  \item
    added isfet
  \item
    added noiseless, protective, chassis, signal and reference grounds
    (Luigi «Liverpool»)
  \end{itemize}
\item
  Version 0.2.4

  \begin{itemize}
  \tightlist
  \item
    added square voltage source (contributed by Alistair Kwan)
  \item
    added buffer and plain amplifier (contributed by Danilo Piazzalunga)
  \item
    added squid and barrier (contributed by Cor Molenaar)
  \item
    added antenna and transmission line symbols contributed by Leonardo
    Azzinnari
  \item
    added the changeover switch spdt (suggestion of Fabio Maria
    Antoniali)
  \item
    rename of context.tex and context.pdf (thanks to Karl Berry)
  \item
    updated the email address
  \item
    in documentation, fixed wrong (non-standard) labelling of the axis
    in an example (thanks to prof. Claudio Beccaria)
  \item
    fixed scaling inconsistencies in quadrupoles
  \item
    fixed division by zero error on certain vertical paths
  \item
    introduced options straighlabels, rotatelabels, smartlabels
  \end{itemize}
\item
  Version 0.2.3

  \begin{itemize}
  \tightlist
  \item
    fixed compatibility problem with label option from tikz
  \item
    Fixed resizing problem for shape ground
  \item
    Variable capacitor
  \item
    polarized capacitor
  \item
    ConTeXt support (read the manual!)
  \item
    nfet, nigfete, nigfetd, pfet, pigfete, pigfetd (contribution of
    Clemens Helfmeier and Theodor Borsche)
  \item
    njfet, pjfet (contribution of Danilo Piazzalunga)
  \item
    pigbt, nigbt
  \item
    \emph{backward incompatibility} potentiometer is now the standard
    resistor-with-arrow-in-the-middle; the old potentiometer is now
    known as variable resistor (or vR), similarly to variable inductor
    and variable capacitor
  \item
    triac, thyristor, memristor
  \item
    new property ``name'' for bipoles
  \item
    fixed voltage problem for batteries in american voltage mode
  \item
    european logic gates
  \item
    \emph{backward incompatibility} new american standard inductor. Old
    american inductor now called ``cute inductor''
  \item
    \emph{backward incompatibility} transformer now linked with the
    chosen type of inductor, and version with core, too. Similarly for
    variable inductor
  \item
    \emph{backward incompatibility} styles for selecting shape variants
    now end are in the plural to avoid conflict with paths
  \item
    new placing option for some tripoles (mostly transistors)
  \item
    mirror path style
  \end{itemize}
\item
  Version 0.2.2 - 20090520

  \begin{itemize}
  \tightlist
  \item
    Added the shape for lamps.
  \item
    Added options \texttt{europeanresistor}, \texttt{europeaninductor},
    \texttt{americanresistor} and \texttt{americaninductor}, with
    corresponding styles.
  \item
    FIXED: error in transistor arrow positioning and direction under
    negative \texttt{xscale} and \texttt{yscale}.
  \end{itemize}
\item
  Version 0.2.1 - 20090503

  \begin{itemize}
  \tightlist
  \item
    Op-amps added
  \item
    added options arrowmos and noarrowmos, to add arrows to pmos and
    nmos
  \end{itemize}
\item
  Version 0.2 - 20090417 First public release on CTAN

  \begin{itemize}
  \tightlist
  \item
    \emph{Backward incompatibility}: labels ending with
    \texttt{:}\textit{angle} are not parsed for positioning anymore.
  \item
    Full use of \TikZ~keyval features.
  \item
    White background is not filled anymore: now the network can be drawn
    on a background picture as well.
  \item
    Several new components added (logical ports, transistors, double
    bipoles, \ldots).
  \item
    Color support.
  \item
    Integration with \{\ttfamily siunitx\}.
  \item
    Voltage, american style.
  \item
    Better code, perhaps. General cleanup at the very least.
  \end{itemize}
\item
  Version 0.1 - 2007-10-29 First public release
\end{itemize}


==> circuitikz/doc/circuitikz-context.tex <==

\usemodule[circuitikz]

\starttext
 
A simple example to test the installation.

\startcircuitikz[scale=1.2]
	\draw 
  (0,2) to[I=1\milli\ampere] (2,2)
        to[R, l_=2\kilo\ohm, *-*] (0,0)
        to[R, l_=2\kilo\ohm] (2,0)
        to[V, v_=2\volt] (2,2)
        to[cspst, l=$t_0$] (4,2) -- (4,1.5)
        to [generic, i=$i_1$, v=$v_1$] (4,-.5) -- (4,-1.5)
  (0,2) -- (0,-1.5) to[V, v_=4\volt] (2,-1.5)
        to [R, l=1\kilo\ohm] (4,-1.5);
\stopcircuitikz
 
\stoptext


==> circuitikz/tex/pgfcirc.defines.tex <==

%% Options

%%%%%%%%%%%%
%% Dimensions

% coordinates
\newdimen\pgf@circ@res@up
\newdimen\pgf@circ@res@down
\newdimen\pgf@circ@res@zero
\newdimen\pgf@circ@res@left
\newdimen\pgf@circ@res@right
\newdimen\pgf@circ@res@other
\newdimen\pgf@circ@res@step
\newdimen\pgf@circ@res@temp
% inital thickness
\newdimen \pgfstartlinewidth
%% Keys

\long\def\pgf@circ@comment#1{}

\def\circuitikzbasekey{/tikz/circuitikz}

\pgfkeys{\circuitikzbasekey/.is family}

\def\circuitikzset#1{\pgfkeys{\circuitikzbasekey,#1}}
\let\ctikzset\circuitikzset
\def\ctikzvalof#1{\pgfkeysvalueof{\circuitikzbasekey/#1}}
\def\ctikzsetvalof#1#2{\pgfkeyssetvalue{\circuitikzbasekey/#1}{#2}}

\newif\ifpgf@circ@siunitx
\newif\ifpgf@circuit@compat
\newif\ifpgf@circ@oldvoltagedirection

% Option ">" for twoports
\newif\ifpgf@circuit@inputarrow
\ctikzset{>/.add code={}{\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/.is choice}
\ctikzset{inputarrow/true/.code={\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/false/.code={\pgf@circuit@inputarrowfalse}}

% Option "boxed" for nodes and twoports
\newif\ifpgf@circuit@boxed
\pgfkeys{/tikz/boxed/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{boxed/.add code={}{\pgf@circuit@boxedtrue}}
\pgfkeys{/tikz/box/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{box/.add code={}{\pgf@circuit@boxedtrue}}

% Option "dashed" for nodes and twoports
\newif\ifpgf@circuit@dashed
\pgfkeys{/tikz/dashed/.add code={}{\pgf@circuit@dashedtrue}}
\ctikzset{dashed/.add code={}{\pgf@circuit@dashedtrue}}

% Option "t=*" for nodes
\pgfkeys{/tikz/t/.add code={}{\ctikzset{text=#1}}}



\ctikzset{bipoles/.is family}
\ctikzset{bipoles/border margin/.initial=1.1}
\ctikzset{bipoles/thickness/.initial=2} 
\ctikzset{nodes width/.initial=.04}
\newdimen\pgf@circ@Rlen 
\ctikzset{bipoles/length/.code={\pgf@circ@Rlen = #1}}
\pgf@circ@Rlen = 1.4cm

\ctikzset{monopoles/.is family}
\ctikzset{monopoles/ground/width/.initial=.25}
\ctikzset{monopoles/tground/thickness/.initial=3}
\ctikzset{monopoles/vcc/width/.initial=.2}
\ctikzset{monopoles/match/width/.initial=.4}
\ctikzset{monopoles/chassis/width/.initial=.25}
\ctikzset{monopoles/alternative chassis/width/.initial=.25}
\ctikzset{monopoles/equipotentiality/width/.initial=.25}
\ctikzset{monopoles/tlinestub/width/.initial=.25}          
\ctikzset{monopoles/antenna/width/.initial=.25}            
\ctikzset{monopoles/antenna/label/xanchor/.initial=.4}            
\ctikzset{monopoles/antenna/label/yanchor/.initial=.75}            
\ctikzset{monopoles/txantenna/label/xanchor/.initial=.4}            
\ctikzset{monopoles/txantenna/label/yanchor/.initial=.75}            
\ctikzset{monopoles/txantenna/width/.initial=.25}
\ctikzset{monopoles/rxantenna/label/xanchor/.initial=.4}            
\ctikzset{monopoles/rxantenna/label/yanchor/.initial=.75}            
\ctikzset{monopoles/rxantenna/width/.initial=.25}

\ctikzset{bipoles/resistor/height/.initial=.3}
\ctikzset{bipoles/resistor/width/.initial=.8}
\ctikzset{bipoles/potentiometer/height/.initial=.8}
\ctikzset{bipoles/potentiometer/height 2/.initial=.3}
\ctikzset{bipoles/potentiometer/width/.initial=.8}
\ctikzset{bipoles/photoresistor/height/.initial=.6}
\ctikzset{bipoles/photoresistor/height 2/.initial=.3}
\ctikzset{bipoles/photoresistor/width/.initial=.8}
\ctikzset{bipoles/thermistor/main/.initial=.7}
\ctikzset{bipoles/thermistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/width/.initial=.8}
\ctikzset{bipoles/thermistorntc/main/.initial=.7}
\ctikzset{bipoles/thermistorntc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistorptc/width/.initial=.8}
\ctikzset{bipoles/thermistorptc/main/.initial=.7}
\ctikzset{bipoles/thermistorptc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorptc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistor/width/.initial=.8}
\ctikzset{bipoles/varistor/main/.initial=.7}
\ctikzset{bipoles/varistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/varistor/width/.initial=.8}
\ctikzset{bipoles/vresistor/height/.initial=.6}
\ctikzset{bipoles/vresistor/width/.initial=.8}
\ctikzset{bipoles/cuteinductor/height/.initial=.3}
\ctikzset{bipoles/cuteinductor/lower coil height/.initial=.15}	
\ctikzset{bipoles/cuteinductor/width/.initial=.6}
\ctikzset{bipoles/cuteinductor/coils/.initial=5}
\ctikzset{bipoles/cuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
\ctikzset{bipoles/americaninductor/height/.initial=.3}
\ctikzset{bipoles/americaninductor/height 2/.initial=.1}
\ctikzset{bipoles/americaninductor/width/.initial=.8}
\ctikzset{bipoles/americaninductor/coils/.initial=4}
\ctikzset{bipoles/americaninductor/coil height/.initial=.15}
\ctikzset{bipoles/vcuteinductor/height/.initial=.6}
\ctikzset{bipoles/vcuteinductor/lower coil height/.initial=.3}	
\ctikzset{bipoles/vcuteinductor/width/.initial=.6}
\ctikzset{bipoles/vcuteinductor/coils/.initial=5}
\ctikzset{bipoles/vcuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
\ctikzset{bipoles/vamericaninductor/height/.initial=.6}
\ctikzset{bipoles/vamericaninductor/height 2/.initial=.2}
\ctikzset{bipoles/vamericaninductor/width/.initial=.8}
\ctikzset{bipoles/vamericaninductor/coils/.initial=4}
\ctikzset{bipoles/vamericaninductor/coil height/.initial=.15}
\ctikzset{bipoles/esource/height/.initial=.60}
\ctikzset{bipoles/esource/width/.initial=.60}
\ctikzset{bipoles/pvsource/height/.initial=.60}
\ctikzset{bipoles/pvsource/width/.initial=.60}
\ctikzset{bipoles/isource/height/.initial=.60}
\ctikzset{bipoles/isource/width/.initial=.60}
\ctikzset{bipoles/oosource/height/.initial=.60}
\ctikzset{bipoles/oosource/width/.initial=.60}
\ctikzset{bipoles/oosource/circlesize/.initial=.65}%circlesize+circleoffset should be =1
\ctikzset{bipoles/oosource/circleoffset/.initial=.35}%circlesize+circleoffset should be =1
\ctikzset{bipoles/dcisource/height/.initial=.60}
\ctikzset{bipoles/dcisource/width/.initial=.60}
\ctikzset{bipoles/dcvsource/height/.initial=.60}
\ctikzset{bipoles/dcvsource/width/.initial=.60}
\ctikzset{bipoles/vsourcetri/height/.initial=.60}
\ctikzset{bipoles/vsourcetri/width/.initial=.60}
\ctikzset{bipoles/isourceam/height/.initial=.60}
\ctikzset{bipoles/isourceam/width/.initial=.60}
\ctikzset{bipoles/vsource/height/.initial=.60}
\ctikzset{bipoles/vsource/width/.initial=.60}
\ctikzset{bipoles/vsourceam/height/.initial=.60}
\ctikzset{bipoles/vsourceam/width/.initial=.60}
\ctikzset{bipoles/vsourceam/margin/.initial=.7}
\ctikzset{bipoles/isourcesin/height/.initial=.60}
\ctikzset{bipoles/isourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesin/height/.initial=.60}
\ctikzset{bipoles/vsourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesquare/height/.initial=.60}
\ctikzset{bipoles/vsourcesquare/width/.initial=.60}
\ctikzset{bipoles/cisource/height/.initial=.7}
\ctikzset{bipoles/cisource/width/.initial=.7}
\ctikzset{bipoles/cisourceam/height/.initial=.7}
\ctikzset{bipoles/cisourceam/width/.initial=.7}
\ctikzset{bipoles/cvsource/height/.initial=.7}
\ctikzset{bipoles/cvsource/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/height/.initial=.7}
\ctikzset{bipoles/cvsourceam/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/margin/.initial=.7}
\ctikzset{bipoles/cvsourceam/text scale/.initial=1}
\ctikzset{bipoles/cisourcesin/width/.initial=.7}
\ctikzset{bipoles/cvsourcesin/height/.initial=.7}
\ctikzset{bipoles/cvsourcesin/width/.initial=.7}
\ctikzset{bipoles/capacitor/height/.initial=.6}
\ctikzset{bipoles/capacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/height/.initial=.5}
\ctikzset{bipoles/ecapacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/font/.initial= \fontsize{6}{0}\selectfont\boldmath}
\ctikzset{bipoles/pcapacitor/height/.initial=.6}
\ctikzset{bipoles/pcapacitor/width/.initial=.2}
\ctikzset{bipoles/pcapacitor/bend width/.initial=1.1}
\ctikzset{bipoles/vcapacitor/height/.initial=.6}
\ctikzset{bipoles/vcapacitor/width/.initial=.5}
\ctikzset{bipoles/vcapacitor/capacitor width/.initial=.4}
\ctikzset{bipoles/piezoelectric/height/.initial=.7}
\ctikzset{bipoles/piezoelectric/width/.initial=.5}
\ctikzset{bipoles/battery/height/.initial=.6}
\ctikzset{bipoles/battery/width/.initial=.3}
\ctikzset{bipoles/battery1/height/.initial=.6}
\ctikzset{bipoles/battery1/width/.initial=.3}
\ctikzset{bipoles/battery2/height/.initial=.6}
\ctikzset{bipoles/battery2/width/.initial=.3}
\ctikzset{bipoles/diode/height/.initial=.50}
\ctikzset{bipoles/diode/width/.initial=.40}
\ctikzset{bipoles/varcap/height/.initial=.50}
\ctikzset{bipoles/varcap/width/.initial=.45}
\ctikzset{bipoles/spst/height/.initial=.35}
\ctikzset{bipoles/spst/width/.initial=.35}
\ctikzset{bipoles/spst/depth/.initial=.2}
\ctikzset{bipoles/nos/height/.initial=.3}
\ctikzset{bipoles/nos/width/.initial=.35}
\ctikzset{bipoles/ncs/height/.initial=.35}
\ctikzset{bipoles/ncs/width/.initial=.35}
\ctikzset{bipoles/generic/height/.initial=.30}
\ctikzset{bipoles/generic/width/.initial=.80}
\ctikzset{bipoles/european gas filled surge arrester/height/.initial=.30}
\ctikzset{bipoles/european gas filled surge arrester/width/.initial=.80}
\ctikzset{bipoles/european gas filled surge arrester/inside/.initial=.30}
\ctikzset{bipoles/american gas filled surge arrester/height/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/width/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/inside/.initial=.15}
\ctikzset{bipoles/american gas filled surge arrester/dot x/.initial=.25}
\ctikzset{bipoles/american gas filled surge arrester/dot y/.initial=.45}
\ctikzset{bipoles/american gas filled surge arrester/size/.initial=.1}
\ctikzset{bipoles/fuse/height/.initial=.20}
\ctikzset{bipoles/fuse/width/.initial=.50}
\ctikzset{bipoles/afuse/height/.initial=.20}
\ctikzset{bipoles/afuse/width/.initial=.50}
\ctikzset{bipoles/generic potentiometer/height/.initial=.80}
\ctikzset{bipoles/generic potentiometer/height 2/.initial=.30}
\ctikzset{bipoles/generic potentiometer/width/.initial=.80}
\ctikzset{bipoles/ageneric/height/.initial=.30}
\ctikzset{bipoles/ageneric/width/.initial=.80}
\ctikzset{bipoles/memristor/height/.initial=.30}
\ctikzset{bipoles/memristor/wave height/.initial=.5}
\ctikzset{bipoles/memristor/width/.initial=.80}
\ctikzset{bipoles/tgeneric/height/.initial=.70}
\ctikzset{bipoles/tgeneric/width/.initial=.80}
\ctikzset{bipoles/tfullgeneric/height/.initial=.70}
\ctikzset{bipoles/tfullgeneric/width/.initial=.80}
\ctikzset{bipoles/fullgeneric/height/.initial=.30}
\ctikzset{bipoles/fullgeneric/width/.initial=.80}
\ctikzset{bipoles/open/height/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/width/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/voltage/straight label distance/.initial=0}
\ctikzset{bipoles/open/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/short/height/.initial=0} %dummy height for voltage positioning
\ctikzset{bipoles/short/width/.initial=0} %dummy width for voltage positioning
%\ctikzset{bipoles/short/voltage/straight label distance/.initial=.2}
%\ctikzset{bipoles/short/voltage/distance from node/.initial=.5}
\ctikzset{bipoles/ammeter/height/.initial=.60}
\ctikzset{bipoles/ammeter/width/.initial=.60}
\ctikzset{bipoles/ohmmeter/height/.initial=.60}
\ctikzset{bipoles/ohmmeter/width/.initial=.60}
\ctikzset{bipoles/voltmeter/height/.initial=.60}
\ctikzset{bipoles/voltmeter/width/.initial=.60}
\ctikzset{bipoles/buffer/height/.initial=1}
\ctikzset{bipoles/buffer/width/.initial=1}
\ctikzset{bipoles/not port/width/.initial=1}
\ctikzset{bipoles/not port/height/.initial=.8}
\ctikzset{bipoles/not port/circle width/.initial=.15}
\ctikzset{bipoles/lamp/height/.initial=.60}
\ctikzset{bipoles/lamp/width/.initial=.60}
\ctikzset{bipoles/tline/height/.initial=.3}
\ctikzset{bipoles/tline/width/.initial=.8}
\ctikzset{bipoles/squid/height/.initial=.60}
\ctikzset{bipoles/squid/width/.initial=.60}
\ctikzset{bipoles/barrier/height/.initial=.60}
\ctikzset{bipoles/barrier/width/.initial=.60}
\ctikzset{bipoles/thermocouple/height/.initial=.250}
\ctikzset{bipoles/thermocouple/height 2/.initial=.60}
\ctikzset{bipoles/thermocouple/width/.initial=.140}
\ctikzset{bipoles/pushbutton/height/.initial=.5}
\ctikzset{bipoles/pushbutton/height 2/.initial=.0}
\ctikzset{bipoles/pushbutton/width/.initial=.50}

\ctikzset{bipoles/twoport/width/.initial=.7}
\ctikzset{bipoles/twoport/height/.initial=.7}
\ctikzset{bipoles/twoport/text/.initial=}
\ctikzset{bipoles/vco/width/.initial=.7}
\ctikzset{bipoles/bandpass/width/.initial=.7}
\ctikzset{bipoles/bandstop/width/.initial=.7}
\ctikzset{bipoles/highpass/width/.initial=.7}
\ctikzset{bipoles/lowpass/width/.initial=.7}
\ctikzset{bipoles/adc/width/.initial=.7}
\ctikzset{bipoles/dac/width/.initial=.7}
\ctikzset{bipoles/dsp/width/.initial=.7}
\ctikzset{bipoles/fft/width/.initial=.7}
\ctikzset{bipoles/amp/width/.initial=.7}
\ctikzset{bipoles/vamp/width/.initial=.7}
\ctikzset{bipoles/piattenuator/width/.initial=.7}
\ctikzset{bipoles/vpiattenuator/width/.initial=.7}
\ctikzset{bipoles/tattenuator/width/.initial=.7}
\ctikzset{bipoles/vtattenuator/width/.initial=.7}
\ctikzset{bipoles/phaseshifter/width/.initial=.7}
\ctikzset{bipoles/vphaseshifter/width/.initial=.7}
\ctikzset{bipoles/detector/width/.initial=.7}


\newif\ifpgf@circuit@trans@depletiontype
\pgf@circuit@trans@depletiontypefalse

\newif\ifpgf@circuit@mos@arrows
\ctikzset{tripoles/mos style/.is choice}
\ctikzset{tripoles/mos style/no arrows/.code={\pgf@circuit@mos@arrowsfalse}}
\ctikzset{tripoles/mos style/arrows/.code={\pgf@circuit@mos@arrowstrue}}

% Option solderdot for fet 
\newif\ifpgf@circuit@fet@solderdot
\pgfkeys{/tikz/solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\ctikzset{solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\pgfkeys{/tikz/nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}
\ctikzset{nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}

% Option bodydiode for fet 
\newif\ifpgf@circuit@fet@bodydiode
\pgfkeys{/tikz/bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\ctikzset{bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\pgfkeys{/tikz/nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}
\ctikzset{nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}

% Option draw fet without gate connection
\newif\ifpgf@circuit@bpt@drawgate
\pgf@circuit@bpt@drawgatetrue
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}

% Option draw bpt without base connection
\newif\ifpgf@circuit@bpt@drawbase
\pgf@circuit@bpt@drawbasetrue
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}

% Option draw bpt with optical input
\newif\ifpgf@circuit@bpt@drawphoto
\pgf@circuit@bpt@drawphotofalse
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}

% Option draw pmos with empty circle
\newif\ifpgf@circuit@pmos@emptycircle
\newif\ifpgf@circuit@pmos@emptycircle
\pgf@circuit@pmos@emptycirclefalse
\pgfkeys{/tikz/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}
\ctikzset{tripoles/pmos style/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}


\newif\ifpgf@circuit@trans@ntype
\pgf@circuit@trans@ntypetrue %default true
%\newif\ifpgf@circuit@trans@ptype
%\ctikzset{tripoles/nmos/.add code={\pgf@circuit@trans@ntypetrue}}
\ctikzset{tripoles/nmos/width/.initial=.7}
\ctikzset{tripoles/nmos/gate height/.initial=.35}
\ctikzset{tripoles/nmos/base height/.initial=.5}
\ctikzset{tripoles/nmos/conn height/.initial=0}
\ctikzset{tripoles/nmos/height/.initial=1.1}
\ctikzset{tripoles/nmos/base width/.initial=.5}
\ctikzset{tripoles/nmos/gate width/.initial=.62}
\ctikzset{tripoles/nmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nmos/curr direction/.initial=1}

\ctikzset{tripoles/pmos/width/.initial=.7}
\ctikzset{tripoles/pmos/gate height/.initial=.35}
\ctikzset{tripoles/pmos/base height/.initial=.5}
\ctikzset{tripoles/pmos/conn height/.initial=0}
\ctikzset{tripoles/pmos/height/.initial=1.1}
\ctikzset{tripoles/pmos/base width/.initial=.5}
\ctikzset{tripoles/pmos/gate width/.initial=.62}
\ctikzset{tripoles/pmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pmos/curr direction/.initial=-1}

\ctikzset{tripoles/nfet/width/.initial=.7}
\ctikzset{tripoles/nfet/gate height/.initial=.35}
\ctikzset{tripoles/nfet/base height/.initial=.5}
\ctikzset{tripoles/nfet/conn height/.initial=0}
\ctikzset{tripoles/nfet/height/.initial=1.1}
\ctikzset{tripoles/nfet/base width/.initial=.5}
\ctikzset{tripoles/nfet/gate width/.initial=.62}
\ctikzset{tripoles/nfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nfet/curr direction/.initial=1}

\ctikzset{tripoles/pfet/width/.initial=.7}
\ctikzset{tripoles/pfet/gate height/.initial=.35}
\ctikzset{tripoles/pfet/base height/.initial=.5}
\ctikzset{tripoles/pfet/conn height/.initial=0}
\ctikzset{tripoles/pfet/height/.initial=1.1}
\ctikzset{tripoles/pfet/base width/.initial=.5}
\ctikzset{tripoles/pfet/gate width/.initial=.62}
\ctikzset{tripoles/pfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pfet/curr direction/.initial=-1}

\ctikzset{tripoles/nigfete/width/.initial=.7}
\ctikzset{tripoles/nigfete/gate height/.initial=.35}
\ctikzset{tripoles/nigfete/base height/.initial=.5}
\ctikzset{tripoles/nigfete/conn height/.initial=.35}
\ctikzset{tripoles/nigfete/height/.initial=1.1}
\ctikzset{tripoles/nigfete/base width/.initial=.5}
\ctikzset{tripoles/nigfete/gate width/.initial=.62}
\ctikzset{tripoles/nigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfete/curr direction/.initial=1}

\ctikzset{tripoles/nigfetd/width/.initial=.7}
\ctikzset{tripoles/nigfetd/gate height/.initial=.35}
\ctikzset{tripoles/nigfetd/base height/.initial=.5}
\ctikzset{tripoles/nigfetd/conn height/.initial=.35}
\ctikzset{tripoles/nigfetd/height/.initial=1.1}
\ctikzset{tripoles/nigfetd/base width/.initial=.5}
\ctikzset{tripoles/nigfetd/gate width/.initial=.62}
\ctikzset{tripoles/nigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetd/curr direction/.initial=1}

\ctikzset{tripoles/nigfetebulk/width/.initial=.7}
\ctikzset{tripoles/nigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/nigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/nigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/nigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/nigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetebulk/curr direction/.initial=1}

\ctikzset{tripoles/pigfete/width/.initial=.7}
\ctikzset{tripoles/pigfete/gate height/.initial=.35}
\ctikzset{tripoles/pigfete/base height/.initial=.5}
\ctikzset{tripoles/pigfete/conn height/.initial=.35}
\ctikzset{tripoles/pigfete/height/.initial=1.1}
\ctikzset{tripoles/pigfete/base width/.initial=.5}
\ctikzset{tripoles/pigfete/gate width/.initial=.62}
\ctikzset{tripoles/pigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfete/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetd/width/.initial=.7}
\ctikzset{tripoles/pigfetd/gate height/.initial=.35}
\ctikzset{tripoles/pigfetd/base height/.initial=.5}
\ctikzset{tripoles/pigfetd/conn height/.initial=.35}
\ctikzset{tripoles/pigfetd/height/.initial=1.1}
\ctikzset{tripoles/pigfetd/base width/.initial=.5}
\ctikzset{tripoles/pigfetd/gate width/.initial=.62}
\ctikzset{tripoles/pigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetd/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetebulk/width/.initial=.7}
\ctikzset{tripoles/pigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/pigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/pigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/pigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/pigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetebulk/curr direction/.initial=-1}

\ctikzset{tripoles/npn/width/.initial=.6}
\ctikzset{tripoles/npn/base height/.initial=.45}
\ctikzset{tripoles/npn/base height 2/.initial=.15}
\ctikzset{tripoles/npn/base height/.initial=.4}
\ctikzset{tripoles/npn/conn height/.initial=0}
\ctikzset{tripoles/npn/height/.initial=1.1}
\ctikzset{tripoles/npn/base width/.initial=.5}
\ctikzset{tripoles/npn/bodydiode scale/.initial=.3}
\ctikzset{tripoles/npn/bodydiode distance/.initial=.3}
\ctikzset{tripoles/npn/bodydiode conn/.initial=.6}
\ctikzset{tripoles/npn/curr direction/.initial=1}

\ctikzset{tripoles/pnp/width/.initial=.6}
\ctikzset{tripoles/pnp/base height/.initial=.45}
\ctikzset{tripoles/pnp/base height 2/.initial=.15}
\ctikzset{tripoles/pnp/base height/.initial=.4}
\ctikzset{tripoles/pnp/conn height/.initial=0}
\ctikzset{tripoles/pnp/height/.initial=1.1}
\ctikzset{tripoles/pnp/base width/.initial=.5}
\ctikzset{tripoles/pnp/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pnp/curr direction/.initial=-1}

\ctikzset{tripoles/pigbt/width/.initial=.6}
\ctikzset{tripoles/pigbt/gate height/.initial=.45}
\ctikzset{tripoles/pigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/pigbt/base height/.initial=.4}
\ctikzset{tripoles/pigbt/conn height/.initial=0}
\ctikzset{tripoles/pigbt/height/.initial=1.1}
\ctikzset{tripoles/pigbt/gate width/.initial=.62}
\ctikzset{tripoles/pigbt/base width/.initial=.5}
\ctikzset{tripoles/pigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigbt/curr direction/.initial=-1}

\ctikzset{tripoles/nigbt/width/.initial=.6}
\ctikzset{tripoles/nigbt/gate height/.initial=.45}
\ctikzset{tripoles/nigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/nigbt/base height/.initial=.4}
\ctikzset{tripoles/nigbt/conn height/.initial=0}
\ctikzset{tripoles/nigbt/height/.initial=1.1}
\ctikzset{tripoles/nigbt/gate width/.initial=.62}
\ctikzset{tripoles/nigbt/base width/.initial=.5}
\ctikzset{tripoles/nigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigbt/curr direction/.initial=1}

\ctikzset{tripoles/Lpigbt/width/.initial=.6}
\ctikzset{tripoles/Lpigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lpigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lpigbt/base height/.initial=.4}
\ctikzset{tripoles/Lpigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lpigbt/height/.initial=1.1}
\ctikzset{tripoles/Lpigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lpigbt/base width/.initial=.5}
\ctikzset{tripoles/Lpigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lpigbt/curr direction/.initial=-1}

\ctikzset{tripoles/Lnigbt/width/.initial=.6}
\ctikzset{tripoles/Lnigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lnigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lnigbt/base height/.initial=.4}
\ctikzset{tripoles/Lnigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lnigbt/height/.initial=1.1}
\ctikzset{tripoles/Lnigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lnigbt/base width/.initial=.5}
\ctikzset{tripoles/Lnigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lnigbt/curr direction/.initial=1}

\ctikzset{tripoles/njfet/width/.initial=.7}
\ctikzset{tripoles/njfet/gate height/.initial=.5}
\ctikzset{tripoles/njfet/gate height 2/.initial=.35}
\ctikzset{tripoles/njfet/gate width/.initial=.5}
\ctikzset{tripoles/njfet/conn height/.initial=.35}
\ctikzset{tripoles/njfet/height/.initial=1.1}
\ctikzset{tripoles/njfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/njfet/curr direction/.initial=1}

\ctikzset{tripoles/pjfet/width/.initial=.7}
\ctikzset{tripoles/pjfet/gate height/.initial=.5}
\ctikzset{tripoles/pjfet/gate height 2/.initial=.35}
\ctikzset{tripoles/pjfet/gate width/.initial=.5}
\ctikzset{tripoles/pjfet/conn height/.initial=.35}
\ctikzset{tripoles/pjfet/height/.initial=1.1}
\ctikzset{tripoles/pjfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pjfet/curr direction/.initial=-1}

\ctikzset{tripoles/isfet/width/.initial=1}
\ctikzset{tripoles/isfet/gate height/.initial=.35}
\ctikzset{tripoles/isfet/base height/.initial=.5}
\ctikzset{tripoles/isfet/height/.initial=1.1}
\ctikzset{tripoles/isfet/base width/.initial=.3}
\ctikzset{tripoles/isfet/gate width/.initial=.5}
\ctikzset{tripoles/isfet/conn height/.initial=0}
\ctikzset{tripoles/isfet/wave width/.initial=.16}
\ctikzset{tripoles/isfet/wave amp/.initial=.06}
\ctikzset{tripoles/isfet/waves y sep/.initial=.22}
\ctikzset{tripoles/isfet/waves x sep/.initial=.8}
\ctikzset{tripoles/isfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/isfet/curr direction/.initial=1}

\newif\ifpgf@circuit@europeanlogicport
\ctikzset{logic ports/.is choice}
\ctikzset{logic ports/european/.code= {\pgf@circuit@europeanlogicporttrue } }
\ctikzset{logic ports/american/.code= {\pgf@circuit@europeanlogicportfalse } } 


\ctikzset{tripoles/american and port/width/.initial=1.1}
\ctikzset{tripoles/american and port/height/.initial=.8}
\ctikzset{tripoles/american and port/port width/.initial=.7}
\ctikzset{tripoles/american and port/input height/.initial=.5}
\ctikzset{tripoles/american nand port/width/.initial=1.1}
\ctikzset{tripoles/american nand port/height/.initial=.8}
\ctikzset{tripoles/american nand port/port width/.initial=.7}
\ctikzset{tripoles/american nand port/circle width/.initial=.15}
\ctikzset{tripoles/american nand port/input height/.initial=.5}
\ctikzset{tripoles/american or port/width/.initial=1.1}
\ctikzset{tripoles/american or port/height/.initial=.8}
\ctikzset{tripoles/american or port/port width/.initial=.7}
\ctikzset{tripoles/american or port/input height/.initial=.5}
\ctikzset{tripoles/american or port/input skip/.initial=.25}
\ctikzset{tripoles/american or port/aaa/.initial=.6}
\ctikzset{tripoles/american or port/bbb/.initial=.4} 
\ctikzset{tripoles/american or port/ccc/.initial=.5} 
\ctikzset{tripoles/american or port/ddd/.initial=.0}
\ctikzset{tripoles/american nor port/width/.initial=1.1}
\ctikzset{tripoles/american nor port/height/.initial=.8}
\ctikzset{tripoles/american nor port/port width/.initial=.7}
\ctikzset{tripoles/american nor port/input height/.initial=.5}
\ctikzset{tripoles/american nor port/input skip/.initial=.25}
\ctikzset{tripoles/american nor port/circle width/.initial=.15}
\ctikzset{tripoles/american nor port/aaa/.initial=.6}
\ctikzset{tripoles/american nor port/bbb/.initial=.4} 
\ctikzset{tripoles/american nor port/ccc/.initial=.5} 
\ctikzset{tripoles/american nor port/ddd/.initial=.0}
\ctikzset{tripoles/american xor port/width/.initial=1.1}
\ctikzset{tripoles/american xor port/height/.initial=.8}
\ctikzset{tripoles/american xor port/port width/.initial=.7}
\ctikzset{tripoles/american xor port/input height/.initial=.5}
\ctikzset{tripoles/american xor port/input skip/.initial=.15}
\ctikzset{tripoles/american xor port/distance/.initial=.1} 
\ctikzset{tripoles/american xor port/aaa/.initial=.6}
\ctikzset{tripoles/american xor port/bbb/.initial=.4} 
\ctikzset{tripoles/american xor port/ccc/.initial=.5} 
\ctikzset{tripoles/american xor port/ddd/.initial=.0}
\ctikzset{tripoles/american xnor port/width/.initial=1.1}
\ctikzset{tripoles/american xnor port/height/.initial=.8}
\ctikzset{tripoles/american xnor port/port width/.initial=.7}
\ctikzset{tripoles/american xnor port/input height/.initial=.5}
\ctikzset{tripoles/american xnor port/input skip/.initial=.15}
\ctikzset{tripoles/american xnor port/distance/.initial=.1} 
\ctikzset{tripoles/american xnor port/aaa/.initial=.6}
\ctikzset{tripoles/american xnor port/bbb/.initial=.4} 
\ctikzset{tripoles/american xnor port/ccc/.initial=.5} 
\ctikzset{tripoles/american xnor port/ddd/.initial=.0}
\ctikzset{tripoles/american xnor port/circle width/.initial=.15}
\ctikzset{tripoles/european and port/width/.initial=1.4}
\ctikzset{tripoles/european and port/height/.initial=.65}
\ctikzset{tripoles/european and port/reserved/.initial=.6}
\ctikzset{tripoles/european and port/input height/.initial=.6}
\ctikzset{tripoles/european or port/width/.initial=1.4}
\ctikzset{tripoles/european or port/height/.initial=.65}
\ctikzset{tripoles/european or port/reserved/.initial=.6}
\ctikzset{tripoles/european or port/input height/.initial=.6}
\ctikzset{tripoles/european xor port/width/.initial=1.4}
\ctikzset{tripoles/european xor port/height/.initial=.65}
\ctikzset{tripoles/european xor port/reserved/.initial=.6}
\ctikzset{tripoles/european xor port/input height/.initial=.6}
\ctikzset{tripoles/european nand port/width/.initial=1.4}
\ctikzset{tripoles/european nand port/not height/.initial=.3}
\ctikzset{tripoles/european nand port/not width/.initial=.8}
\ctikzset{tripoles/european nand port/height/.initial=.65}
\ctikzset{tripoles/european nand port/reserved/.initial=.6}
\ctikzset{tripoles/european nand port/input height/.initial=.6}
\ctikzset{tripoles/european not port/width/.initial=1.4}
\ctikzset{tripoles/european not port/not height/.initial=.3}
\ctikzset{tripoles/european not port/not width/.initial=.8}
\ctikzset{tripoles/european not port/height/.initial=.65}
\ctikzset{tripoles/european not port/reserved/.initial=.6}
\ctikzset{tripoles/european not port/input height/.initial=0}
\ctikzset{tripoles/european xnor port/width/.initial=1.4}
\ctikzset{tripoles/european xnor port/not height/.initial=.3}
\ctikzset{tripoles/european xnor port/not width/.initial=.8}
\ctikzset{tripoles/european xnor port/height/.initial=.65}
\ctikzset{tripoles/european xnor port/reserved/.initial=.6}
\ctikzset{tripoles/european xnor port/input height/.initial=.6}
\ctikzset{tripoles/european nor port/width/.initial=1.4}
\ctikzset{tripoles/european nor port/not height/.initial=.3}
\ctikzset{tripoles/european nor port/not width/.initial=.8}
\ctikzset{tripoles/european nor port/height/.initial=.65}
\ctikzset{tripoles/european nor port/reserved/.initial=.6}
\ctikzset{tripoles/european nor port/input height/.initial=.6}
\ctikzset{tripoles/op amp/width/.initial=1.7}
\ctikzset{tripoles/op amp/port width/.initial=.7}
\ctikzset{tripoles/op amp/height/.initial=1.4}
\ctikzset{tripoles/op amp/input height/.initial=.5}
\ctikzset{tripoles/op amp/up pos/.initial=.45}
\ctikzset{tripoles/op amp/font/.initial= \fontsize{10}{0}\selectfont\boldmath}%absolut font size needed!
\ctikzset{tripoles/en amp/width/.initial=1.7}
\ctikzset{tripoles/en amp/port width/.initial=.7}
\ctikzset{tripoles/en amp/height/.initial=1.6}
\ctikzset{tripoles/en amp/input height/.initial=.3}
\ctikzset{tripoles/en amp/up pos/.initial=.45}
\ctikzset{tripoles/en amp/font/.initial= \fontsize{10}{0}\selectfont\boldmath}%absolut font size needed!
\ctikzset{tripoles/en amp/font2/.initial= \fontsize{14}{0}\selectfont\boldmath}%absolut font size needed!
\ctikzset{tripoles/gm amp/width/.initial=1.7}
\ctikzset{tripoles/gm amp/port width/.initial=.7}
\ctikzset{tripoles/gm amp/height/.initial=1.4}
\ctikzset{tripoles/gm amp/input height/.initial=.5}
\ctikzset{tripoles/gm amp/up pos/.initial=.45}
\ctikzset{tripoles/plain amp/width/.initial=1.7}
\ctikzset{tripoles/plain amp/port width/.initial=.7}
\ctikzset{tripoles/plain amp/height/.initial=1.4}
\ctikzset{tripoles/plain amp/input height/.initial=.5}
\ctikzset{tripoles/plain amp/up pos/.initial=.45}

\ctikzset{tripoles/thyristor/height/.initial=1.10}
\ctikzset{tripoles/thyristor/height 2/.initial=.5}
\ctikzset{tripoles/thyristor/width/.initial=1.0}
\ctikzset{tripoles/thyristor/diode height/.initial=.5}
\ctikzset{tripoles/thyristor/diode width left/.initial=.4}
\ctikzset{tripoles/thyristor/diode width right/.initial=.3}

\ctikzset{tripoles/triac/height/.initial=1.1}
\ctikzset{tripoles/triac/width/.initial=1}
\ctikzset{tripoles/triac/diode width left/.initial=.3}
\ctikzset{tripoles/triac/diode width right/.initial=.3}

\ctikzset{tripoles/spdt/width/.initial=.85}
\ctikzset{tripoles/spdt/height/.initial=.45}
\ctikzset{tripoles/spdt/margin/.initial=.45}

\ctikzset{tripoles/toggleswitch/height/.initial=.8}
\ctikzset{tripoles/toggleswitch/height 2/.initial=.0}
\ctikzset{tripoles/toggleswitch/width/.initial=.80}

\ctikzset{tripoles/mixer/width/.initial=0.7}
\ctikzset{tripoles/adder/width/.initial=0.7}
\ctikzset{tripoles/circulator/width/.initial=.7}
\ctikzset{tripoles/oscillator/width/.initial=.7}


\ctikzset{tripoles/wilkinson/height/.initial=1.3}
\ctikzset{tripoles/wilkinson/width/.initial=1.3}

\ctikzset{quadpoles/transformer/width/.initial=1.5}
\ctikzset{quadpoles/transformer/width1/.initial=.4}
\ctikzset{quadpoles/transformer/height/.initial=1.5}
\ctikzset{quadpoles/transformer/height1/.initial=.8}
\ctikzset{quadpoles/transformer core/width/.initial=1.5}
\ctikzset{quadpoles/transformer core/height/.initial=1.5}
\ctikzset{quadpoles/transformer core/core height/.initial=.5}
\ctikzset{quadpoles/transformer core/core width/.initial=.05}
\ctikzset{quadpoles/gyrator/width/.initial=1.5}
\ctikzset{quadpoles/gyrator/height/.initial=1.5}
\ctikzset{quadpoles/fourport/width/.initial=1.3}
\ctikzset{quadpoles/fourport/height/.initial=1.3}
\ctikzset{quadpoles/coupler/width/.initial=1.3}
\ctikzset{quadpoles/coupler/height/.initial=1.3}
\ctikzset{quadpoles/coupler2/width/.initial=1.3}
\ctikzset{quadpoles/coupler2/height/.initial=1.3}

\ctikzset{/tikz/circuitikz/tripoles/magnetron/width/.initial=1}


% %Mechanical section
\ctikzset{/tikz/circuitikz/tripoles/elmech/height/.initial=.8}
\ctikzset{/tikz/circuitikz/tripoles/elmech/width/.initial=.6}
\ctikzset{bipoles/spring/height/.initial=.5}
\ctikzset{bipoles/spring/width/.initial=.5}
\ctikzset{bipoles/mass/height/.initial=.55}
\ctikzset{bipoles/mass/box height/.initial=.4}
\ctikzset{bipoles/mass/width/.initial=.5}

\ctikzset{bipoles/damper/height/.initial=.35}
\ctikzset{bipoles/damper/length/.initial=.3}
\ctikzset{bipoles/damper/width/.initial=.4}


\ctikzset{bipole/.is family}
\ctikzset{bipole/kind/.initial = }
\ctikzset{bipole/name/.initial = }
\newif\ifpgf@circuit@bipole@isvoltage
\ctikzset{bipole/is voltage/.is if=pgf@circuit@bipole@isvoltage}
\newif\ifpgf@circuit@bipole@voltageoutsideofsymbol
\ctikzset{bipole/is voltageoutsideofsymbol/.is if=pgf@circuit@bipole@voltageoutsideofsymbol}
\newif\ifpgf@circuit@bipole@strokedsymbol
\ctikzset{bipole/is strokedsymbol/.is if=pgf@circuit@bipole@strokedsymbol}
\newif\ifpgf@circuit@bipole@iscurrent
\ctikzset{bipole/is current/.is if=pgf@circuit@bipole@iscurrent}

\ctikzset{bipole/voltage/.is family}
\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}
\newif\ifpgf@circuit@bipole@voltage@below
\ctikzset{bipole/voltage/position/.is choice}
\ctikzset{bipole/voltage/position/above/.code={\pgf@circuit@bipole@voltage@belowfalse}}
\ctikzset{bipole/voltage/position/below/.code={\pgf@circuit@bipole@voltage@belowtrue}}

\ctikzset{bipole/voltage/label/unit/.initial=}
\ctikzset{bipole/voltage/label/name/.initial=}

\ctikzset{bipole/current/.is family}
\newif\ifpgf@circuit@bipole@current@backward
\ctikzset{bipole/current/direction/.is choice}
\ctikzset{bipole/current/direction/forward/.code={\pgf@circuit@bipole@current@backwardfalse}}
\ctikzset{bipole/current/direction/backward/.code={\pgf@circuit@bipole@current@backwardtrue}}
\newif\ifpgf@circuit@bipole@current@before
\ctikzset{bipole/current/x position/.is choice}
\ctikzset{bipole/current/x position/after/.code={\pgf@circuit@bipole@current@beforefalse}}
\ctikzset{bipole/current/x position/before/.code={\pgf@circuit@bipole@current@beforetrue}}
\newif\ifpgf@circuit@bipole@current@below
\ctikzset{bipole/current/y position/.is choice}
\ctikzset{bipole/current/y position/above/.code={\pgf@circuit@bipole@current@belowfalse}}
\ctikzset{bipole/current/y position/below/.code={\pgf@circuit@bipole@current@belowtrue}}
\ctikzset{bipole/current/label/unit/.initial=}
\ctikzset{bipole/current/label/name/.initial=}

\ctikzset{bipole/flow/.is family}
\newif\ifpgf@circuit@bipole@flow@backward
\ctikzset{bipole/flow/direction/.is choice}
\ctikzset{bipole/flow/direction/forward/.code={\pgf@circuit@bipole@flow@backwardfalse}}
\ctikzset{bipole/flow/direction/backward/.code={\pgf@circuit@bipole@flow@backwardtrue}}
\newif\ifpgf@circuit@bipole@flow@before
\ctikzset{bipole/flow/x position/.is choice}
\ctikzset{bipole/flow/x position/after/.code={\pgf@circuit@bipole@flow@beforefalse}}
\ctikzset{bipole/flow/x position/before/.code={\pgf@circuit@bipole@flow@beforetrue}}
\newif\ifpgf@circuit@bipole@flow@below
\ctikzset{bipole/flow/y position/.is choice}
\ctikzset{bipole/flow/y position/above/.code={\pgf@circuit@bipole@flow@belowfalse}}
\ctikzset{bipole/flow/y position/below/.code={\pgf@circuit@bipole@flow@belowtrue}}
\ctikzset{bipole/flow/label/unit/.initial=}
\ctikzset{bipole/flow/label/name/.initial=}
\ctikzset{flow/distance/.initial = .5}
\ctikzset{flow/offset/.initial = .2}%distance between flow-arrow and conductor


\ctikzset{bipole/label/.is family}
\ctikzset{bipole/label/position/.initial=90}
\ctikzset{bipole/label/unit/.initial=}
\ctikzset{bipole/label/name/.initial=}
\ctikzset{bipole/annotation/.is family}
\ctikzset{bipole/annotation/position/.initial=-90}
\ctikzset{bipole/annotation/unit/.initial=}
\ctikzset{bipole/annotation/name/.initial=}
\ctikzset{bipole/nodes/.is family}
\ctikzset{bipole/nodes/left/.is choice}
\ctikzset{bipole/nodes/left/none/.code={\ctikzsetvalof{bipole/nodes/left}{none}}}
\ctikzset{bipole/nodes/left/empty/.code={\ctikzsetvalof{bipole/nodes/left}{empty}}}
\ctikzset{bipole/nodes/left/full/.code={\ctikzsetvalof{bipole/nodes/left}{full}}}
\ctikzset{bipole/nodes/left/diamond/.code={\ctikzsetvalof{bipole/nodes/left}{diamond}}}
\ctikzset{bipole/nodes/left/rectjoinfill/.code={\ctikzsetvalof{bipole/nodes/left}{rectjoinfill}}}
\ctikzset{bipole/nodes/right/.is choice}
\ctikzset{bipole/nodes/right/none/.code={\ctikzsetvalof{bipole/nodes/right}{none}}}
\ctikzset{bipole/nodes/right/empty/.code={\ctikzsetvalof{bipole/nodes/right}{empty}}}
\ctikzset{bipole/nodes/right/full/.code={\ctikzsetvalof{bipole/nodes/right}{full}}}
\ctikzset{bipole/nodes/right/diamond/.code={\ctikzsetvalof{bipole/nodes/right}{diamond}}}
\ctikzset{bipole/nodes/right/rectjoinfill/.code={\ctikzsetvalof{bipole/nodes/right}{rectjoinfill}}}




\newif\ifpgf@circuit@europeanresistor
\ctikzset{resistor/.is choice}
\ctikzset{resistor/american/.code = \pgf@circuit@europeanresistorfalse }
\ctikzset{resistor/european/.code = \pgf@circuit@europeanresistortrue }

\ctikzset{inductor/.is choice}
\ctikzset{inductor/cute/.code={\ctikzsetvalof{inductor}{cute}}}
\ctikzset{inductor/european/.code={\ctikzsetvalof{inductor}{european}}}
\ctikzset{inductor/american/.code={\ctikzsetvalof{inductor}{american}}}

\newif\ifpgf@circuit@strokediode
\newif\ifpgf@circuit@fulldiode
\pgf@circuit@strokediodefalse
\pgf@circuit@fulldiodefalse

\ctikzset{diode/.is choice}
\ctikzset{diode/empty/.code = \pgf@circuit@fulldiodefalse\pgf@circuit@strokediodefalse}%default
\ctikzset{diode/full/.code = \pgf@circuit@fulldiodetrue }
\ctikzset{diode/stroke/.code = \pgf@circuit@strokediodetrue}

\tikzset{full diodes/.style = { \circuitikzbasekey/diode = full }}
\tikzset{empty diodes/.style = { \circuitikzbasekey/diode = empty }}
\tikzset{stroke diodes/.style = { \circuitikzbasekey/diode = stroke }}

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}


\newif\ifpgf@circ@siunitx
\newif\ifpgf@circ@siunitx@res

\ctikzset{straight/.is choice}
\ctikzset{straightvoltage value/.initial=true}
\ctikzset{straight/true/.code = {\pgf@circuit@bipole@voltage@straighttrue}}
\ctikzset{straight/false/.code = {\pgf@circuit@bipole@voltage@straightfalse}}
\ctikzset{straightvoltage/.style = {/tikz/circuitikz/straight=true}}
\newif\ifpgf@circuit@bipole@voltage@straight
\ctikzset{bipole/straight/.is if=pgf@circuit@bipole@voltage@straight}


\ctikzset{voltage/.is family}
\ctikzset{voltage/distance from node/.initial=.5} %\pgf@circ@Rlen units
\ctikzset{voltage/distance from line/.initial=.08} % pos, tra 0 e 1
\ctikzset{voltage/bump a/.initial=1.2}
\ctikzset{voltage/bump b/.initial=1.5}
\ctikzset{voltage/european label distance/.initial=1.4}
\ctikzset{voltage/american label distance/.initial=1.1}
% special cases
\ctikzset{bipoles/generic/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/generic/voltage/bump b/.initial=2}
\ctikzset{bipoles/generic/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermocouple/voltage/distance from node/.initial=.3}
\ctikzset{bipoles/thermocouple/voltage/bump b/.initial=2.2}
\ctikzset{bipoles/thermocouple/voltage/european label distance/.initial=1.5}
\ctikzset{bipoles/ageneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/ageneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/ageneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/fullgeneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/fullgeneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/fullgeneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/memristor/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/memristor/voltage/bump b/.initial=2}
\ctikzset{bipoles/memristor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/tline/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/tline/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/tline/voltage/european label distance/.initial=2.1}
%\ctikzset{bipoles/varistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/varistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/varistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/photoresistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/photoresistor/voltage/bump b/.initial=2}
\ctikzset{bipoles/photoresistor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/thermistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/thermistorntc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorntc/voltage/bump b/.initial=1.6}
%\ctikzset{bipoles/thermistorptc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorptc/voltage/bump b/.initial=1.6}

\ctikzset{current/.is family}
\ctikzset{current/distance/.initial = .5}


\tikzset{american currents/.style = { \circuitikzbasekey/current = american } }
\tikzset{european currents/.style = { \circuitikzbasekey/current = european } }
\tikzset{american voltages/.style = { \circuitikzbasekey/voltage = american } }
\tikzset{european voltages/.style = { \circuitikzbasekey/voltage = european } }
\tikzset{american resistors/.style = { \circuitikzbasekey/resistor = american } }
\tikzset{european resistors/.style = { \circuitikzbasekey/resistor = european } }

\newif\ifpgf@circuit@europeangfsurgearrester
\ctikzset{gas filled surge arrester choice/.is choice}
\ctikzset{gas filled surge arrester choice/european/.code= {\pgf@circuit@europeangfsurgearrestertrue } }
\ctikzset{gas filled surge arrester choice/american/.code= {\pgf@circuit@europeangfsurgearresterfalse } }

\tikzset{american gas filled surge arrester set/.style = { \circuitikzbasekey/gas filled surge arrester choice=american } }
\tikzset{european gas filled surge arrester set/.style = { \circuitikzbasekey/gas filled surge arrester choice=european } }
\tikzset{american inductors/.style = { \circuitikzbasekey/inductor = american } }
\tikzset{european inductors/.style = { \circuitikzbasekey/inductor = european } }
\tikzset{cute inductors/.style = { \circuitikzbasekey/inductor = cute } }
\tikzset{american ports/.style = { \circuitikzbasekey/logic ports = american } }
\tikzset{european ports/.style = { \circuitikzbasekey/logic ports = european } }
\tikzset{european/.style = { european currents, european voltages, european resistors, european inductors, european ports, european gas filled surge arrester set} }
\tikzset{american/.style = { american currents, american voltages, american resistors, american inductors, american ports, american gas filled surge arrester set} }
\tikzset{cute/.style = { european currents, european voltages, american resistors, cute inductors, american ports } }

% I should try to make the tree clearer (this voltaege conflicts with the options above)

\newif\ifpgf@circuit@europeanvoltage
\ctikzset{voltage/.is choice}
\ctikzset{voltage/american/.code = {\pgf@circuit@europeanvoltagefalse } }
\ctikzset{voltage/european/.code = {\pgf@circuit@europeanvoltagetrue } }

\newif\ifpgf@circuit@europeancurrent
\ctikzset{current/.is choice}
\ctikzset{current/american/.code = \pgf@circuit@europeancurrentfalse }
\ctikzset{current/european/.code = \pgf@circuit@europeancurrenttrue }

\ctikzset{label/align/.is choice}
\ctikzset{label/align/straight/.code={\ctikzsetvalof{label/align}{straight}}}
\ctikzset{label/align/rotate/.code={\ctikzsetvalof{label/align}{rotate}}}
\ctikzset{label/align/smart/.code={\ctikzsetvalof{label/align}{smart}}}

%%%%%%%%%% new
\pgfkeys{\circuitikzbasekey/.search also={/tikz}}


==> circuitikz/tex/pgfcircbipoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%% Generic macro for defining a bipole shape
% #1 - additional anchors
% #2 - lower y-size of the bipole (from the center).
% #3 - #shape is the name of the shape
% #4 - upper y-size of the bipole (from the center)
% #5 - width of the bipole
% #6 - macros drawing the bipole


\long\def\pgfcircdeclarebipole#1#2#3#4#5#6{
	\pgfdeclareshape{#3shape}{
	
	\savedanchor{\northeast}{
		\pgf@y=#4\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=#5\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	}
	\savedanchor{\northeastborder}{
		\pgf@y=#4\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
		\pgf@x=#5\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
		\pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
	}
	\savedanchor{\southwestborder}{
		\pgf@y=-#2\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
		\pgf@x=-#5\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
		\pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
	}
	\savedanchor{\southwest}{
		\pgf@y=-#2\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-#5\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	}
	\savedanchor{\centerpoint}{
		\pgf@circ@res@down=-#2\pgf@circ@Rlen
		\pgf@circ@res@up=#4\pgf@circ@Rlen
		\pgfpointorigin
		\pgf@y=\pgf@circ@res@up
		\advance\pgf@y by\pgf@circ@res@down
		\pgf@y=.5\pgf@y
	}
	\anchor{center}{\pgfpointorigin}
	\anchor{n}{
		\northeast
		\pgf@x=0cm
	}
	\anchor{ne}{
		\northeast
	}
	\anchor{nw}{
		\northeast
		\pgf@x=-\pgf@x
	}
	\anchor{e}{%
		\northeast
		\pgf@y=0cm
   }
	\anchor{s}{%
		\southwest
		\pgf@x=0cm
   }
	\anchor{se}{%
		\southwest
		\pgf@x=-\pgf@x
   }
	\anchor{sw}{%
		\southwest
   }
	\anchor{w}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{north}{
		\northeast
		\pgf@x=0cm
	}
	\anchor{east}{%
		\northeast
		\pgf@y=0cm
   }
	\anchor{south}{%
		\southwest
		\pgf@x=0cm
   }
	\anchor{west}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{right}{
		\northeast
		\pgf@y=0cm
	}
	\anchor{above}{
		\northeast
		\pgf@x=0cm
	}
	\anchor{left}{%
		\southwest
		\pgf@y=0cm
   }
	\anchor{below}{%
		\southwest
		\pgf@x=0cm                    
   }
	\anchor{a}{%
		\northeast
		\pgf@y=0cm
   }
	\anchor{b} {
		\southwest
		\pgf@y=0cm
	}
	\savedanchor{\textanchor}{%
		\pgf@y=\ht\pgfnodeparttextbox
		\pgf@x=-.5\wd\pgfnodeparttextbox
   }
	\anchor{text}{%
		\textanchor
   }
	\anchorborder{%
		\ifpgf@circuit@bipole@inverted
			\pgf@circ@res@left=-\pgf@x
			\pgf@circ@res@right=-\pgf@y
		\else
			\pgf@circ@res@left=\pgf@x
			\pgf@circ@res@right=\pgf@y
		\fi
		\ifdim\pgf@circ@res@right>0cm
			\pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\northeastborder}
		\else
	  		\southwestborder	
	  	\pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\pgfpoint{-\pgf@x}{-\pgf@y}}
		\fi
	}
	
	#1
	
	\backgroundpath{	
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
		
		\northeast
		\pgf@circ@res@up = \pgf@y 
		\pgf@circ@res@zero = 0cm
		\pgf@circ@res@left = -\pgf@x
		\pgf@circ@res@right = \pgf@x
		\southwest
		\pgf@circ@res@down = \pgf@y

 		\pgfstartlinewidth=\pgflinewidth
		\pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
		#6
			
		\pgfsetlinewidth{\pgfstartlinewidth}
	}
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Standard bipole shapes declarations

%% Resistor
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/resistor/height}}{resistor}{\ctikzvalof{bipoles/resistor/height}}{\ctikzvalof{bipoles/resistor/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments
	\pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
	\divide \pgf@circ@res@step by 12
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
	\pgf@circ@res@other = \pgf@circ@res@left
	\advance\pgf@circ@res@other by \pgf@circ@res@step 
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step 
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfsetbeveljoin
	\pgfusepath{draw}
}



%% Variable resistor
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vresistor/height}}{vresistor}{\ctikzvalof{bipoles/vresistor/height}}{\ctikzvalof{bipoles/vresistor/width}}{		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments
	\pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
	\divide \pgf@circ@res@step by 12
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
	
	\pgf@circ@res@other = \pgf@circ@res@left
	\advance\pgf@circ@res@other by \pgf@circ@res@step 
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step 
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfsetbeveljoin
	\pgfusepath{draw}
	
	\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@other}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@other}{\pgf@circ@res@down}}
		\pgfusepath{draw}
	\endpgfscope
}



%% Capacitor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/capacitor/height}}{capacitor}{\ctikzvalof{bipoles/capacitor/height}}{\ctikzvalof{bipoles/capacitor/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/capacitor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 5

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
}


%% Polar Capacitor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/pcapacitor/height}}{polarcapacitor}{\ctikzvalof{bipoles/pcapacitor/height}}{\ctikzvalof{bipoles/pcapacitor/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/pcapacitor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 5

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
				
		\pgfscope
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left+ \ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}{\pgf@circ@res@up}}
			\pgftransformrotate{-90}
			\pgfpathsine{\pgfpoint{\pgf@circ@res@up}{-\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
			\pgfpathcosine{\pgfpoint{\pgf@circ@res@up}{\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
			\pgfusepath{draw}
		\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
}

%% Electrolytic Capacitor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/ecapacitor/height}}{ecapacitor}{\ctikzvalof{bipoles/ecapacitor/height}}{\ctikzvalof{bipoles/ecapacitor/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/ecapacitor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 5
		\pgfsetrectcap
		% % % Draw plus pole
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfsetfillcolor{white} 
		\pgfusepath{draw,fill}
		% % Draw minus pole
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
				 \pgfsetfillcolor{black} 
				\pgfusepath{draw,fill}
		\pgfsetfillcolor{black} 
		% % plus pole annotation
		\pgftext[right,at=\pgfpoint{1.2\pgf@circ@res@left}{.6\pgf@circ@res@up}]
		{\pgfkeysvalueof{/tikz/circuitikz/bipoles/ecapacitor/font} $+$}	
}

%% Battery

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/battery/height}}{battery}{\ctikzvalof{bipoles/battery/height}}{\ctikzvalof{bipoles/battery/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/battery/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 6

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}

		\pgfusepath{draw}
}


%% Battery 1 % poles with equl thickness

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/battery1/height}}{battery1}{\ctikzvalof{bipoles/battery1/height}}{\ctikzvalof{bipoles/battery1/width}}{
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
		\pgfusepath{draw}

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
}

%% Battery 2 % negative pole thicker

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/battery2/height}}{battery2}{\ctikzvalof{bipoles/battery2/height}}{\ctikzvalof{bipoles/battery2/width}}{
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
		\pgfusepath{draw}

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfsetlinewidth{3\pgflinewidth}
		\pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}
		\pgfusepath{draw}
}


%% cute inductor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cuteinductor/lower coil height}}{cuteinductor}{\ctikzvalof{bipoles/cuteinductor/height}}{\ctikzvalof{bipoles/cuteinductor/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments

	\pgfmathsetlength{\pgf@circ@res@other}%width of small coil
	{0.5*\ctikzvalof{bipoles/cuteinductor/coil aspect}*\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/cuteinductor/coils}-1)}


	\pgfmathsetlength{\pgf@circ@res@step}
		{(\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cuteinductor/coils}/2}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
	\foreach \x in {2,...,\ctikzvalof{bipoles/cuteinductor/coils}}
	{
		\pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
		\pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
	}
	\pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}
}

%% variable cute inductor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vcuteinductor/lower coil height}}{vcuteinductor}{\ctikzvalof{bipoles/vcuteinductor/height}}{\ctikzvalof{bipoles/vcuteinductor/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments	
	
	\pgfmathsetlength{\pgf@circ@res@other}%width of small coil
	{0.5*\ctikzvalof{bipoles/vcuteinductor/coil aspect}*\ctikzvalof{bipoles/vcuteinductor/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/vcuteinductor/coils}-1)}


	\pgfmathsetlength{\pgf@circ@res@step}
		{(\ctikzvalof{bipoles/vcuteinductor/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/vcuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/vcuteinductor/coils}/2}

	\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
	\foreach \x in {2,...,\ctikzvalof{bipoles/vcuteinductor/coils}}
	{
		\pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
		\pgfpatharc{0}{-180}{\pgf@circ@res@other and -.5\pgf@circ@res@down}
	}
	\pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}
}

%% american inductor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/americaninductor/height 2}}{americaninductor}{\ctikzvalof{bipoles/americaninductor/height}}{\ctikzvalof{bipoles/americaninductor/width}}{
	\pgf@circ@res@step=\ctikzvalof{bipoles/americaninductor/width}\pgf@circ@Rlen
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}	
	\pgftransformationadjustments
	\advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
	\divide \pgf@circ@res@step by \ctikzvalof{bipoles/americaninductor/coils}
	\divide \pgf@circ@res@step by 2
	\pgf@circ@res@other = \ctikzvalof{bipoles/americaninductor/coil height}\pgf@circ@Rlen

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
	\foreach \x in {1,...,\ctikzvalof{bipoles/americaninductor/coils}}
	{
	\pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
	}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}
}

%% variable american inductor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vamericaninductor/height 2}}{vamericaninductor}{\ctikzvalof{bipoles/vamericaninductor/height}}{\ctikzvalof{bipoles/vamericaninductor/width}}{
	\pgf@circ@res@step=\ctikzvalof{bipoles/vamericaninductor/width}\pgf@circ@Rlen
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments
	\advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
	\divide \pgf@circ@res@step by \ctikzvalof{bipoles/vamericaninductor/coils}
	\divide \pgf@circ@res@step by 2
	\pgf@circ@res@other = \ctikzvalof{bipoles/vamericaninductor/coil height}\pgf@circ@Rlen

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
	\foreach \x in {1,...,\ctikzvalof{bipoles/vamericaninductor/coils}}
	{
	\pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
	}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}

	\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}


%% Independent voltage source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsource/height}}{vsource}{\ctikzvalof{bipoles/vsource/height}}{\ctikzvalof{bipoles/vsource/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}
}


%% Independent voltage source - American style

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourceam/height}}{vsourceAM}{\ctikzvalof{bipoles/vsourceam/height}}{\ctikzvalof{bipoles/vsourceam/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}
	\ifpgf@circ@oldvoltagedirection
		\pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$+$}
		\pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$-$}
	\else
		\pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$-$}
		\pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$+$}
	\fi
}



%% Independent sinusoidal voltage source
 
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourcesin/height}}{vsourcesin}{\ctikzvalof{bipoles/vsourcesin/height}}{\ctikzvalof{bipoles/vsourcesin/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}		
		
		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope
}

% Triangle Voltage source - contributed by Ralf Farkas
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourcetri/height}}{vsourcetri}{\ctikzvalof{bipoles/vsourcetri/height}}{\ctikzvalof{bipoles/vsourcetri/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}		
		
		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
			\pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@up}{0.75\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@up}{-0.75\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope
}


% Square Voltage source -  contributed by Alistair Kwan
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourcesquare/height}}{vsourcesquare}{\ctikzvalof{bipoles/vsourcesquare/height}}{\ctikzvalof{bipoles/vsourcesquare/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}
	\pgf@circ@res@up = .5\pgf@circ@res@up
	\pgfscope
		\pgftransformrotate{90}
		\pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
		\pgfpathlineto{\pgfpoint{-1\pgf@circ@res@up}{1\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{1\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{-1\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{-1\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}

% Triangle Voltage source - contributed by Ralf Farkas
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourcetri/height}}{vsourcetri}{\ctikzvalof{bipoles/vsourcetri/height}}{\ctikzvalof{bipoles/vsourcetri/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}		
		
		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
			\pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@up}{0.75\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@up}{-0.75\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope
}


%% Empty Source
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/esource/height}}{esource}{\ctikzvalof{bipoles/esource/height}}{\ctikzvalof{bipoles/esource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
	\pgfusepath{draw}
}

%% PV Source
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/pvsource/height}}{pvsource}{\ctikzvalof{bipoles/pvsource/height}}{\ctikzvalof{bipoles/pvsource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
	\pgfusepath{draw}

	\pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{0}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
	\pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{0}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@down}}

	\pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@down}}
	\pgfusepath{draw}

	%Arrow Part
	\pgfscope
	\pgfsetarrowsend{latex}
	\pgfpathmoveto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
	\pgfpathlineto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
	\pgfpathlineto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
	\pgfusepath{draw}
	\endpgfscope

}

%% Empty Source
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/esource/height}}{esource}{\ctikzvalof{bipoles/esource/height}}{\ctikzvalof{bipoles/esource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
	\pgfusepath{draw}
}

%% DC Current Source with open shape
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/dcisource/height}}{dcisource}{\ctikzvalof{bipoles/dcisource/height}}{\ctikzvalof{bipoles/dcisource/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpointorigin}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}}\pgfpatharc{0}{90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}}\pgfpatharc{0}{-90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}\pgfpatharc{180}{270}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}\pgfpatharc{180}{90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}	
	\pgfusepath{draw}

	\pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}
	\pgfscope

	\pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
	\endpgfscope
}

%% DC-Voltage source
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/dcvsource/height}}{dcvsource}{\ctikzvalof{bipoles/dcvsource/height}}{\ctikzvalof{bipoles/dcvsource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@left}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@right}}
	\pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@left}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@right}}
	\pgfusepath{draw}	
}


%% Independent current source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/isource/height}}{isource}{\ctikzvalof{bipoles/isource/height}}{\ctikzvalof{bipoles/isource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
	\pgfusepath{draw}
}

%% Independent double oo source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/oosource/height}}{oosource}{\ctikzvalof{bipoles/oosource/height}}{\ctikzvalof{bipoles/oosource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@left}{0}}
		{\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@left}
	\pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@right}{0}}
		{\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@right}	
	\pgfusepath{draw}
}


%% Independent current source - American

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/isourceam/height}}{isourceAM}{\ctikzvalof{bipoles/isourceam/height}}{\ctikzvalof{bipoles/isourceam/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}

	\pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}
	\pgfscope
		\pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
		\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
	\endpgfscope
}


%% Independent sinusoidal current source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/isource/height}}{isourcesin}{\ctikzvalof{bipoles/isource/height}}{\ctikzvalof{bipoles/isource/width}}{
	\pgfpointorigin
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfusepath{draw}
	
		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope

}


%% Controlled voltage source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cvsource/height}}{cvsource}{\ctikzvalof{bipoles/cvsource/height}}{\ctikzvalof{bipoles/cvsource/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfusepath{draw}		
}




%% Controlled voltage source - American
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cvsourceam/height}}{cvsourceAM}{\ctikzvalof{bipoles/cvsourceam/height}}{\ctikzvalof{bipoles/cvsourceam/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfusepath{draw}

	\ifpgf@circ@oldvoltagedirection
		\pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$+$}
		\pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$-$}
	\else
		\pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$-$}
		\pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$+$}
	\fi
}


%% Controlled sinusoidal voltage source
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cvsourcesin/height}}{cvsourcesin}{\ctikzvalof{bipoles/cvsourcesin/height}}{\ctikzvalof{bipoles/cvsourcesin/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

		\pgfscope
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfusepath{draw}		
		\endpgfscope	

		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope
}



%% Controlled sinusoidal current source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cvsourcesin/height}}{cisourcesin}{\ctikzvalof{bipoles/cvsourcesin/height}}{\ctikzvalof{bipoles/cvsourcesin/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

		\pgfscope
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfusepath{draw}		
		\endpgfscope	

		\pgf@circ@res@up = .5\pgf@circ@res@up
		\pgfscope
			\pgftransformrotate{90}
			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope
}




%% Controlled current source

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cisource/height}}{cisource}{\ctikzvalof{bipoles/cisource/height}}{\ctikzvalof{bipoles/cisource/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfusepath{draw}		
}




%% Controlled current source - American

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/cisourceam/height}}{cisourceAM}{\ctikzvalof{bipoles/cisourceam/height}}{\ctikzvalof{bipoles/cisourceam/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
			\pgfusepath{draw}		

	\pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}
	\pgfscope
		\pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
		\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
	\endpgfscope
}

%% Black generic diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fulldiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% Black Zener diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fullzdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}

%% Black alternative zigzag Zener diode
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fullzzdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black Schottky diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fullsdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope

}

%% Black tunnel diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fulltdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}

%% Black light emitting diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fulllediode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}

			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetarrowsend{latex'}
			\pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
			\pgfusepath{draw}
			\pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
			\pgfusepath{draw}

}

%% Black photodiode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{fullpdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw,fill}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}

			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetarrowsstart{latex'}
			\pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
			\pgfusepath{draw}
			\pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
			\pgfusepath{draw}
}

%% Black varcap

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/varcap/height}}{fullvarcap}{\ctikzvalof{bipoles/varcap/height}}{\ctikzvalof{bipoles/varcap/width}}{
	\pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
	\pgfsetlinewidth{\pgf@circ@res@temp}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
	\pgfusepath{draw,fill}
	%
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
}

%% Empty generic diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptydiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{


	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% Empty Zener diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptyzdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.6\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}

%% Empty alternative zigzag Zener diode
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptyzzdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}
%% Empty Schottky diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptysdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope

}

%% Empty tunnel diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptytdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}

%% Empty light emitting diode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptylediode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{
		
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}

			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetarrowsend{latex'}
			\pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
			\pgfusepath{draw}
			\pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
			\pgfusepath{draw}
}

%% Empty photodiode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/diode/height}}{emptypdiode}{\ctikzvalof{bipoles/diode/height}}{\ctikzvalof{bipoles/diode/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfscope
		\pgftransformxshift{\pgf@circ@res@left}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
		\pgfusepath{draw}
	\endpgfscope
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}

			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetarrowsstart{latex'}
			\pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
			\pgfusepath{draw}
			\pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
			\pgfusepath{draw}
}

%% Empty varcap

\pgfcircdeclarebipole{
	\anchor{strokepathstart}{
			\northeast
				\pgf@y=0cm
				\advance\pgf@x by -\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth
				\advance\pgf@x by -\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth
	}
	\anchor{strokepathend}{
		\northeast
		\pgf@y=0cm
	}	
	}{\ctikzvalof{bipoles/varcap/height}}{emptyvarcap}{\ctikzvalof{bipoles/varcap/height}}{\ctikzvalof{bipoles/varcap/width}}{
	\pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
	\pgfsetlinewidth{\pgf@circ@res@temp}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
	\pgfusepath{draw}
	%
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
}

%% (Closing) SPST
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/spst/depth}}{cspst}{\ctikzvalof{bipoles/spst/height}}{\ctikzvalof{bipoles/spst/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	
	\pgfsetarrowsstart{latex'}
	\pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{0\pgf@circ@res@down}}
	\pgfpatharcto{1.2\pgf@circ@res@right}{1.2\pgf@circ@res@right}{0}{0}{1}{\pgfpoint{.9\pgf@circ@res@left}{.9\pgf@circ@res@up}}
	\pgfsetbeveljoin
	\pgfusepath{draw}
}

%% Opening SPST
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/spst/depth}}{ospst}{\ctikzvalof{bipoles/spst/height}}{\ctikzvalof{bipoles/spst/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	
	\pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
	\pgfpatharcto{1.1\pgf@circ@res@right}{1.1\pgf@circ@res@right}{0}{0}{1}{\pgfpoint{.7\pgf@circ@res@left}{.9\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@left}{1\pgf@circ@res@up}}
	\pgfsetarrowsend{latex'}
	\pgfsetbeveljoin
	\pgfusepath{draw}
}

%% Normal open Switch
\pgfcircdeclarebipole{}{0}{nos}{\ctikzvalof{bipoles/nos/height}}{\ctikzvalof{bipoles/nos/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfsetbuttcap
	\pgfusepath{draw}
}

%% Normal closed Switch
\pgfcircdeclarebipole{}{0}{ncs}{\ctikzvalof{bipoles/ncs/height}}{\ctikzvalof{bipoles/ncs/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
}

%% Push Button
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/pushbutton/height 2}}{pushbutton}{\ctikzvalof{bipoles/pushbutton/height}}{\ctikzvalof{bipoles/pushbutton/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{0}{.5\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	
	\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
	\pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
	\pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
}

% % METERINGSHAPE
\long\def\drawmeteringcircle{
	\def\pgf@circ@temp{right}
	\ifx\tikz@res@label@pos\pgf@circ@temp
		\pgf@circ@res@step=-1.2\pgf@circ@res@up
	\else
		\def\pgf@circ@temp{below}
		\ifx\tikz@res@label@pos\pgf@circ@temp
			\pgf@circ@res@step=-1.2\pgf@circ@res@up
		\else
			\pgf@circ@res@step=1.2\pgf@circ@res@up
		\fi
	\fi
	%draw connections to circle
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}		
	\pgfpathlineto{\pgfpoint{.9\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathmoveto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}
	%draw circle
	\pgfscope
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
		\pgfusepath{draw}
	\endpgfscope
	%draw arrow
	\pgfscope
		\pgfsetarrowsend{latex}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
}
%AMPEREMETER
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/ammeter/height}}{ammeter}{\ctikzvalof{bipoles/ammeter/height}}{\ctikzvalof{bipoles/ammeter/width}}{
	\drawmeteringcircle
	\pgfnode{circle}{center}{\textbf{A}}{}{}
}
%OHMMETER
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/ohmmeter/height}}{ohmmeter}{\ctikzvalof{bipoles/ohmmeter/height}}{\ctikzvalof{bipoles/ohmmeter/width}}{
	\drawmeteringcircle
	\pgfnode{circle}{center}{\boldmath$\Omega$}{}{}
}
%VOLTMETER
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/voltmeter/height}}{voltmeter}{\ctikzvalof{bipoles/voltmeter/height}}{\ctikzvalof{bipoles/voltmeter/width}}{
	\drawmeteringcircle
	\pgfnode{circle}{center}{\textbf{V}}{}{}
		
}

%% Short circuit

\pgfcircdeclarebipole{}{0}{short}{0}{0}{ }

%% Open circuit

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/open/height}}{open}{\ctikzvalof{bipoles/open/height}}{\ctikzvalof{bipoles/open/width}}{

}

%% Generic bipole - used as resistor by some (bleah)

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/generic/height}}{generic}{\ctikzvalof{bipoles/generic/height}}{\ctikzvalof{bipoles/generic/width}}{

		%\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		%\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw} 
}


%% fuse

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/fuse/height}}{fuse}{\ctikzvalof{bipoles/fuse/height}}{\ctikzvalof{bipoles/fuse/width}}{

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
		\pgfusepath{draw}
		
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw} 
}



%% Generic bipole, filled - used as inductor by some (bleah)

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/fullgeneric/height}}{fullgeneric}{\ctikzvalof{bipoles/fullgeneric/height}}{\ctikzvalof{bipoles/fullgeneric/width}}{

		%\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		%\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw,fill} 
}


%% Generic asymmetric bipole 

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/ageneric/height}}{ageneric}{\ctikzvalof{bipoles/ageneric/height}}{\ctikzvalof{bipoles/ageneric/width}}{
		%\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		%\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw} 

			\pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
			\pgfusepath{stroke,fill}		
}


%% asymmetric fuse

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/afuse/height}}{afuse}{\ctikzvalof{bipoles/afuse/height}}{\ctikzvalof{bipoles/afuse/width}}{

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
		\pgfusepath{draw}
		
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw}
		
		\pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
			\pgfusepath{stroke,fill}		 
}




%% Memristor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/memristor/height}}{memristor}{\ctikzvalof{bipoles/memristor/height}}{\ctikzvalof{bipoles/memristor/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{.8*\pgf@circ@res@right}{0pt}}
					
		\pgfusepath{draw} 

			\pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
			\pgfusepath{stroke,fill}		
}




%% Generic empty tunable

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/tgeneric/height}}{tgeneric}{\ctikzvalof{bipoles/tgeneric/height}}{\ctikzvalof{bipoles/tgeneric/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		\endpgfscope
}

%% Photoresistor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/photoresistor/height 2}}{photoresistor}{\ctikzvalof{bipoles/photoresistor/height}}{\ctikzvalof{bipoles/photoresistor/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.3\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.05\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
		\pgfusepath{draw}
		\endpgfscope
}




%% Thermistor
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/thermistor/height}}{thermistor}{\ctikzvalof{bipoles/thermistor/height}}{\ctikzvalof{bipoles/thermistor/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistor/main}\pgf@circ@res@up}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		%\pgfscope
		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		%\endpgfscope
}


%% Thermistor PTC
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/thermistorptc/height 2}}{thermistorptc}{\ctikzvalof{bipoles/thermistorptc/height}}{\ctikzvalof{bipoles/thermistorptc/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorptc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorptc/main}\pgf@circ@res@up}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
		\pgfusepath{draw}
		
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\tiny$\vartheta$}
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
		\pgfusepath{draw}
}

%% Thermistor NTC
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/thermistorntc/height 2}}{thermistorntc}{\ctikzvalof{bipoles/thermistorntc/height}}{\ctikzvalof{bipoles/thermistorntc/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorntc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorntc/main}\pgf@circ@res@up}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
		\pgfusepath{draw}
		
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\tiny$\vartheta$}
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
}

%% thermocouple
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/thermocouple/height 2}}{thermocouple}{\ctikzvalof{bipoles/thermocouple/height}}{\ctikzvalof{bipoles/thermocouple/width}}{
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
		\pgfusepath{draw}
}

%% Varistor
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/varistor/height}}{varistor}{\ctikzvalof{bipoles/varistor/height}}{\ctikzvalof{bipoles/varistor/width}}{
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/varistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/varistor/main}\pgf@circ@res@up}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw}
		
		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\pgftext[top,x=.65\pgf@circ@res@left,y=1.2\pgf@circ@res@down]{{\tiny\textsf{U}}}
}



%% Generic full tunable

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/tfullgeneric/height}}{tfullgeneric}{\ctikzvalof{bipoles/tfullgeneric/height}}{\ctikzvalof{bipoles/tfullgeneric/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfusepath{draw,fill}
		
		\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		\endpgfscope
}







%% Variable Capacitor

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vcapacitor/height}}{vcapacitor}{\ctikzvalof{bipoles/vcapacitor/height}}{\ctikzvalof{bipoles/vcapacitor/width}}{
		%\pgf@circ@res@step = \ctikzvalof{bipoles/vcapacitor/width}\pgf@circ@Rlen
		\pgf@circ@res@step = \ctikzvalof{bipoles/vcapacitor/capacitor width} \pgf@circ@res@right

		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfusepath{draw}
}


%% Piezoelectric Element

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/piezoelectric/height}}{piezoelectric}{\ctikzvalof{bipoles/piezoelectric/height}}{\ctikzvalof{bipoles/piezoelectric/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/piezoelectric/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 5

		%% Outer markings
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}

		%% Inner Box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left+4}{\pgf@circ@res@up-1}}{\pgfpoint{\pgf@circ@res@right-4}{\pgf@circ@res@down+1}}
		\pgfusepath{draw}

}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Handling of terminals


%% Easily usable styles

\ctikzset{o-o/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{-o/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{*-o/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-*/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-o/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-d/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{*-/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-*/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-d/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{*-*/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-*/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{*-d/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{d-d/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=diamond}}

\ctikzset{.-/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{.-*/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{.-o/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{.-d/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{-./.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{o-./.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{*-./.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{d-./.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{.-./.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}

\tikzset{reversed/.style = {\circuitikzbasekey/bipole/inverted=true}}


%% The output routine

\def\drawpoles{
	\pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/left}} \def\pgf@temp{diamond}  }
	\ifx\pgf@temp\pgf@circ@temp 
		 (\tikztostart) node[diamondpole] {} 
	\else 
		\pgfextra{ \def\pgf@temp{empty}  }
		\ifx\pgf@temp\pgf@circ@temp 
			 (\tikztostart) node[ocirc] {} 
		\else 
			\pgfextra{  \def\pgf@temp{full}  }
			\ifx\pgf@temp\pgf@circ@temp 
				(\tikztostart) node[circ] {} 
			\else 
				\pgfextra{ \def\pgf@temp{rectjoinfill} }
				\ifx\pgf@temp\pgf@circ@temp 
				 (\tikztostart) node[rectjoinfill] {} 
				\else 
				\fi
			\fi
		\fi
	\fi
	\pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/right}} \def\pgf@temp{diamond}  }
	\ifx\pgf@temp\pgf@circ@temp 
		 (\tikztotarget) node[diamondpole] {} 
	\else 
		\pgfextra{ \def\pgf@temp{empty}  }
		\ifx\pgf@temp\pgf@circ@temp 
			 (\tikztotarget) node[ocirc] {} 
		\else 
			\pgfextra{  \def\pgf@temp{full}  }
			\ifx\pgf@temp\pgf@circ@temp 
				(\tikztotarget) node[circ] {} 
			\else 
				\pgfextra{ \def\pgf@temp{rectjoinfill} }
				\ifx\pgf@temp\pgf@circ@temp 
				 (\tikztotarget) node[rectjoinfill] {} 
				\else 
				\fi
			\fi
		\fi
	\fi
}



%% Lamp

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/lamp/height}}{lamp}{\ctikzvalof{bipoles/lamp/height}}{\ctikzvalof{bipoles/lamp/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@down}}
	\pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@up}}
	\pgfusepath{draw}
}


\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/tline/height}
                        }{tline}{\ctikzvalof{bipoles/tline/height}
                                 }{\ctikzvalof{bipoles/tline/width}
                                   }    
          {
          \pgf@circ@res@step=.2\pgf@circ@res@right % half x axis
          \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
          \pgfpathellipse{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{0}}
                         {\pgfpoint{\pgf@circ@res@step}{0}}
                         {\pgfpoint{0}{-\pgf@circ@res@up}}
          \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@up}}
          \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@up}}
          \pgfpatharc{-90}{90}{-\pgf@circ@res@step and -\pgf@circ@res@up}
          \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@down}}
          \pgfusepath{draw}
}




%% SQUID added by Cor Molenaar 5 March 2010

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/squid/height}}{squid}{\ctikzvalof{bipoles/squid/height}}{\ctikzvalof{bipoles/squid/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@down}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@down}}

	\pgfusepath{draw}
}



% Generic barrier added by Cor Molenaar 5 March 2010

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/barrier/height}}{barrier}{\ctikzvalof{bipoles/barrier/height}}{\ctikzvalof{bipoles/barrier/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@step}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@step}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@down}}
	\pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@up}}

	\pgfusepath{draw}
}


% Contributed by Danilo Piazzalunga
 
\pgfdeclareshape{buffer}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/buffer/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/buffer/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{in}{
		\northwest
		\pgf@y=0pt
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfusepath{draw}
	\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	
		\pgfusepath{draw}
	  
	  }
	}





\pgfdeclareshape{plain amp}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }	  
	  \anchor{-}{
		\inOne
	  }
	  \anchor{+}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\up{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
	    \pgfpointlineattime{
			\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/up pos}}{
			\pgfpoint{
				\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
				{\pgf@circ@res@up}}
			{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	  }
	  \anchor{up}{
		\up
	  }
	  \anchor{down}{
		\up
		\pgf@y=-\pgf@y
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@up}}
	

	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@down}}
		
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	
	\pgfusepath{draw}

						
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfusepath{draw}
	\endpgfscope
		
		
	  
	  }
	}
	
%% Generic two port box
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/twoport/height}}{twoport}{\ctikzvalof{bipoles/twoport/height}}{\ctikzvalof{bipoles/twoport/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi
		
		% draw inner symbol
		\pgftext[center,x=0,y=0]{\ctikzvalof{bipoles/twoport/text}}
		
}

%% voltage controled oscillator
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vco/width}}{vco}{\ctikzvalof{bipoles/twoport/width}}{\ctikzvalof{bipoles/vco/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/vco/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		% draw circle
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@step}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi

		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi
		
		% draw inner sine waves
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{-.5\pgf@circ@res@step}{0\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		
}

%% bandpass filter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/bandpass/width}}{bandpass}{\ctikzvalof{bipoles/bandpass/width}}{\ctikzvalof{bipoles/bandpass/width}}{
		
		\pgf@circ@res@step = \ctikzvalof{bipoles/bandpass/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi
		
		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
		\pgfusepath{draw}
}

%% bandstop filter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/bandstop/width}}{bandstop}{\ctikzvalof{bipoles/bandstop/width}}{\ctikzvalof{bipoles/bandstop/width}}{
	\pgf@circ@res@step = \ctikzvalof{bipoles/bandstop/width}\pgf@circ@Rlen
	\divide \pgf@circ@res@step by 2

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgf@circ@res@other = \pgf@circ@res@left
	\advance\pgf@circ@res@other by \pgf@circ@res@step

	\ifpgf@circuit@dashed
	\pgfsetdash{{0.1cm}{0.1cm}}{0cm}
	\fi

	% draw outer box
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfusepath{draw}

	\ifpgf@circuit@inputarrow
	{
		\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
		\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
	}
	\fi

	% rotate inner symbol
	\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
	\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
	\pgftransformrotate{270}
	\fi\fi
	\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225% 134 degree, because >= 135 is not possible
	\pgftransformrotate{180}
	\fi\fi
	\ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
	\pgftransformrotate{90}
	\fi\fi

	% draw inner symbol
	\pgfsetdash{}{0pt}% always draw solid line for inner symbol
	\pgfsetarrows{-}%never draw arrows
	\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfusepath{draw}

	\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
	\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
	\pgfusepath{draw}

	\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
	\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
	\pgfusepath{draw}
}

%% highpass filter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/highpass/width}}{highpass}{\ctikzvalof{bipoles/highpass/width}}{\ctikzvalof{bipoles/highpass/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/highpass/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
		\pgfusepath{draw}
}

%% lowpass filter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/lowpass/width}}{lowpass}{\ctikzvalof{bipoles/lowpass/width}}{\ctikzvalof{bipoles/lowpass/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/lowpass/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
		\pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
		\pgfusepath{draw}
}

%% ADC
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/adc/width}}{adc}{\ctikzvalof{bipoles/adc/width}}{\ctikzvalof{bipoles/adc/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/adc/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\texti{A}
		\def\textii{D}
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\def\texti{D}
			\def\textii{A}
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\def\texti{D}
			\def\textii{A}
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
			\def\texti{A}
			\def\textii{D}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows				
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}
		
		\pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
		\pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DAC
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/dac/width}}{dac}{\ctikzvalof{bipoles/dac/width}}{\ctikzvalof{bipoles/dac/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/dac/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\texti{D}
		\def\textii{A}
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\def\texti{A}
			\def\textii{D}
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
			\def\texti{A}
			\def\textii{D}
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
			\def\texti{D}
			\def\textii{A}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows				
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfusepath{draw}
		
		\pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
		\pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DSP
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/dsp/width}}{dsp}{\ctikzvalof{bipoles/dsp/width}}{\ctikzvalof{bipoles/dsp/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/dsp/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgftext[center,x=0,y=0]{\textsf{DSP}}
}

%% FFT
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/fft/width}}{fft}{\ctikzvalof{bipoles/fft/width}}{\ctikzvalof{bipoles/fft/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/fft/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgftext[center,x=0,y=0]{\textsf{FFT}}
}

%% Amplifier
\pgfcircdeclarebipole{}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{amp}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@Rlen

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi		

		% draw outer box
		\ifpgf@circuit@boxed
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}	
			\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
		\fi
		
		% draw input arrow
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi

		\ifpgf@circuit@boxed
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
			\pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
		\else
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}	
		\fi
		
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
		\pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

		\pgfpathclose
		\pgfusepath{draw}
		
		% draw inner text
		\pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
}


%% variable amplifier
\pgfcircdeclarebipole{}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{vamp}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{
		\ifpgf@circuit@boxed
			\ctikzvalof{bipoles/twoport/width}
		\else
			\ctikzvalof{bipoles/amp/width}
		\fi
	}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@Rlen

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\ifpgf@circuit@boxed
			\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
		\fi

		% draw input arrow
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi

		\ifpgf@circuit@boxed
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
			\pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
		\else
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}	
		\fi
		

		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
		\pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

		\pgfpathclose
		\pgfusepath{draw}
		
		% draw inner text
		\pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
		
		% draw arrow
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfsetarrowsend{latex}
		\pgfpathmoveto{\pgfpoint{-0.8\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@step}{0.6\pgf@circ@res@step}}
		\pgfusepath{draw}
}

%% pi attenuator
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/piattenuator/width}}{piattenuator}{\ctikzvalof{bipoles/piattenuator/width}}{\ctikzvalof{bipoles/piattenuator/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/piattenuator/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% variable pi attenuator
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vpiattenuator/width}}{vpiattenuator}{\ctikzvalof{bipoles/vpiattenuator/width}}{\ctikzvalof{bipoles/vpiattenuator/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/vpiattenuator/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}

		\pgfsetarrowsend{latex}
		\pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% T attenuator
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/tattenuator/width}}{tattenuator}{\ctikzvalof{bipoles/tattenuator/width}}{\ctikzvalof{bipoles/tattenuator/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/tattenuator/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% variable T attenuator
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vtattenuator/width}}{vtattenuator}{\ctikzvalof{bipoles/vtattenuator/width}}{\ctikzvalof{bipoles/vtattenuator/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/vtattenuator/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 

		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi

		% draw inner symbol
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
		\pgfusepath{draw}
		
		\pgfsetarrowsend{latex}
		\pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% phase shifter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/phaseshifter/width}}{phaseshifter}{\ctikzvalof{bipoles/phaseshifter/width}}{\ctikzvalof{bipoles/phaseshifter/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/phaseshifter/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi
		
		% inner symbol
		\pgftext[center,x=0,y=0]{\Large$\varphi$}
}

%% variable phase shifter
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/phaseshifter/width}}{vphaseshifter}{\ctikzvalof{bipoles/vphaseshifter/width}}{\ctikzvalof{bipoles/vphaseshifter/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/vphaseshifter/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% rotate inner symbol
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
			\pgftransformrotate{270}
		\fi\fi
		\ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
			\pgftransformrotate{180}
		\fi\fi
		\ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
			\pgftransformrotate{90}
		\fi\fi
		
		% inner symbol
		\pgftext[center,x=0,y=0]{\Large$\varphi$}
		
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfsetarrowsend{latex}
		\pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.65\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.65\pgf@circ@res@up}}
		\pgfusepath{draw}
}

%% detector
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/detector/width}}{detector}{\ctikzvalof{bipoles/detector/width}}{\ctikzvalof{bipoles/detector/width}}{
		\pgf@circ@res@step = \ctikzvalof{bipoles/detector/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 2

		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgf@circ@res@other = \pgf@circ@res@left
		\advance\pgf@circ@res@other by \pgf@circ@res@step 
		
		\ifpgf@circuit@dashed
			\pgfsetdash{{0.1cm}{0.1cm}}{0cm} 
		\fi	
		
		% draw outer box
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@inputarrow
			{
				\advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
				\pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
			}
		\fi
		
		% draw inner stuff
		\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
		\pgfsetarrows{-} %never draw arrows
		\pgfsetlinewidth{0.8\pgfstartlinewidth}
		\pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0}}
		\pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0}}
		\pgfusepath{draw}
		
		\ifpgf@circuit@fulldiode
			\pgfmathparse{2\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/generic/width}}
			\pgftransformscale{\pgfmathresult}
			\pgfnode{fulldiodeshape}{center}{}{pgf@fulldiode}{\pgfusepath{fill}}
		\else
			\pgfmathparse{2\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/resistor/width}}
			\pgftransformscale{\pgfmathresult}
			\pgfnode{emptydiodeshape}{center}{}{pgf@emptydiode}{\pgfusepath{fill}}
		\fi
		
}




%% european gas filled surge arrester

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/european gas filled surge arrester/height}}{european gas filled surge arrester}{\ctikzvalof{bipoles/european gas filled surge arrester/height}}{\ctikzvalof{bipoles/european gas filled surge arrester/width}}{

		%\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		%\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw} 
		
		\pgfscope
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/european gas filled surge arrester/inside}\pgf@circ@res@left}{0pt}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}	
				\pgfusepath{draw} 
	
		\endpgfscope
}




%% american gas filled surge arrester

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/american gas filled surge arrester/height}}{american gas filled surge arrester}{\ctikzvalof{bipoles/american gas filled surge arrester/height}}{\ctikzvalof{bipoles/american gas filled surge arrester/width}}{
	%\def\pgf@circ@temp{right}
	%\ifx\tikz@res@label@pos\pgf@circ@temp
	%	\pgf@circ@res@step=-1.2\pgf@circ@res@up
	%\else
%		\def\pgf@circ@temp{below}
%		\ifx\tikz@res@label@pos\pgf@circ@temp
%			\pgf@circ@res@step=-1.2\pgf@circ@res@up
%		\else
%			\pgf@circ@res@step=1.2\pgf@circ@res@up
%		\fi
%	\fi

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}		
	\pgfpointorigin	\pgf@circ@res@other =  \pgf@x  \advance \pgf@circ@res@other by -\pgf@circ@res@up
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfusepath{draw}

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

		\pgfscope
			\pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
			\pgfusepath{draw}		
		\endpgfscope	

	\pgfsetlinewidth{\pgfstartlinewidth}


	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
	\pgfusepath{draw}

	\pgfnode{circle}{center}{}{}{}
	
	\pgfscope
		\pgfsetarrowsend{latex}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/inside}\pgf@circ@res@right}{\pgf@circ@res@zero}}
		\pgfusepath{draw}	
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/inside}\pgf@circ@res@left}{\pgf@circ@res@zero}}
		\pgfusepath{draw}	
	\endpgfscope{}
	
	%\pgftransformshift{\pgfpoint{.25\pgf@circ@res@left}{.45\pgf@circ@res@down}}
	%\pgfnode{circ}{center}{}{}{}
	%\pgftransformshift{}
	\pgfcircle{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/dot x}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/dot y}\pgf@circ@res@down}}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/size}\pgf@circ@res@down}
	\pgfusepath{fill}
}

% % MECHANICAL SYMBOLS

%% mechanical capacitance - stiffness/spring

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/spring/height}}{spring}{\ctikzvalof{bipoles/spring/height}}{\ctikzvalof{bipoles/spring/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments

	\pgfmathsetlength{\pgf@circ@res@step}
	{(\ctikzvalof{bipoles/spring/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth)/16}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
	\pgfsetcornersarced{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
	\pgf@circ@res@other = \pgf@circ@res@left
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step 
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}
}

%% mechanical inductance - mass
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/mass/box height}}{mass}{\ctikzvalof{bipoles/mass/height}}{\ctikzvalof{bipoles/mass/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments
	\pgfpathrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{-2\pgf@circ@res@down}{-2\pgf@circ@res@down}}

\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfsetrectcap
	\pgfsetmiterjoin
	\pgfusepath{stroke}
}

%% mechanical resistor - damper
\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/damper/height}}{damper}{\ctikzvalof{bipoles/damper/height}}{\ctikzvalof{bipoles/damper/width}}{
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
	\pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
					{\pgf@circ@res@zero}}
	\pgfusepath{stroke}

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}

	\pgfsetrectcap
	\pgfsetmiterjoin
	\pgfusepath{stroke}
	
	\pgfpathmoveto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
						{.8\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
						{.8\pgf@circ@res@up}}
	\pgfsetbuttcap
	\pgfusepath{stroke}
	
}




==> circuitikz/tex/pgfcirccurrent.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Current handling

%% Options
\ctikzset{i^>/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = forward,
		\circuitikzbasekey/bipole/current/x position = after,
		\circuitikzbasekey/bipole/current/y position = above
	}
}

\ctikzset{i_>/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = forward,
		\circuitikzbasekey/bipole/current/x position = after,
		\circuitikzbasekey/bipole/current/y position = below
	}
}

\ctikzset{i>^/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = forward,
		\circuitikzbasekey/bipole/current/x position = before,
		\circuitikzbasekey/bipole/current/y position = above
	}
}

\ctikzset{i>_/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = forward,
		\circuitikzbasekey/bipole/current/x position = before,
		\circuitikzbasekey/bipole/current/y position = below
	}
}

\ctikzset{i^</.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = backward,
		\circuitikzbasekey/bipole/current/x position = after,
		\circuitikzbasekey/bipole/current/y position = above
	}
}

\ctikzset{i_</.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = backward,
		\circuitikzbasekey/bipole/current/x position = after,
		\circuitikzbasekey/bipole/current/y position = below
	}
}

\ctikzset{i<^/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = backward,
		\circuitikzbasekey/bipole/current/x position = before,
		\circuitikzbasekey/bipole/current/y position = above
	}
}

\ctikzset{i<_/.style = {
		i = #1,
		\circuitikzbasekey/bipole/current/direction = backward,
		\circuitikzbasekey/bipole/current/x position = before,
		\circuitikzbasekey/bipole/current/y position = below
	}
}

\ctikzset{i/.code = {
	\pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
					\circuitikzbasekey/bipole/current/x position = after,
					\circuitikzbasekey/bipole/current/y position = above }
	\pgfkeys{/tikz/circuitikz/bipole/current/label/name=#1}
	\ctikzsetvalof{bipole/current/label/unit}{}
	\ifpgf@circ@siunitx 
		\pgf@circ@handleSI{#1}
		\ifpgf@circ@siunitx@res 
			\edef\pgf@temp{\pgf@circ@handleSI@val}
			\pgfkeyslet{/tikz/circuitikz/bipole/current/label/name}{\pgf@temp}
			\edef\pgf@temp{\pgf@circ@handleSI@unit}
			\pgfkeyslet{/tikz/circuitikz/bipole/current/label/unit}{\pgf@temp}
		\else
		\fi
	\else
	\fi
%reverse current direction for voltage sources
	\ifpgf@circ@oldvoltagedirection\else
		\ifpgf@circuit@bipole@isvoltage
		\ifpgf@circuit@bipole@voltage@backward
			\pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
					\circuitikzbasekey/bipole/current/x position = after,
					\circuitikzbasekey/bipole/current/y position = below }
		\else
			\pgfkeys{\circuitikzbasekey/bipole/current/direction = backward,
					\circuitikzbasekey/bipole/current/x position = before,
					\circuitikzbasekey/bipole/current/y position = above }
	\fi\fi\fi
}
}


\ifpgf@circ@oldvoltagedirection
	\ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward } }
\else
	\ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward, \circuitikzbasekey/bipole/current/x position = before } }
\fi
\ctikzset{i_/.style = { i = #1, \circuitikzbasekey/bipole/current/y position = below } }
\ctikzset{i>/.style = {i = #1, \circuitikzbasekey/bipole/current/direction = forward } }
\ctikzset{i^/.style = { i= #1, \circuitikzbasekey/bipole/current/y position = above } }

%% Output routine 
\def\pgf@circ@drawcurrent{
	\pgfextra{
		\edef\pgf@circ@ffffff{\pgf@circ@direction}
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

		\ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
			\ifpgf@circuit@bipole@current@below
				\def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
			\ifpgf@circuit@bipole@current@below
				\def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east} 
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
			\ifpgf@circuit@bipole@current@below
				 \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
			\ifpgf@circuit@bipole@current@below
				  \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
			\ifpgf@circuit@bipole@current@below
				 \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
			\ifpgf@circuit@bipole@current@below
				 \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
			\ifpgf@circuit@bipole@current@below
				  \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult <5
			\ifpgf@circuit@bipole@current@below
				 \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south} 
			\fi
		\fi
		\ifnum\pgfcircmathresult >355
			\ifpgf@circuit@bipole@current@below
				 \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south} 
			\fi
		\fi
		
		\ifpgf@circuit@bipole@current@below
			\def\pgf@circ@bipole@current@label@where{-90}
		\else
			\def\pgf@circ@bipole@current@label@where{+90}
		\fi
	}
	
	\pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
		\ifx\pgf@circ@temp\pgf@temp%draw current at a short at middle of the line
				(\tikztostart)--(\tikztotarget)
		\else% normal bipole or source
			\ifpgf@circuit@bipole@current@before
				 (\tikztostart)--(anchorstartnode)
			\else
				(anchorendnode)--(\tikztotarget)
			\fi
		\fi
		\ifpgf@circuit@bipole@current@backward
			\pgfextra{
				\pgfmathsubtract{\pgf@circ@ffffff}{180}
				\edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
				}
		\fi
	coordinate[currarrow,pos=\ctikzvalof{current/distance},rotate=\pgf@circ@ffffff](Iarrow)
	(Iarrow.\pgf@circ@bipole@current@label@where) node[anchor=\pgf@circ@dir]{\pgf@circ@finallabels{current/label}}
}

\endinput

==> circuitikz/tex/pgfcircflow.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% flow handling

%% Options
\ctikzset{f^>/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = forward,
		\circuitikzbasekey/bipole/flow/x position = after,
		\circuitikzbasekey/bipole/curflowrent/y position = above
	}
}

\ctikzset{f_>/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = forward,
		\circuitikzbasekey/bipole/flow/x position = after,
		\circuitikzbasekey/bipole/flow/y position = below
	}
}

\ctikzset{f>^/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = forward,
		\circuitikzbasekey/bipole/flow/x position = before,
		\circuitikzbasekey/bipole/flow/y position = above
	}
}

\ctikzset{f>_/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = forward,
		\circuitikzbasekey/bipole/flow/x position = before,
		\circuitikzbasekey/bipole/flow/y position = below
	}
}

\ctikzset{f^</.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = backward,
		\circuitikzbasekey/bipole/flow/x position = after,
		\circuitikzbasekey/bipole/flow/y position = above
	}
}

\ctikzset{f_</.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = backward,
		\circuitikzbasekey/bipole/flow/x position = after,
		\circuitikzbasekey/bipole/flow/y position = below
	}
}

\ctikzset{f<^/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = backward,
		\circuitikzbasekey/bipole/flow/x position = before,
		\circuitikzbasekey/bipole/flow/y position = above
	}
}

\ctikzset{f<_/.style = {
		f = #1,
		\circuitikzbasekey/bipole/flow/direction = backward,
		\circuitikzbasekey/bipole/flow/x position = before,
		\circuitikzbasekey/bipole/flow/y position = below
	}
}

\ctikzset{f</.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = backward} }
\ctikzset{f_/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = below } }
\ctikzset{f>/.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = forward } }
\ctikzset{f^/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = above } }

\ctikzset{f/.code = {
	\pgfkeys{\circuitikzbasekey/bipole/flow/direction = forward,
					\circuitikzbasekey/bipole/flow/x position = after,
					\circuitikzbasekey/bipole/flow/y position = above }
	\pgfkeys{/tikz/circuitikz/bipole/flow/label/name=#1}
	\ctikzsetvalof{bipole/flow/label/unit}{}
	\ifpgf@circ@siunitx 
		\pgf@circ@handleSI{#1}
		\ifpgf@circ@siunitx@res 
			\edef\pgf@temp{\pgf@circ@handleSI@val}
			\pgfkeyslet{/tikz/circuitikz/bipole/flow/label/name}{\pgf@temp}
			\edef\pgf@temp{\pgf@circ@handleSI@unit}
			\pgfkeyslet{/tikz/circuitikz/bipole/flow/label/unit}{\pgf@temp}
		\else
		\fi
	\else
	\fi
}
}

%% Output routine 
\def\pgf@circ@drawflow{
	\pgfextra{
		\edef\pgf@circ@ffffff{\pgf@circ@direction}
		\def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

		\ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
			\ifpgf@circuit@bipole@flow@below
				\def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
			\ifpgf@circuit@bipole@flow@below
				\def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east} 
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
			\ifpgf@circuit@bipole@flow@below
				 \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
			\ifpgf@circuit@bipole@flow@below
				  \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
			\ifpgf@circuit@bipole@flow@below
				 \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
			\ifpgf@circuit@bipole@flow@below
				 \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
			\ifpgf@circuit@bipole@flow@below
				  \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult <5
			\ifpgf@circuit@bipole@flow@below
				 \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south} 
			\fi
		\fi
		\ifnum\pgfcircmathresult >355
			\ifpgf@circuit@bipole@flow@below
				 \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south} 
			\fi
		\fi
		
		\ifpgf@circuit@bipole@flow@below
			\def\pgf@circ@bipole@flow@label@where{-90}
		\else
			\def\pgf@circ@bipole@flow@label@where{+90}
		\fi
	}
	
	\pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
		\ifx\pgf@circ@temp\pgf@temp%draw flow at a short at middle of the line
				(\tikztostart)--(\tikztotarget)
		\else% normal bipole or source
			\ifpgf@circuit@bipole@flow@before
				 (\tikztostart)--(anchorstartnode)
			\else
				(anchorendnode)--(\tikztotarget)
			\fi
		\fi
	\pgfextra{
		\ifpgf@circuit@bipole@flow@backward
			\ifpgf@circuit@bipole@flow@below
				\def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
			\else
				\def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
			\fi
			\pgfmathsubtract{\pgf@circ@ffffff}{180}
			\edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}	
		\else
			\ifpgf@circuit@bipole@flow@below
				\def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
			\else
				\def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
			\fi
		\fi
	}
	coordinate[flowarrow,pos=\ctikzvalof{flow/distance},rotate=\pgf@circ@ffffff,yshift=\flow@offset](Farrowpos)
	(Farrowpos.\pgf@circ@bipole@flow@label@where) node[anchor=\pgf@circ@dir]{ \pgf@circ@finallabels{flow/label}}
}

\endinput


==> circuitikz/tex/pgfcirclabel.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Bipole label positioning

%% Options
\ctikzset{label/.style = { l=#1 } }
\ctikzset{l/.code = { 
	\pgfkeys{/tikz/circuitikz/bipole/label/name=#1}
	\ctikzsetvalof{bipole/label/unit}{}
	\ifpgf@circ@siunitx 
		\pgf@circ@handleSI{#1}
		\ifpgf@circ@siunitx@res 
			\edef\pgf@temp{\pgf@circ@handleSI@val}
			\pgfkeyslet{/tikz/circuitikz/bipole/label/name}{\pgf@temp}
			\edef\pgf@temp{\pgf@circ@handleSI@unit}
			\pgfkeyslet{/tikz/circuitikz/bipole/label/unit}{\pgf@temp}
		\else
		\fi
	\else
	\fi
}}

\ctikzset{label above/.code = { 
		l=#1, 
		\circuitikzbasekey/bipole/label/position=90 }
}

\ctikzset{l^/.style = { 
		l=#1,
		\circuitikzbasekey/bipole/label/position=90 } 
}

\ctikzset{label below/.code = { 
		l=#1,
		\circuitikzbasekey/bipole/label/position=-90 } 
}

\ctikzset{l_/.style = { 
		l=#1,
		\circuitikzbasekey/bipole/label/position=-90 } 
}

\ctikzset{annotation/.style = { a=#1 } }
\ctikzset{a/.code = {
		\pgfkeys{/tikz/circuitikz/bipole/annotation/name=#1}
		\ctikzsetvalof{bipole/annotation/unit}{}
		\ifpgf@circ@siunitx
		\pgf@circ@handleSI{#1}
		\ifpgf@circ@siunitx@res
		\edef\pgf@temp{\pgf@circ@handleSI@val}
		\pgfkeyslet{/tikz/circuitikz/bipole/annotation/name}{\pgf@temp}
		\edef\pgf@temp{\pgf@circ@handleSI@unit}
		\pgfkeyslet{/tikz/circuitikz/bipole/annotation/unit}{\pgf@temp}
		\else
		\fi
		\else
		\fi
	}}

\ctikzset{annotation above/.code = { 
	a=#1, 
	\circuitikzbasekey/bipole/annotation/position=90 }
}

\ctikzset{a^/.style = { 
	a=#1,
	\circuitikzbasekey/bipole/annotation/position=90 } 
}

\ctikzset{annotation below/.code = { 
	a=#1,
	\circuitikzbasekey/bipole/annotation/position=-90 } 
}
\ctikzset{a_/.style = { 
	a=#1,
	\circuitikzbasekey/bipole/annotation/position=-90 } 
}



\def\pgf@circ@drawlabels#1{
	\pgfextra{
		\pgfmathsubtract{\pgf@circ@direction}{90}
		\edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
		
		\edef\pgf@circ@temp{\ctikzvalof{bipole/#1/position}} 
		\ifnum \pgf@circ@temp < 0
			\pgfmathadd{\pgf@circ@labanc}{180}
			\edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
		\fi
		\ifpgf@circuit@bipole@inverted
			\pgfmathadd{\pgf@circ@temp}{180} %If shape is inverted, use opposite anchor
			\edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
		\fi
		
		\ifnum \ctikzvalof{mirror value} = -1
			\pgfmathadd{\pgf@circ@temp}{180} %If shape is mirrored, use opposite anchor
			\edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
		\fi
	}
		%Firstly, place a coodinate directly at the edge of the shape
		(\ctikzvalof{bipole/name}.\pgf@circ@temp) coordinate (labelcoor)
		%now decide, which labels should be drawn
		\pgfextra{
			\edef\pgf@temp{\ctikzvalof{label/align}}
			\def\pgf@circ@temp{straight}
		}
		\ifx\pgf@temp\pgf@circ@temp %straight
			\pgf@circ@drawreglabels{#1}
		\else
			\pgfextra{\def\pgf@circ@temp{rotate}}
			\ifx\pgf@temp\pgf@circ@temp %rotate
				\pgf@circ@drawrotlabels{#1}
			\else% smart
				\pgf@circ@drawsmartlabels{#1}
			\fi
		\fi
}


\def\pgf@circ@drawsmartlabels#1{
	\pgfextra{
		\pgfmathmod{\pgf@circ@direction}{90}
		\edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
	}
	\ifnum \pgfcircmathresult > 20	
		\ifnum \pgfcircmathresult < 70
			\pgf@circ@drawrotlabels{#1}
		\else
			\pgf@circ@drawreglabels{#1}
		\fi
	\else
		\pgf@circ@drawreglabels{#1}
	\fi
}


\def\pgf@circ@drawrotlabels#1{
	\pgfextra{
		\ifnum \ctikzvalof{bipole/#1/position}>0
		%we need some more space for placement below, due to mid-anchor
			\def\pgf@circ@labposdistance{1.5ex}
			\else
			\def\pgf@circ@labposdistance{2ex}
		\fi
		%Calculate rotation of the label from direction and strip decimals
		\edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		% rotate the label at second or third quadrant:
		\ifnum \pgfcirclabrot > 90 \ifnum \pgfcirclabrot < 270
			\pgfmathsubtract{\pgf@circ@direction}{180}
			\edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
			%invert the space relationships due to rotatet strings
			\ifnum \ctikzvalof{bipole/#1/position}>0
				\def\pgf@circ@labposdistance{2ex}
			\else
				\def\pgf@circ@labposdistance{1.5ex}
			\fi
		\fi\fi
		\pgfmathparse{\ctikzvalof{bipole/#1/position}>0?\pgf@circ@direction+90:\pgf@circ@direction-90}
		\edef\pgf@circ@labposangle{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
	}				
	(labelcoor)++(\pgf@circ@labposangle:\pgf@circ@labposdistance) coordinate(labelcoor)
	node[anchor=mid,rotate=\pgfcirclabrot](\ctikzvalof{bipole/name}#1){\pgf@circ@finallabels{#1}}
}

\def\pgf@circ@drawreglabels#1{

	%Now calculate all shape positions
	%Use mid-anchor at x-axis and base-anchor at y-axis, respectively.
	%All points between will be addressed by angled-anchors:
	\pgfextra{
		\pgfmathadd{\pgf@circ@labanc}{90}
		\edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
		\pgfmathparse{mod(\pgf@circ@temp,180)>135?mod(\pgf@circ@temp,180)-180:mod(\pgf@circ@temp,180)}
		\edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
	}
	%Values between -5 and 5 are at pos /neg x-axis, values around 90 are at both y-axis
	\ifnum \pgfcircmathresult > 84 \ifnum \pgfcircmathresult< 96
		\pgfextra{\edef\pgf@circ@labpos{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}}
		\ifnum \pgf@circ@labpos > 180
			\ifnum \ctikzvalof{bipole/#1/position} > 0
				\pgfextra{\def\pgf@circ@labanc{mid west}}
			\else
				\pgfextra{\def\pgf@circ@labanc{mid east}}
			\fi
		\else
			\ifnum \ctikzvalof{bipole/#1/position} > 0
				\pgfextra{\def\pgf@circ@labanc{mid east}}
			\else
				\pgfextra{\def\pgf@circ@labanc{mid west}}
			\fi
		\fi
	\fi\fi
	\ifnum \pgfcircmathresult <6
		\ifnum \ctikzvalof{bipole/#1/position} < 0
			%we need some more space for placement below, due to mid-anchor
			(labelcoor)++(-\pgf@circ@labanc:2ex) coordinate(labelcoor)
		\else
			(labelcoor)++(-\pgf@circ@labanc:1.5ex) coordinate(labelcoor)
		\fi
		\pgfextra{\def\pgf@circ@labanc{mid}}
	\fi
	 (labelcoor) node[anchor=\pgf@circ@labanc](\ctikzvalof{bipole/name}#1){\pgf@circ@finallabels{#1}}
}

\def\pgf@circ@finallabels#1{%
	\edef\pgf@temp{}%
	\edef\pgf@circ@temp{\ctikzvalof{bipole/#1/unit}}%
	\ifx\pgf@temp\pgf@circ@temp%
	\ctikzvalof{bipole/#1/name}%
	\else%
	$\SI{\ctikzvalof{bipole/#1/name}}{\ctikzvalof{bipole/#1/unit}}$%
	\fi%
}

\ctikzset{text/.style = { t=#1 } }
\ctikzset{t/.code = { 
	\ctikzsetvalof{bipoles/twoport/text}{#1}
}}
\endinput

==> circuitikz/tex/pgfcircmonopoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Monopoles

%% Ground symbol

\pgfdeclareshape{ground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			%\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfusepath{draw}
						
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfpathmoveto{\pgfpoint{-.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw}
		
			
			\pgfsetlinewidth{\pgfstartlinewidth}
	
		\endpgfscope
	}

}



\pgfdeclareshape{rground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfusepath{draw}
						
						
			\pgfsetlinewidth{\pgfstartlinewidth}
	
		\endpgfscope
	}
}

\pgfdeclareshape{tground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			%\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/monopoles/tground/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
			\pgfusepath{draw}
						
						
			\pgfsetlinewidth{\pgfstartlinewidth}
	
		\endpgfscope
	}
}

\pgfdeclareshape{sground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{0}{-1.8\pgf@circ@res@step}}
			\pgfpathclose
			\pgfusepath{draw}
						
						
			\pgfsetlinewidth{\pgfstartlinewidth}
	
		\endpgfscope
	}

}

% noiseless ground
\pgfdeclareshape{nground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			%\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfusepath{draw}
						
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfpathmoveto{\pgfpoint{-.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfusepath{draw}
			
			\pgfpathmoveto{\pgfpoint{1.3\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfpatharc{0}{180}{1.3\pgf@circ@res@step}
			\pgfusepath{draw}
					
			\pgfsetlinewidth{\pgfstartlinewidth}
		\endpgfscope
	}
}

% protective ground
\pgfdeclareshape{pground}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
			\pgfusepath{draw}

			\pgfstartlinewidth=\pgflinewidth
			%\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfpathcircle{\pgfpoint{0pt}{-\pgf@circ@res@step}} {1.2\pgf@circ@res@step}
			\pgfusepath{draw}
						
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfpathmoveto{\pgfpoint{-.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.8\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
			\pgfusepath{draw}
					
			\pgfsetlinewidth{\pgfstartlinewidth}
		\endpgfscope
	}
}

% chassis ground 
\pgfdeclareshape{cground}{ 
\anchor{center}{ 
    \pgfpointorigin 
} 
\behindforegroundpath{       
    \pgf@circ@res@step=\ctikzvalof{monopoles/chassis/width}\pgf@circ@Rlen 
 
    \pgfscope        
        \pgfpathmoveto{\pgfpointorigin} 
        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}} 
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{-1.5\pgf@circ@res@step}{-2\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-2\pgf@circ@res@step}}
        \pgfpathmoveto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-2\pgf@circ@res@step}}
        \pgfusepath{draw}                        
    \endpgfscope 
    } 
}

% Contributed by Leonardo Azzinnari
\pgfdeclareshape{tlinestub}{
	\anchor{center}{\pgfpointorigin}
	\behindforegroundpath{
		\pgfstartlinewidth=\pgflinewidth
		
		\pgf@circ@res@step=\ctikzvalof{bipoles/tline/width} \pgf@circ@Rlen
        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
        
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0pt}}
            \pgfusepath{draw}
         \pgfscope
            \pgfpathellipse{\pgfpoint{0.5\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0.125\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{1.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpatharc{90}{-90}{0.125\pgf@circ@res@step and 0.25\pgf@circ@res@step}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-0.25\pgf@circ@res@step}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfusepath{draw}
         \endpgfscope
      }
}
                            



\pgfdeclareshape{antenna}{
\anchor{center}{\pgfpointorigin}
	\savedanchor{\northeast}{
		\pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
		\pgf@x=5\pgf@circ@res@step%-0.5\pgflinewidth
		\pgf@y=6\pgf@circ@res@step
	}
	\anchor{text}{
		\northeast
		\pgf@x=\ctikzvalof{monopoles/antenna/label/xanchor}\pgf@x
		\pgf@y=\ctikzvalof{monopoles/antenna/label/yanchor}\pgf@y
	}
   \behindforegroundpath{
     \pgfstartlinewidth=\pgflinewidth
     \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
                           
        % \pgfpathmoveto{\pgfpointorigin}
        % \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
        % \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        %     \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
        
        \pgftransformxshift{ -4\pgf@circ@res@step }

        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             
         \pgfusepath{draw}
             
          \pgfscope   
          \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
             \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
             \pgfusepath{draw}
           \endpgfscope
                           \pgfsetlinewidth{\pgfstartlinewidth}
                        
                           }
     }


\pgfdeclareshape{txantenna}{
	\anchor{center}{\pgfpointorigin}
	\savedanchor{\northeast}{
		\pgf@circ@res@step=\ctikzvalof{monopoles/txantenna/width}\pgf@circ@Rlen
		\pgf@x=5\pgf@circ@res@step%-0.5\pgflinewidth
		\pgf@y=6\pgf@circ@res@step
	}
	\anchor{text}{
		\northeast
		\pgf@x=\ctikzvalof{monopoles/txantenna/label/xanchor}\pgf@x
		\pgf@y=\ctikzvalof{monopoles/txantenna/label/yanchor}\pgf@y
	}
       \behindforegroundpath{
       \pgfstartlinewidth=\pgflinewidth
       \pgf@circ@res@step=\ctikzvalof{monopoles/txantenna/width}\pgf@circ@Rlen
        
         \pgfpathmoveto{\pgfpointorigin}
         \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
         \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             
         \pgfusepath{draw}
             
          \pgfscope   
          \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
             \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
             \pgfusepath{draw}
           \endpgfscope
          \pgfpathmoveto{\pgfpoint{5.5\pgf@circ@res@step}{6\pgf@circ@res@step}}
%        \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
        \pgfpatharc{30}{-30}{2\pgf@circ@res@step}         \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{2.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{7\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{4\pgf@circ@res@step}
        \pgfusepath{draw}
        \pgfsetlinewidth{\pgfstartlinewidth}
        
        }
     }


\pgfdeclareshape{rxantenna}{
	\anchor{center}{\pgfpointorigin}
	\savedanchor{\northeast}{
		\pgf@circ@res@step=\ctikzvalof{monopoles/txantenna/width}\pgf@circ@Rlen
		\pgf@x=5\pgf@circ@res@step%-0.5\pgflinewidth
		\pgf@y=6\pgf@circ@res@step
	}
	\anchor{text}{
		\northeast
		\pgf@x=\ctikzvalof{monopoles/rxantenna/label/xanchor}\pgf@x
		\pgf@y=\ctikzvalof{monopoles/rxantenna/label/yanchor}\pgf@y
	}
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@res@step=\ctikzvalof{monopoles/rxantenna/width}\pgf@circ@Rlen
             
         \pgfpathmoveto{\pgfpointorigin}
         \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
         \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             
         \pgfusepath{draw}
             
          \pgfscope   
          \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
             \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
             \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
             \pgfusepath{draw}
           \endpgfscope
           
           \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{7\pgf@circ@res@step}}
%             \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
             \pgfpatharc{150}{210}{4\pgf@circ@res@step}              \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
             \pgfpatharc{150}{210}{3.5\pgf@circ@res@step}
             \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
             \pgfpatharc{150}{210}{3\pgf@circ@res@step}
             \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
             \pgfpatharc{150}{210}{2.5\pgf@circ@res@step}
             \pgfpathmoveto{\pgfpoint{8\pgf@circ@res@step}{6\pgf@circ@res@step}}
             \pgfpatharc{150}{210}{2\pgf@circ@res@step}
             \pgfusepath{draw}
             \pgfsetlinewidth{\pgfstartlinewidth}
             
             }
}

% Vcc
\pgfdeclareshape{vcc}{
\anchor{center}{\pgfpointorigin}
\anchor{text}{
	\pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
	\pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}                          
	\pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}                
	\pgf@x=0pt
	\pgf@y=2\pgf@circ@res@step
	\advance \pgf@y by 0.5\ht\pgfnodeparttextbox
	\pgf@x=-.5\wd\pgfnodeparttextbox
	}
\behindforegroundpath{                             
	\pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen           
	\pgfscope           
		\pgfpathmoveto{\pgfpointorigin}
		\pgfpathlineto{\pgfpoint{0pt}{1.5\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfstartlinewidth=\pgflinewidth
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0}{1.5\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
		\pgfusepath{draw}
																						
		\pgfsetlinewidth{\pgfstartlinewidth}

	\endpgfscope
}

}

% Vee
\pgfdeclareshape{vee}{
\anchor{center}{\pgfpointorigin}
\anchor{text}{
	\pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
	\pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}                        
	\pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}        
	\pgf@x=0pt
	\pgf@y=-2\pgf@circ@res@step
	\advance \pgf@y by -1.5\ht\pgfnodeparttextbox
	\pgf@x=-.5\wd\pgfnodeparttextbox
	}

\behindforegroundpath{                             
	\pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
	
	\pgfscope                           
		\pgfpathmoveto{\pgfpointorigin}
		\pgfpathlineto{\pgfpoint{0pt}{-1.5\pgf@circ@res@step}}
		\pgfusepath{draw}

		\pgfstartlinewidth=\pgflinewidth
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

		\pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0}{-1.5\pgf@circ@res@step}}
		\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
		\pgfusepath{draw}
		\pgfsetlinewidth{\pgfstartlinewidth}

	\endpgfscope
}

}


% match
\pgfdeclareshape{match}{
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{text}{
		\pgf@x=\ctikzvalof{monopoles/match/width}\pgf@circ@Rlen
		\pgf@x=1.5\pgf@x
		\advance \pgf@x by -.5\wd\pgfnodeparttextbox
		\pgf@y=-1.5\ht\pgfnodeparttextbox
	}
	\behindforegroundpath{		
		\pgf@circ@res@step=\ctikzvalof{monopoles/match/width}\pgf@circ@Rlen
		
		\pgfscope		
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0pt}}
			\pgfusepath{draw}

			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0}}
			\pgfusepath{fill}
									
			\pgfsetlinewidth{\pgfstartlinewidth}
	
		\endpgfscope
	}

}


\endinput


==> circuitikz/tex/pgfcircpath.tex <==

\def\pgf@circ@direction{0.0}

% Names
\ctikzset{name/.style = { n=#1 } } %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%@@@
\ctikzset{n/.code = { 
	\pgfkeys{/tikz/circuitikz/bipole/name=#1}
}}

% Reflect the node along
\ctikzset{mirrored/.is choice}
\ctikzset{mirror value/.initial=1}
\ctikzset{mirrored/true/.code = {\ctikzsetvalof{mirror value}{-1}} }
\ctikzset{mirrored/false/.code = {\ctikzsetvalof{mirror value}{1}} }
\ctikzset{mirror/.style = {/tikz/circuitikz/mirrored=true}}

% Invert node along path
\ctikzset{inverted/.is choice}
\ctikzset{invert value/.initial=1}
\ctikzset{inverted/true/.code = {\ctikzsetvalof{invert value}{-1}\pgf@circuit@bipole@invertedtrue}}
\ctikzset{inverted/false/.code = {\ctikzsetvalof{invert value}{1}\pgf@circuit@bipole@invertedfalse}}
\ctikzset{invert/.style = {/tikz/circuitikz/inverted=true}}
\newif\ifpgf@circuit@bipole@inverted
\ctikzset{bipole/inverted/.is if=pgf@circuit@bipole@inverted}


\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}



% Initialize paths
\def\pgfcircresetpath{
	\ctikzset{bipole/name=, bipole/label/name=, bipole/label/position=90, ,bipole/annotation/name=, bipole/annotation/position=-90, 
		bipole/inverted=false, bipole/kind=,
	  	bipole/voltage/direction=backward, bipole/voltage/label/name=, bipole/voltage/position=below,
	  	bipole/nodes/left=none, bipole/nodes/right=none, bipole/is voltage=false,bipole/is voltageoutsideofsymbol=false,bipole/is strokedsymbol=false,
		bipole/is current=false, bipole/current/label/name=, bipole/current/x position=after,
		bipole/current/y position=above, bipole/current/direction=forward, 
		mirrored=false
   }
}

%% Helper function for path-function to ensure using anchors between nodes
\def\set@explicit@center@anchor#1{
	\pgfutil@ifundefined{pgf@sh@ns@#1}
	{
	%This coordinate is no node(but a relative position or a coordinate), no further handling needed
	}{
	\pgfutil@in@.{#1}
	\ifpgfutil@in@
	% Anchor is used, do nothing!
	\else%
		\let\tikz@moveto@waiting=\relax
		\pgfpathmoveto{\tikz@last@position}%force movement, because tikz@moveto@waiting
		\edef#1{#1.center}%ensure using center anchor
	\fi
	}
}


%% Generic bipole path
\def\pgf@circ@bipole@path#1#2{

\pgfextra{
		\set@explicit@center@anchor{\tikztostart}
		\set@explicit@center@anchor{\tikztotarget}
		\pgfsyssoftpath@getcurrentpath{\myp@th}%% save current path to extend after calculation of correct start/end coordinates
		\ctikzset{bipole/kind = #1}
		\edef\pgf@temp{\ctikzvalof{bipole/name}}
		\def\pgf@circ@temp{}
		\ifx\pgf@temp\pgf@circ@temp % if it has not a name
			\pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
			\ctikzset{bipole/name = #2\pgf@circ@rand} % create it
		\fi
	}
	
		(\tikztostart) coordinate (\ctikzvalof{bipole/name}start)%necessary to get correct coordinates in the case of relativ start/end or constructions like ((node1)-|(node2))
		(\tikztotarget) coordinate (\ctikzvalof{bipole/name}end)
		\pgfextra{
			\pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
							{\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
			\edef\pgf@circ@direction{\pgfmathresult}%Calculate direction(angle) of path
			\pgfsyssoftpath@setcurrentpath{\myp@th}		
		}
	\pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
	\ifx\pgf@temp\pgf@circ@temp  % if it is an open
	\else
		--($(\ctikzvalof{bipole/name}start) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}end)$) %ugly workaround to get correct linejoins(node breaks path?)
	\fi
		($(\tikztostart) ! .5 ! (\tikztotarget)$)%%positio of middle node 
		node[#1shape, rotate=\pgf@circ@direction, yscale=\ctikzvalof{mirror value}, xscale=\ctikzvalof{invert value}] 
			(\ctikzvalof{bipole/name}) {}
			\ifpgf@circuit@bipole@inverted
				\ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
					coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathend)
					coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathstart)
				\else
					coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.right)
					coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.left)
				\fi
			\else
				\ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
					coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathstart)
					coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathend)
				\else
					coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.left)
					coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.right)
				\fi
			\fi
	\pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
	\ifx\pgf@temp\pgf@circ@temp  % if it is an open
	\else
		\ifpgf@circuit@bipole@strokedsymbol%draw line thrue symbol(e.g. diodes)
			\ifcsname pgf@anchor@#1shape@strokepathstart\endcsname%if special path-anchors are defined, use them!
				(\ctikzvalof{bipole/name}start.center) -- (\ctikzvalof{bipole/name}.strokepathstart)
				(\ctikzvalof{bipole/name}.strokepathend)  -- (\ctikzvalof{bipole/name}end.center)
			\else
				(\ctikzvalof{bipole/name}start.center) -- (\ctikzvalof{bipole/name}end.center)
			\fi
		\else		
			(\ctikzvalof{bipole/name}start.center) -- (anchorstartnode)
			(anchorendnode)  -- (\ctikzvalof{bipole/name}end.center)
		\fi
	\fi
	
	\drawpoles
	\pgf@circ@ifkeyempty{bipole/label/name}\else\pgf@circ@drawlabels{label}\fi
	\pgf@circ@ifkeyempty{bipole/annotation/name}\else\pgf@circ@drawlabels{annotation}\fi
	\pgf@circ@ifkeyempty{bipole/voltage/label/name}\else\pgf@circ@drawvoltage\fi
	\pgf@circ@ifkeyempty{bipole/current/label/name}\else\pgf@circ@drawcurrent\fi
	\pgf@circ@ifkeyempty{bipole/flow/label/name}\else\pgf@circ@drawflow\fi
	\pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
	\ifx\pgf@temp\pgf@circ@temp  % if it is an open
		(\ctikzvalof{bipole/name}end)%Move to end of path
	\else
		($(\ctikzvalof{bipole/name}end) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}start)$) -- (\ctikzvalof{bipole/name}end)%ugly workaround to get correct linejoins(node breaks path?)
		%tikztostart and tikztotarget could not be used, because it would break if target coordinate is something like (node1-|node2)
		
	\fi
	% reset
	\pgfextra{
		\pgfcircresetpath
	}  
	\tikztonodes%draw pending nodes an path
}


%% Path definitions
\def\pgf@circ@resistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{generic}{#1}\else\pgf@circ@bipole@path{resistor}{#1}\fi}
\def\pgf@circ@vresistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{tgeneric}{#1}\else\pgf@circ@bipole@path{vresistor}{#1}\fi}
\def\pgf@circ@potentiometer@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{genericpotentiometer}{#1}\else\pgf@circ@bipole@path{potentiometer}{#1}\fi}
\def\pgf@circ@thermistor@path#1{\pgf@circ@bipole@path{thermistor}{#1}}
\def\pgf@circ@thermistorptc@path#1{\pgf@circ@bipole@path{thermistorptc}{#1}}
\def\pgf@circ@thermistorntc@path#1{\pgf@circ@bipole@path{thermistorntc}{#1}}
\def\pgf@circ@varistor@path#1{\pgf@circ@bipole@path{varistor}{#1}}
\def\pgf@circ@capacitor@path#1{\pgf@circ@bipole@path{capacitor}{#1}}
\def\pgf@circ@ecapacitor@path#1{\pgf@circ@bipole@path{ecapacitor}{#1}}
\def\pgf@circ@polarcapacitor@path#1{\pgf@circ@bipole@path{polarcapacitor}{#1}}
\def\pgf@circ@vcapacitor@path#1{\pgf@circ@bipole@path{vcapacitor}{#1}}
\def\pgf@circ@piezoelectric@path#1{\pgf@circ@bipole@path{piezoelectric}{#1}}
\def\pgf@circ@battery@path#1{\pgf@circ@bipole@path{battery}{#1}}
\def\pgf@circ@batteryone@path#1{\pgf@circ@bipole@path{battery1}{#1}}
\def\pgf@circ@batterytwo@path#1{\pgf@circ@bipole@path{battery2}{#1}}
\def\pgf@circ@europeaninductor@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@americaninductor@path#1{\pgf@circ@bipole@path{americaninductor}{#1}}
\def\pgf@circ@cuteinductor@path#1{\pgf@circ@bipole@path{cuteinductor}{#1}}
\def\pgf@circ@inductor@path#1{%
	\pgfextra{
		\edef\pgf@circ@temp{\ctikzvalof{inductor}}%
		\def\pgf@temp{european}%
	}
	\ifx\pgf@temp\pgf@circ@temp%
		\pgf@circ@europeaninductor@path{#1}%
	\else%
		\pgfextra{	\def\pgf@temp{cute} }%
		\ifx\pgf@temp\pgf@circ@temp%
			\pgf@circ@cuteinductor@path{#1}%
		\else%
			\pgf@circ@americaninductor@path{#1}%
		\fi%
	\fi%
}
\def\pgf@circ@vinductor@path#1{
	\pgfextra{
		\edef\pgf@circ@temp{\ctikzvalof{inductor}}%
		\def\pgf@temp{european}%
	}
	\ifx\pgf@temp\pgf@circ@temp%
		\pgf@circ@veuropeaninductor@path{#1}%
	\else%
		\pgfextra{	\def\pgf@temp{cute} }%
		\ifx\pgf@temp\pgf@circ@temp%
			\pgf@circ@vcuteinductor@path{#1}%
		\else%
			\pgf@circ@vamericaninductor@path{#1}%
		\fi%
	\fi%
}
\def\pgf@circ@veuropeaninductor@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@vamericaninductor@path#1{\pgf@circ@bipole@path{vamericaninductor}{#1}}
\def\pgf@circ@vcuteinductor@path#1{\pgf@circ@bipole@path{vcuteinductor}{#1}}
\def\pgf@circ@lamp@path#1{\pgf@circ@bipole@path{lamp}{#1}}
\def\pgf@circ@esource@path#1{\pgf@circ@bipole@path{esource}{#1}}
\def\pgf@circ@pvsource@path#1{\pgf@circ@bipole@path{pvsource}{#1}}
\def\pgf@circ@vsource@path#1{\pgf@circ@bipole@path{vsource}{#1}}
\def\pgf@circ@dcvsource@path#1{\pgf@circ@bipole@path{dcvsource}{#1}}
\def\pgf@circ@vsourceam@path#1{\pgf@circ@bipole@path{vsourceAM}{#1}}
\def\pgf@circ@vsourcesin@path#1{\pgf@circ@bipole@path{vsourcesin}{#1}}
\def\pgf@circ@isource@path#1{\pgf@circ@bipole@path{isource}{#1}}
\def\pgf@circ@oosource@path#1{\pgf@circ@bipole@path{oosource}{#1}}
\def\pgf@circ@dcisource@path#1{\pgf@circ@bipole@path{dcisource}{#1}}
\def\pgf@circ@isourcesin@path#1{\pgf@circ@bipole@path{isourcesin}{#1}}
\def\pgf@circ@vsourcesquare@path#1{\pgf@circ@bipole@path{vsourcesquare}{#1}}
\def\pgf@circ@vsourcetri@path#1{\pgf@circ@bipole@path{vsourcetri}{#1}}
\def\pgf@circ@isourceam@path#1{\pgf@circ@bipole@path{isourceAM}{#1}}
\def\pgf@circ@cvsource@path#1{\pgf@circ@bipole@path{cvsource}{#1}}
\def\pgf@circ@cvsourceam@path#1{\pgf@circ@bipole@path{cvsourceAM}{#1}}
\def\pgf@circ@cvsourcesin@path#1{\pgf@circ@bipole@path{cvsourcesin}{#1}}
\def\pgf@circ@cisource@path#1{\pgf@circ@bipole@path{cisource}{#1}}
\def\pgf@circ@cisourceam@path#1{\pgf@circ@bipole@path{cisourceAM}{#1}}
\def\pgf@circ@cisourcesin@path#1{\pgf@circ@bipole@path{cisourcesin}{#1}}
\def\pgf@circ@short@path#1{\pgf@circ@bipole@path{short}{#1}}
\def\pgf@circ@cspst@path#1{\pgf@circ@bipole@path{cspst}{#1}}
\def\pgf@circ@ospst@path#1{\pgf@circ@bipole@path{ospst}{#1}}
\def\pgf@circ@nos@path#1{\pgf@circ@bipole@path{nos}{#1}}
\def\pgf@circ@ncs@path#1{\pgf@circ@bipole@path{ncs}{#1}}
\def\pgf@circ@pushbutton@path#1{\pgf@circ@bipole@path{pushbutton}{#1}}
\def\pgf@circ@open@path#1{\pgf@circ@bipole@path{open}{#1}}
\def\pgf@circ@generic@path#1{\pgf@circ@bipole@path{generic}{#1}}
\def\pgf@circ@ageneric@path#1{\pgf@circ@bipole@path{ageneric}{#1}}
\def\pgf@circ@tgeneric@path#1{\pgf@circ@bipole@path{tgeneric}{#1}}
\def\pgf@circ@fullgeneric@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@tfullgeneric@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@ammeter@path#1{\pgf@circ@bipole@path{ammeter}{#1}}
\def\pgf@circ@ohmmeter@path#1{\pgf@circ@bipole@path{ohmmeter}{#1}}
\def\pgf@circ@voltmeter@path#1{\pgf@circ@bipole@path{voltmeter}{#1}}
\def\pgf@circ@empty@path#1{}
\def\pgf@circ@photoresistor@path#1{\pgf@circ@bipole@path{photoresistor}{#1}}
\def\pgf@circ@emptythyristor@path#1{\pgf@circ@bipole@path{emptythyristor}{#1}}
\def\pgf@circ@fullthyristor@path#1{\pgf@circ@bipole@path{fullthyristor}{#1}}
\def\pgf@circ@toggleswitch@path#1{\pgf@circ@bipole@path{toggleswitch}{#1}}
\def\pgf@circ@memristor@path#1{\pgf@circ@bipole@path{memristor}{#1}}
\def\pgf@circ@emptytriac@path#1{\pgf@circ@bipole@path{emptytriac}{#1}}
\def\pgf@circ@fulltriac@path#1{\pgf@circ@bipole@path{fulltriac}{#1}}
\def\pgf@circ@tline@path#1{\pgf@circ@bipole@path{tline}{#1}}
\def\pgf@circ@squid@path#1{\pgf@circ@bipole@path{squid}{#1}}
\def\pgf@circ@barrier@path#1{\pgf@circ@bipole@path{barrier}{#1}}
\def\pgf@circ@thermocouple@path#1{\pgf@circ@bipole@path{thermocouple}{#1}}
\def\pgf@circ@fuse@path#1{\pgf@circ@bipole@path{fuse}{#1}}
\def\pgf@circ@afuse@path#1{\pgf@circ@bipole@path{afuse}{#1}}

\def\pgf@circ@gfsurgearrester@path#1{\ifpgf@circuit@europeangfsurgearrester\pgf@circ@europeangfsurgearrester@path{#1}\else\pgf@circ@americangfsurgearrester@path{#1}\fi}
\def\pgf@circ@europeangfsurgearrester@path#1{\pgf@circ@bipole@path{european gas filled surge arrester}{#1}}
\def\pgf@circ@americangfsurgearrester@path#1{\pgf@circ@bipole@path{american gas filled surge arrester}{#1}}

\def\pgf@circ@twoport@path#1{\pgf@circ@bipole@path{twoport}{#1}}
\def\pgf@circ@vco@path#1{\pgf@circ@bipole@path{vco}{#1}}
\def\pgf@circ@bandpass@path#1{\pgf@circ@bipole@path{bandpass}{#1}}
\def\pgf@circ@bandstop@path#1{\pgf@circ@bipole@path{bandstop}{#1}}
\def\pgf@circ@highpass@path#1{\pgf@circ@bipole@path{highpass}{#1}}
\def\pgf@circ@lowpass@path#1{\pgf@circ@bipole@path{lowpass}{#1}}
\def\pgf@circ@adc@path#1{\pgf@circ@bipole@path{adc}{#1}}
\def\pgf@circ@dac@path#1{\pgf@circ@bipole@path{dac}{#1}}
\def\pgf@circ@dsp@path#1{\pgf@circ@bipole@path{dsp}{#1}}
\def\pgf@circ@fft@path#1{\pgf@circ@bipole@path{fft}{#1}}
\def\pgf@circ@amp@path#1{\pgf@circ@bipole@path{amp}{#1}}
\def\pgf@circ@vamp@path#1{\pgf@circ@bipole@path{vamp}{#1}}
\def\pgf@circ@piattenuator@path#1{\pgf@circ@bipole@path{piattenuator}{#1}}
\def\pgf@circ@vpiattenuator@path#1{\pgf@circ@bipole@path{vpiattenuator}{#1}}
\def\pgf@circ@tattenuator@path#1{\pgf@circ@bipole@path{tattenuator}{#1}}
\def\pgf@circ@vtattenuator@path#1{\pgf@circ@bipole@path{vtattenuator}{#1}}
\def\pgf@circ@phaseshifter@path#1{\pgf@circ@bipole@path{phaseshifter}{#1}}
\def\pgf@circ@vphaseshifter@path#1{\pgf@circ@bipole@path{vphaseshifter}{#1}}
\def\pgf@circ@detector@path#1{\pgf@circ@bipole@path{detector}{#1}}

%%Mechanical
\def\pgf@circ@spring@path#1{\pgf@circ@bipole@path{spring}{#1}}
\def\pgf@circ@mass@path#1{\pgf@circ@bipole@path{mass}{#1}}
\def\pgf@circ@damper@path#1{\pgf@circ@bipole@path{damper}{#1}}




%% Styles

\def\comnpatname{\ifpgf@circuit@compat *\else\fi}
\def\compattikzset#1{\tikzset{\comnpatname#1}}

%\def\ctikzsetbipole#1#2{%
%	\tikzset{#1/.style= {to path=#2, \circuitikzbasekey, l=##1}}%
%}

\compattikzset{spring/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@spring@path, l=#1}}
\compattikzset{mass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mass@path, l=#1}}
\compattikzset{damper/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@damper@path, l=#1}}
\compattikzset{resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@resistor@path, l=#1}}
\compattikzset{american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{resistor}{#1}, l=#1}}
\compattikzset{european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{generic}{#1}, l=#1}}
\compattikzset{potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@potentiometer@path, l=#1}}
\compattikzset{varistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@varistor@path, l=#1}}
\compattikzset{photoresistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@photoresistor@path, l=#1}}
\compattikzset{thermistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistor@path, l=#1}}
\compattikzset{thermistor ptc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorptc@path, l=#1}}
\compattikzset{thermistor ntc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorntc@path, l=#1}}
\compattikzset{american potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{potentiometer}{#1}, l=#1}}
\compattikzset{european potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{genericpotentiometer}{#1}, l=#1}}
\compattikzset{variable resistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vresistor@path, l=#1}}
\compattikzset{variable american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{vresistor}{#1}, l=#1}}
\compattikzset{variable european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{tgeneric}{#1}, l=#1}}
\compattikzset{capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@capacitor@path, l=#1}}
\compattikzset{elko/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
\compattikzset{ecapacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
\compattikzset{polar capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@polarcapacitor@path, l=#1}}
\compattikzset{variable capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcapacitor@path, l=#1}}
\compattikzset{piezoelectric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piezoelectric@path, l=#1}}
\compattikzset{battery/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@battery@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batteryone@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery2/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batterytwo@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@inductor@path, l=#1}}
\compattikzset{gf surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americangfsurgearrester@path, l=#1}}
\compattikzset{european gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeangfsurgearrester@path, l=#1}}
\compattikzset{gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americaninductor@path, l=#1}}
\compattikzset{cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteinductor@path, l=#1}}
\compattikzset{european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeaninductor@path, l=#1}}
\compattikzset{variable inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vinductor@path, l=#1}}
\compattikzset{variable european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@veuropeaninductor@path, l=#1}}
\compattikzset{variable american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamericaninductor@path, l=#1}}
\compattikzset{variable cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcuteinductor@path, l=#1}}
\compattikzset{tline/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tline@path, l=#1}}
\compattikzset{transmission line/.style = {tline = #1}}
\compattikzset{TL/.style = {tline = #1}}
\compattikzset{european voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{european controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{square voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesquare@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{triangle voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcetri@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{controlled sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{controlled sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}

\compattikzset{voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi current source = #1, \circuitikzbasekey/bipole/is current=true}}
\compattikzset{controlled voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi controlled voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{controlled current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi controlled current source = #1, \circuitikzbasekey/bipole/is current=true}}


\compattikzset{generic/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@generic@path, l=#1}}
\compattikzset{ageneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ageneric@path, l=#1}}
\compattikzset{tgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tgeneric@path, l=#1}}
\compattikzset{fullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullgeneric@path, l=#1}}
\compattikzset{tfullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tfullgeneric@path, l=#1}}
\compattikzset{short/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@short@path}}
\compattikzset{open/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@open@path}}

\compattikzset{lamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lamp@path}}

\compattikzset{squid/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@squid@path}}
\compattikzset{barrier/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@barrier@path}}
\compattikzset{thermocouple/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermocouple@path}}
\compattikzset{fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fuse@path}}
\compattikzset{asymmetric fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@afuse@path}}

\compattikzset{twoport/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@twoport@path}}
\compattikzset{vco/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vco@path}}
\compattikzset{bandpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandpass@path}}
\compattikzset{bandstop/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandstop@path}}
\compattikzset{highpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@highpass@path}}
\compattikzset{lowpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lowpass@path}}
\compattikzset{adc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@adc@path}}
\compattikzset{dac/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dac@path}}
\compattikzset{dsp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dsp@path}}
\compattikzset{fft/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fft@path}}
\compattikzset{amp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@amp@path}}
\compattikzset{vamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamp@path}}
\compattikzset{piattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piattenuator@path}}
\compattikzset{vpiattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vpiattenuator@path}}
\compattikzset{tattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tattenuator@path}}
\compattikzset{vtattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vtattenuator@path}}
\compattikzset{phaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@phaseshifter@path}}
\compattikzset{vphaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vphaseshifter@path}}
\compattikzset{detector/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@detector@path}}

% % % % % %
% % Beginn of Diodes
% % % % % %

\def\pgf@circ@fulldiode@path#1{\pgf@circ@bipole@path{fulldiode}{#1}}
\def\pgf@circ@fullzdiode@path#1{\pgf@circ@bipole@path{fullzdiode}{#1}}
\def\pgf@circ@fullzzdiode@path#1{\pgf@circ@bipole@path{fullzzdiode}{#1}}
\def\pgf@circ@fullsdiode@path#1{\pgf@circ@bipole@path{fullsdiode}{#1}}
\def\pgf@circ@fulltdiode@path#1{\pgf@circ@bipole@path{fulltdiode}{#1}}
\def\pgf@circ@fulllediode@path#1{\pgf@circ@bipole@path{fulllediode}{#1}}
\def\pgf@circ@fullpdiode@path#1{\pgf@circ@bipole@path{fullpdiode}{#1}}
\def\pgf@circ@fullvarcap@path#1{\pgf@circ@bipole@path{fullvarcap}{#1}}
\def\pgf@circ@emptydiode@path#1{\pgf@circ@bipole@path{emptydiode}{#1}}
\def\pgf@circ@emptyzdiode@path#1{\pgf@circ@bipole@path{emptyzdiode}{#1}}
\def\pgf@circ@emptyzzdiode@path#1{\pgf@circ@bipole@path{emptyzzdiode}{#1}}
\def\pgf@circ@emptysdiode@path#1{\pgf@circ@bipole@path{emptysdiode}{#1}}
\def\pgf@circ@emptytdiode@path#1{\pgf@circ@bipole@path{emptytdiode}{#1}}
\def\pgf@circ@emptylediode@path#1{\pgf@circ@bipole@path{emptylediode}{#1}}
\def\pgf@circ@emptypdiode@path#1{\pgf@circ@bipole@path{emptypdiode}{#1}}
\def\pgf@circ@emptyvarcap@path#1{\pgf@circ@bipole@path{emptyvarcap}{#1}}

\compattikzset{full diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulldiode@path}}
\compattikzset{full Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullsdiode@path}}
\compattikzset{full Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzdiode@path}}
\compattikzset{full ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzzdiode@path}}
\compattikzset{full tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltdiode@path}}
\compattikzset{full photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullpdiode@path}}
\compattikzset{full led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulllediode@path}}
\compattikzset{full varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullvarcap@path}}
\compattikzset{full thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullthyristor@path}}
\compattikzset{full triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltriac@path}}

\compattikzset{empty diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{empty Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{empty Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{empty ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{empty tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{empty photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{empty led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{empty varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{empty thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptythyristor@path}}
\compattikzset{empty triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytriac@path}}

\compattikzset{stroke diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{stroke Schottky diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{stroke Zener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{stroke ZZener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{stroke tunnel diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{stroke photodiode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{stroke led/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{stroke varcap/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{stroke thyristor/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptythyristor@path}}
%\compattikzset{stroke triac/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytriac@path}}

\def\pgfcircdiodestylemacro{\ifpgf@circuit@strokediode stroke \else\ifpgf@circuit@fulldiode full \else empty \fi\fi}

\compattikzset{Schottky diode/.style = {\comnpatname \pgfcircdiodestylemacro Schottky diode}}
\compattikzset{Zener diode/.style = {\comnpatname \pgfcircdiodestylemacro Zener diode}}
\compattikzset{ZZener diode/.style = {\comnpatname \pgfcircdiodestylemacro ZZener diode}}
\compattikzset{tunnel diode/.style = {\comnpatname \pgfcircdiodestylemacro tunnel diode}}
\compattikzset{photodiode/.style = {\comnpatname \pgfcircdiodestylemacro photodiode}}
\compattikzset{led/.style = {\comnpatname \pgfcircdiodestylemacro led}}
\compattikzset{varcap/.style = {\comnpatname \pgfcircdiodestylemacro varcap}}
\compattikzset{diode/.style = {\comnpatname \pgfcircdiodestylemacro diode}}
\compattikzset{thyristor/.style =  {\comnpatname \pgfcircdiodestylemacro thyristor}}
\compattikzset{triac/.style =  {\comnpatname \ifpgf@circuit@fulldiode full \else empty \fi triac}}%no stroke triac!

%% Define Shortcuts
\compattikzset{Do/.style = {\comnpatname empty diode}}
\compattikzset{tDo/.style = {\comnpatname empty tunnel diode}}
\compattikzset{zDo/.style = {\comnpatname empty Zener diode}}
\compattikzset{zzDo/.style = {\comnpatname empty ZZener diode}}
\compattikzset{sDo/.style = {\comnpatname empty Schottky diode}}
\compattikzset{pDo/.style = {\comnpatname empty photodiode}}
\compattikzset{leDo/.style = {\comnpatname empty led}}
\compattikzset{VCo/.style = {\comnpatname empty varcap}}
\compattikzset{Tyo/.style = {\comnpatname empty thyristor}}
\compattikzset{Tro/.style = {\comnpatname empty triac}}

\compattikzset{D*/.style = {\comnpatname full diode}}
\compattikzset{tD*/.style = {\comnpatname full tunnel diode}}
\compattikzset{zD*/.style = {\comnpatname full Zener diode}}
\compattikzset{zzD*/.style = {\comnpatname full ZZener diode}}
\compattikzset{sD*/.style = {\comnpatname full Schottky diode}}
\compattikzset{pD*/.style = {\comnpatname full photodiode}}
\compattikzset{leD*/.style = {\comnpatname full led}}
\compattikzset{VC*/.style = {\comnpatname full varcap}}
\compattikzset{Ty*/.style = {\comnpatname full thyristor}}
\compattikzset{Tr*/.style = {\comnpatname full triac}}

\compattikzset{D/.style = {\comnpatname diode}}
\compattikzset{tD/.style = {\comnpatname tunnel diode}}
\compattikzset{zD/.style = {\comnpatname Zener diode}}
\compattikzset{zzD/.style = {\comnpatname ZZener diode}}
\compattikzset{sD/.style = {\comnpatname Schottky diode}}
\compattikzset{pD/.style = {\comnpatname photodiode}}
\compattikzset{leD/.style = {\comnpatname led}}
\compattikzset{VC/.style = {\comnpatname varcap}}
\compattikzset{Ty/.style = {\comnpatname thyristor}}
\compattikzset{Tr/.style = {\comnpatname triac}}

\compattikzset{D-/.style = {\comnpatname stroke diode}}
\compattikzset{tD-/.style = {\comnpatname stroke tunnel diode}}
\compattikzset{zD-/.style = {\comnpatname stroke Zener diode}}
\compattikzset{zzD-/.style = {\comnpatname stroke ZZener diode}}
\compattikzset{sD-/.style = {\comnpatname stroke Schottky diode}}
\compattikzset{pD-/.style = {\comnpatname stroke photodiode}}
\compattikzset{leD-/.style = {\comnpatname stroke led}}
\compattikzset{VC-/.style = {\comnpatname stroke varcap}}
\compattikzset{Ty-/.style = {\comnpatname stroke thyristor}}
\compattikzset{Tr-/.style = {\comnpatname empty triac}}%no stroke triac!

% % % % % %
% % End of Diodes
% % % % % %


\compattikzset{memristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@memristor@path}}
\compattikzset{closing switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{opening switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ospst@path, l=#1}}
\compattikzset{ncs/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{nos/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{normal closed switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{normal open switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{toggle switch/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@toggleswitch@path}}

\compattikzset{ammeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ammeter@path}}
\compattikzset{voltmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@voltmeter@path}}
\compattikzset{ohmmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ohmmeter@path}}

% short forms
\compattikzset{esource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@esource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{pvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{dcvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{dcisource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcisource@path, \circuitikzbasekey/bipole/is current=true, l=#1}}

\compattikzset{ioosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is current=true,/tikz/to path=\pgf@circ@oosource@path, i=#1}}
\compattikzset{voosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is voltage=true,/tikz/to path=\pgf@circ@oosource@path, v=#1}}

\compattikzset{vsource/.style = {\comnpatname voltage source = #1}}
\compattikzset{isource/.style = {\comnpatname current source = #1}}
\compattikzset{cisource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{cvsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{vsourcesin/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{vsourcesquare/.style = {\comnpatname square voltage source = #1}}
\compattikzset{vsourcetri/.style = {triangle voltage source = #1}}
\compattikzset{isourcesin/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{cisourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}
\compattikzset{cvsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}

\compattikzset{controlled vsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{controlled isource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{controlled vsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}
\compattikzset{controlled isourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}

\compattikzset{R/.style= {\comnpatname resistor = #1}}
%\ifpgf@circuit@compat\else\compattikzset{R/.style= {resistor = #1}}\fi
\compattikzset{vR/.style= {\comnpatname variable resistor = #1}}
\compattikzset{phR/.style= {\comnpatname photoresistor = #1}}
\compattikzset{thR/.style= {\comnpatname thermistor = #1}}
\compattikzset{thRp/.style= {\comnpatname thermistor ptc= #1}}
\compattikzset{thRn/.style= {\comnpatname thermistor ntc= #1}}
\compattikzset{pR/.style= {\comnpatname potentiometer = #1}}
\compattikzset{C/.style = {\comnpatname capacitor = #1}}
\compattikzset{eC/.style = {\comnpatname ecapacitor = #1}}
\compattikzset{pC/.style = {\comnpatname polar capacitor = #1}}
\compattikzset{vC/.style = {\comnpatname variable capacitor = #1}}
\compattikzset{PZ/.style = {\comnpatname piezoelectric = #1}}
\compattikzset{L/.style = {\comnpatname inductor = #1}}
\compattikzset{vL/.style = {\comnpatname variable inductor = #1}}
\compattikzset{V/.style = {\comnpatname voltage source = #1}}
\compattikzset{cV/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{sV/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{sqV/.style = {\comnpatname square voltage source = #1}}
\compattikzset{tV/.style = {\comnpatname triangle voltage source = #1}}
\compattikzset{csV/.style = {\comnpatname controlled sinusoidal voltage source = #1}}
\def\pgf@temp#1{ 
	\compattikzset{V#1/.style = {\comnpatname voltage source, v#1=##1} } 
	\compattikzset{cV#1/.style = {\comnpatname controlled  voltage source, v#1=##1} } 
	\compattikzset{sV#1/.style = {\comnpatname sinusoidal  voltage source, v#1=##1} } 
	\compattikzset{csV#1/.style = {\comnpatname controlled sinusoidal voltage source, v#1=##1} } 
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<} 
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}

%current sources
\compattikzset{I/.style = {\comnpatname current source = #1}}
\compattikzset{cI/.style = {\comnpatname controlled current source = #1}}
\compattikzset{sI/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{csI/.style = {\comnpatname controlled sinusoidal current source = #1}}
\def\pgf@temp#1{ 
	\compattikzset{I#1/.style = {\comnpatname current source, i#1=##1} } 
	\compattikzset{cI#1/.style = {\comnpatname controlled current source, i#1=##1} } 
	\compattikzset{sI#1/.style = {\comnpatname sinusoidal current source, i#1=##1} } 
	\compattikzset{csI#1/.style = {\comnpatname controlled sinusoidal current source, i#1=##1} } 
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<}
\pgf@temp{>_} \pgf@temp{<_} \pgf@temp{>^} \pgf@temp{<^}
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}



\compattikzset{Mr/.style = {\comnpatname memristor}}

\compattikzset{cspst/.style = {\comnpatname closing switch = #1}}
\compattikzset{ospst/.style = {\comnpatname opening switch = #1}}
\compattikzset{spst/.style = {\comnpatname switch = #1}}

\compattikzset{afuse/.style = {\comnpatname asymmetric fuse=#1}}

\compattikzset{vdd/.style = {\comnpatname vcc = #1}}
\compattikzset{vss/.style = {\comnpatname vee = #1}}

\def\inheritlogicport#1#2{
	\pgfdeclareshape{#2 port}{
		\inheritsavedanchors[from=#1 #2 port]
		\inheritbackgroundpath[from=#1 #2 port]
		\inheritanchor[from=#1 #2 port]{in}
		\inheritanchor[from=#1 #2 port]{in 1}
		\inheritanchor[from=#1 #2 port]{in 2}
		\inheritanchor[from=#1 #2 port]{out}
		\inheritanchor[from=#1 #2 port]{center}
		\inheritanchor[from=#1 #2 port]{left}
	}
}

\ifpgf@circuit@europeanlogicport
	\inheritlogicport{european}{and}
	\inheritlogicport{european}{or}
	\inheritlogicport{european}{xor}
	\inheritlogicport{european}{not}
	\inheritlogicport{european}{nand}
	\inheritlogicport{european}{nor}
	\inheritlogicport{european}{xnor}
\else
	\inheritlogicport{american}{and}
	\inheritlogicport{american}{or}
	\inheritlogicport{american}{xor}
	\inheritlogicport{american}{not}
	\inheritlogicport{american}{nand}
	\inheritlogicport{american}{nor}
	\inheritlogicport{american}{xnor}
\fi

% Transistor like bipoles

\def\pgf@circ@trans@path#1#2{
	\pgfextra{
		\edef\pgf@temp{\pgfkeysvalueof{/tikz/circuitikz/bipole/name}}
		\def\pgf@circ@temp{#2}
		\ifx\pgf@temp\pgf@circ@temp % if it has not a name
			\pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
			\ctikzset{bipole/name = trans\pgf@circ@rand} % create it
		\fi
	}
	\ifpgf@circuit@bipole@inverted
		(\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}end) {}
		(\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}start) {} 	
	\else
		(\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}start) {}
		(\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}end) {} 
	\fi
	\pgfextra{
		\pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
					   {\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
		\pgfmathadd{\pgfmathresult}{-90}
		\edef\pgf@circ@direction{\pgfmathresult}
	}
	($(\tikztostart) ! .5 ! (\tikztotarget)$) 
		node[#1, /tikz/rotate=\pgf@circ@direction, xscale=\ctikzvalof{mirror value}]
			(\ctikzvalof{bipole/name}) {} node {\ctikzvalof{bipole/label/name}}
		\ifcsname pgf@anchor@#1@pathstart\endcsname%if special path-anchors are defined, use them!
			(\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.pathstart)
			(\ctikzvalof{bipole/name}.pathend)  -- (\ctikzvalof{bipole/name}end.center)
		\else
			(\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.left)
			(\ctikzvalof{bipole/name}.right)  -- (\ctikzvalof{bipole/name}end.center)
		\fi
	\pgfextra{
		\pgfcircresetpath
	}  
	(\tikztotarget) 	\tikztonodes  % e si continua
}


\def\pgf@circ@definetranspath#1{
	\compattikzset{T#1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@trans@path{#1}{}, l=##1}}
}

\pgf@circ@definetranspath{elmech}
\pgf@circ@definetranspath{nmos}
\pgf@circ@definetranspath{pmos}
\pgf@circ@definetranspath{npn}
\pgf@circ@definetranspath{pnp}
\pgf@circ@definetranspath{nfet}
\pgf@circ@definetranspath{nigfete}
\pgf@circ@definetranspath{nigfetd}
\pgf@circ@definetranspath{nigfetebulk}
\pgf@circ@definetranspath{pfet}
\pgf@circ@definetranspath{pigfete}
\pgf@circ@definetranspath{pigfetd}
\pgf@circ@definetranspath{pigfetebulk}
\pgf@circ@definetranspath{njfet}
\pgf@circ@definetranspath{pjfet}
\pgf@circ@definetranspath{pigbt}
\pgf@circ@definetranspath{nigbt}
\pgf@circ@definetranspath{Lpigbt}
\pgf@circ@definetranspath{Lnigbt}


==> circuitikz/tex/pgfcircquadpoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Quadripoles

\long\def\pgfcircdeclarequadpole#1#2#3{
	\pgfdeclareshape{#1}
	{
	  \anchor{center}{
	  	\northwest
		\pgf@x=0pt
	  }
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=.5\pgf@circ@Rlen
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/width}\pgf@x
	  }
	  \anchor{A2}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{B1}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{A1}{
		\northwest
	  }
	  \anchor{B2}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
	  	\northwest
		\pgf@x=0pt
	  }
	  \anchor{south}{
	  	\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{west}{
	  	\northwest
		\pgf@y=0pt
	  }
	  \anchor{east}{
	  	\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \anchor{base}{
	  	\northwest
		\pgf@x=0pt	  	
	  }
	  #3
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
			#2
	  
	  }
	}
}



\def\pgf@circ@drawtransformerbasicanchor{
	\pgfkeysvalueof{/tikz/circuitikz/quadpoles/trans/height}
	 \anchor{AA2}{
		\northwest
		\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
		\pgf@x=.7\pgf@x
		\pgf@y=-\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
	  }
	  \anchor{BB1}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
		\pgf@x=.7\pgf@x
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
	  }
	  \anchor{AA1}{
		\northwest
		\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
		\pgf@x=.7\pgf@x
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
	  }
	  \anchor{BB2}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
		\pgf@x=.7\pgf@x
		\pgf@y=-\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
	  }
}

\def\pgf@circ@drawtransformerbasicbody{
	\def\stretto{.4}
	\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgftransformlineattime{.5}{%
				\pgfpoint%
					{\stretto\pgf@circ@res@left}%
					{\pgf@circ@res@up}%
			}{%
				\pgfpoint
					{\stretto\pgf@circ@res@left}%
					{\pgf@circ@res@down}%
			}
			
			\edef\pgf@circ@temp{\ctikzvalof{inductor}}%
			\def\pgf@temp{european}%
			\ifx\pgf@temp\pgf@circ@temp%
				\pgfnode{fullgenericshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
			\else%
				\def\pgf@temp{cute}
				\ifx\pgf@temp\pgf@circ@temp%
					\pgfnode{cuteinductorshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
				\else%
					\pgfnode{americaninductorshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
				\fi%
			\fi%

			
	\endpgfscope
	\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgftransformlineattime{.5}{%
				\pgfpoint%
					{\stretto\pgf@circ@res@right}%
					{\pgf@circ@res@down}%
			}{%
				\pgfpoint
					{\stretto\pgf@circ@res@right}%
					{\pgf@circ@res@up}%
			}

			\edef\pgf@circ@temp{\ctikzvalof{inductor}}%
			\def\pgf@temp{european}%
			\ifx\pgf@temp\pgf@circ@temp%
				\pgfnode{fullgenericshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
			\else%
				\def\pgf@temp{cute} 
				\ifx\pgf@temp\pgf@circ@temp%
					\pgfnode{cuteinductorshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
				\else%
					\pgfnode{americaninductorshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
				\fi%
			\fi%
			
	\endpgfscope
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpointanchor{pgf@inductor1}{b}}
	
	\pgfpathmoveto{\pgfpointanchor{pgf@inductor1}{a}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpointanchor{pgf@inductor2}{a}}
	
	\pgfpathmoveto{\pgfpointanchor{pgf@inductor2}{b}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	
	\pgfusepath{draw}
	
}


	
	% contrib Kristofer M. Monisit
	
	\pgfdeclareshape{fd op amp}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{-}{
		\inOne
	  }
	  \anchor{+}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\up{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
			\pgf@circ@res@up = \pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
	    \pgfpointlineattime{
			\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/up pos}}{
			\pgfpoint{
				\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
				{\pgf@circ@res@up}}
			{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	  }
	  \anchor{up}{
		\up
	  }
	  \anchor{down}{
		\up
		\pgf@y=-\pgf@y
	  }
	  \anchor{out +}{
		\northwest
		\pgf@y=.5\pgf@y
		\pgf@x=-.7\pgf@x
	  }
	  \anchor{out -}{
		\northwest
		\pgf@y=-.5\pgf@y
		\pgf@x=-.7\pgf@x
	  }
	  \anchor{west}{
	  	\left
      }
		\anchor{east}{
			\left
			\pgf@x=-\pgf@x
		}

	  \backgroundpath{
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

      \northwest
      \pgf@circ@res@up = \pgf@y
      \pgf@circ@res@down = -\pgf@y
      \pgf@circ@res@right = -\pgf@x
      \pgf@circ@res@left = \pgf@x

      % Negative input terminal
      \pgfpathmoveto{\pgfpoint
        {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
      \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $-$}
  

      % Positive input terminal
      \pgfpathmoveto{\pgfpoint
        {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
      \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $+$}
  

      % Negative output terminal
      \pgfpathmoveto{\pgfpoint
        {0.7\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
      \pgftext[left, at=\pgfpoint{0.3\pgf@circ@res@left}{.3\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $-$}
  

      % Positive output terminal
      \pgfpathmoveto{\pgfpoint
        {0.7\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
      \pgftext[left, at=\pgfpoint{0.3\pgf@circ@res@left}{.3\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $+$}
  
	  \pgfsetrectcap
      % Draw them all!
      \pgfusepath{draw}

      % Triangle
      \pgfscope
        \pgfsetlinewidth{2\pgflinewidth}
        \pgftransformxshift{.7\pgf@circ@res@left}
        \pgf@circ@res@step=\pgf@circ@res@right
        \advance\pgf@circ@res@step by -\pgf@circ@res@left
        \pgf@circ@res@step=.7\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
        \pgfpathclose
        \pgfusepath{draw}
      \endpgfscope
	  }
	}




\pgfcircdeclarequadpole{transformer}{

	\pgf@circ@drawtransformerbasicbody

}{\pgf@circ@drawtransformerbasicanchor}

\pgfcircdeclarequadpole{transformer core}{

	\pgf@circ@drawtransformerbasicbody
	
	\pgfmoveto{\pgfpoint%
					{\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@right}%
					{\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
					}
	\pgflineto{
				\pgfpoint
					{\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@right}%
					{\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
					}

	\pgfmoveto{\pgfpoint%
					{\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@left}%
					{\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
					}
	\pgflineto{
				\pgfpoint
					{\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@left}%
					{\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
					}					
	
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth}
	\pgfusepath{draw}
}{\pgf@circ@drawtransformerbasicanchor}


\pgfcircdeclarequadpole{gyrator}{

	\def\stretto{.4}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@left}{.7*\stretto\pgf@circ@res@down}}
	\pgfpatharc{90}{270}{.7*\stretto\pgf@circ@res@down}
	
	\pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@right}{.7*\stretto\pgf@circ@res@up}}
	\pgfpatharc{-90}{90}{.7*\stretto\pgf@circ@res@down}
	\pgfusepath{draw}

}{}

%% four-port
% defines a general outer box for four-ports
% TikZ usage: 
%		\draw (0,0) node[coupler](coup){\SI{-3}{dB}}
%		(coup.port1) to[short,-o] ++(-1,0)
%

\long\def\pgfcircdeclarefourport#1#2{
	\pgfdeclareshape{#1}{
		\anchor{center}{
			\northwest
			\pgf@x=0pt
			\pgf@y=0pt
		}
		\savedanchor\northwest{%
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/height}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=.5\pgf@circ@Rlen
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/width}\pgf@x
			}
		\anchor{north}{
			\northwest
			\pgf@x=0pt
		}
		\anchor{south}{
			\northwest
			\pgf@x=0pt
			\pgf@y=-\pgf@y
		}
		\anchor{west}{
			\northwest
			\pgf@y=0pt
		}
		\anchor{east}{
			\northwest
			\pgf@y=0pt
			\pgf@x=-\pgf@x
		}
		\anchor{south west}{
			\northwest
			\pgf@y=-\pgf@y
		}
		\anchor{north east}{
			\northwest
			\pgf@x=-\pgf@x
		}
			\anchor{north west}{
			\northwest
		}
		\anchor{south east}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=-\pgf@y
		}
		\anchor{port1}{
			\northwest
			\pgf@y=-0.5\pgf@y
		}
		\anchor{port2}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=-0.5\pgf@y
		}
		\anchor{port3}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=0.5\pgf@y
		}
		\anchor{port4}{
			\northwest
			\pgf@y=0.5\pgf@y
		}
		\anchor{1}{
			\northwest
			\pgf@y=-0.5\pgf@y
		}
		\anchor{2}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=-0.5\pgf@y
		}
		\anchor{3}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=0.5\pgf@y
		}
		\anchor{4}{
			\northwest
			\pgf@y=0.5\pgf@y
		}
		
		\anchor{text}{
			\northwest
			\advance \pgf@y by 0.5\ht\pgfnodeparttextbox
			\pgf@x=-.5\wd\pgfnodeparttextbox
		}
		\backgroundpath{			
				\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
				\northwest
				\pgf@circ@res@up = \pgf@y 
				\pgf@circ@res@down = -\pgf@y
				\pgf@circ@res@right = -\pgf@x
				\pgf@circ@res@left = \pgf@x
			
				\pgfstartlinewidth=\pgflinewidth

				% draw outer box
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
				\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
				\pgfusepath{draw}
				
				% draw inner stuff
				#2
				
				% draw inner text
				\pgftext[center,x=-0.15\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
		}
	}
}

% four-port
\pgfcircdeclarefourport{fourport}{}


% straight coupler
\pgfcircdeclarefourport{coupler}{
	\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
	\pgfusepath{draw}
	
	\pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
	\pgfsetarrows{latex-latex}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
	\pgfsetarrows{latex-latex}
	\pgfusepath{draw}
}

% "bended" coupler
\pgfcircdeclarefourport{coupler2}{
	\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
	\pgfusepath{draw}
	
	\pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
	\pgfpatharc{0}{90} {0.4\pgf@circ@res@up}
	\pgfsetarrowsend{latex}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
	\pgfpatharc{0}{-90} {0.4\pgf@circ@res@up}
	\pgfsetarrowsend{latex}
	\pgfusepath{draw}
	
	\pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
	\pgfpatharc{180}{90} {0.4\pgf@circ@res@up}
	\pgfsetarrowsend{latex}
	\pgfusepath{draw}
	\pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
	\pgfpatharc{-180}{-90} {0.4\pgf@circ@res@up}
	\pgfsetarrowsend{latex}
	\pgfusepath{draw}
	
	
}


==> circuitikz/tex/pgfcircshapes.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Other shapes


%% Nothing

\pgfdeclareshape{emptyshape}{
	\savedanchor{\northeast}{%
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
   }
	\anchor{north}{
		\northeast
		\pgf@x=0cm
	}
	\anchor{east}{%
		\northeast
		\pgf@y=0cm
   }
	\anchor{south}{%
		\northeast
		\pgf@y=-\pgf@y
		\pgf@x=0cm
   }
	\anchor{west}{
		\northeast
		\pgf@y=0cm
		\pgf@x=-\pgf@x
	}
	\anchor{text}{%
		\pgfpointorigin
   }
	\anchor{center}{
		\pgfpointorigin
	}
}

%% Full terminal

\pgfdeclareshape{circ}{
	\anchor{center}{
		\pgfpointorigin
	}
	\anchorborder{
		\pgf@circ@res@left=\pgf@x
		\pgf@circ@res@up=\pgf@y
		\pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
}{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}}		
	}
	\behindforegroundpath{		
		
		\pgfscope
			\pgfpathcircle{\pgfpointorigin}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw,fill}		
		\endpgfscope

		}
}

%% Empty terminal

\pgfdeclareshape{ocirc}{
	\anchor{center}{
		\pgfpointorigin
	}
	\anchorborder{
		\pgf@circ@res@left=\pgf@x
		\pgf@circ@res@up=\pgf@y
		\pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
}{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}}		
	}

	\behindforegroundpath{		
		
		\pgfscope
			\pgfpathcircle{\pgfpointorigin}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfsetfillcolor{white}
			\pgfusepath{draw,fill}		
		\endpgfscope

		}
}

%% Diamond terminal

\pgfdeclareshape{diamondpole}{
	\anchor{center}{
		\pgfpointorigin
	}
	\anchorborder{
		\pgf@circ@res@left=\pgf@x
		\pgf@circ@res@up=\pgf@y
	}
	\behindforegroundpath{		
		\pgfscope
			\pgfmathsetlength{\pgf@circ@res@temp}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
			\pgftransformrotate{45}
			\pgfpathrectanglecorners
			{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@temp}{\pgf@circ@res@up+\pgf@circ@res@temp}}
			{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@temp}{\pgf@circ@res@up-\pgf@circ@res@temp}}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw,fill}		
		\endpgfscope
		}
}

%% Fill for correct rectangular joins

\pgfdeclareshape{rectjoinfill}{
	\anchor{center}{
		\pgfpointorigin
	}
	\anchorborder{
		\pgf@circ@res@left=\pgf@x
		\pgf@circ@res@up=\pgf@y
	}
	\behindforegroundpath{		
		\pgfscope
			\pgfpathrectanglecorners
			{\pgfpoint{0}{.5\pgflinewidth}}
			{\pgfpoint{0}{-.5\pgflinewidth}}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw,fill}		
		\endpgfscope
		}
}


%% Current arrow

\pgfdeclareshape{currarrow}{
	\anchor{center}{
		\pgfpointorigin
	}
		\anchor{tip}{
		\pgfpointorigin
			\pgf@circ@res@step = \pgf@circ@Rlen
				\divide \pgf@circ@res@step by 16
		\pgf@x	=\pgf@circ@res@step
		}
	\behindforegroundpath{		
		
		\pgfscope
			\pgf@circ@res@step = \pgf@circ@Rlen
			\divide \pgf@circ@res@step by 16

			\pgfpathmoveto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw,fill}

		\endpgfscope
	}

}

%% Flow arrow

\pgfdeclareshape{flowarrow}{
	\anchor{center}{
		\pgfpointorigin
	}
		\anchor{tip}{
		\pgfpointorigin
			\pgf@circ@res@step = \pgf@circ@Rlen
				\divide \pgf@circ@res@step by 16
		\pgf@x	=\pgf@circ@res@step
		}
	\behindforegroundpath{
		\pgfscope
			\pgf@circ@res@step = \pgf@circ@Rlen
			\divide \pgf@circ@res@step by 4
			\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{draw}
			\pgftransformshift{\pgfpoint{\pgf@circ@res@step}{0pt}}
			\pgfnode{currarrow}{tip}{}{}{\pgfusepath{fill}}
		\endpgfscope
	}
}

%% Input arrow

\pgfdeclareshape{inputarrow}{
	\savedanchor{\tip}{
		\pgfpointorigin
	}
	\anchor{center}{
		\tip
	}
	\anchor{tip}{
		\tip
	}
	\behindforegroundpath{		
		
		\pgfscope
			\pgf@circ@res@step = \pgf@circ@Rlen
			\divide \pgf@circ@res@step by 16

			\pgfpathmoveto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}
			\pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{0pt}{0pt}}
			\pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			\pgfusepath{fill}

		\endpgfscope
	}

}


%% box

\pgfdeclareshape{box}{
	\anchor{center}{
		\pgfpointorigin
	}
	\behindforegroundpath{		
		
		\pgfscope
			\pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@circ@res@step = 0.5\pgf@circ@res@step
			\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@step}}{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
			\pgfusepath{draw}
		\endpgfscope
	}

}

\endinput


==> circuitikz/tex/pgfcirctripoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tripoles



\pgfdeclareshape{spdt}
	{
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{left}{%
	  	\northwest
	  	\pgf@y=0pt
	  }
	  \anchor{in}{
	  	\northwest
	  	\pgf@y=0pt
	  }	  
	  \anchor{out 1}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{out 2}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }
  	  \anchor{center}{
		\pgf@y=0pt
		\pgf@x=0pt
	  }
	  \anchor{east}{
	  	\northwest
		\pgf@y=0pt
	  	\pgf@x=-\pgf@x  
	  }
	  \anchor{west}{
	  	\northwest
		\pgf@y=0pt
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x  
			\pgf@circ@res@left = \pgf@x  
			\pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/margin}\pgf@circ@res@left
			
		
	  	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	  	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}
		
		\pgfusepath{draw}
		
		\pgfscope
			\pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
			\pgfnode{ocirc}{center}{}{spdt1}{\pgfusepath{stroke}}
		\endpgfscope
		\pgfscope
			\pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
			\pgfnode{ocirc}{center}{}{}{\pgfusepath{stroke}}
		\endpgfscope
		\pgfscope
			\pgftransformshift{\pgfpoint{\pgf@circ@res@other}{0pt}}
			\pgfnode{ocirc}{center}{}{spdt2}{\pgfusepath{stroke}}
		\endpgfscope
		
		
		\pgfscope
			\pgfpathmoveto{\pgfpointshapeborder{spdt2}{\pgfpointorigin}}
			\pgfpathlineto{
				\pgfpointadd{\pgfpointshapeborder{spdt1}{\pgfpoint{-\pgf@circ@res@other}{-100pt}}}
				{\pgfpoint{-.05\pgf@circ@res@up}{-.05\pgf@circ@res@up}}
			}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
		\endpgfscope
	  }
	}
	
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%       Logic ports
%%






\long\def\pgfcircdeclarelogicport#1#2{
	\pgfdeclareshape{american #1 port}
	{
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }	  
	  \anchor{in 1}{
		\inOne
	  }
	  \anchor{in}{
		\inOne
	  }	  
	  \anchor{in 2}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
  	  \anchor{center}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-.8\pgf@x  
	  }
	  \anchor{east}{
	  	\left
	  	\pgf@x=-.8\pgf@x  
	  }
	  \anchor{west}{
	  	\left
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
			#2
	  
	  }
	}
}


\pgfcircdeclarelogicport{and}{
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@right}
		{0pt}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
		{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
		{\pgf@circ@res@down}}
	\pgfpathcurveto
		{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@right}
			{.5\pgf@circ@res@down}}
		{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@right}
			{0pt}}
	\pgfpathcurveto
		{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@right}
			{.5\pgf@circ@res@up}}
		{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
			{\pgf@circ@res@up}}	
	\pgfusepath{draw}
}



\pgfcircdeclarelogicport{nand}{
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right}
		{0pt}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{2\pgflinewidth}

	\pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/circle width}\pgf@circ@res@right
	\pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right
	
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
	\pgfpathcurveto
		{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
		{\pgfpoint{.0\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}
			{\pgf@circ@res@up}}	
	\pgfpathellipse
		{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{0pt}{.5\pgf@circ@res@step}}

	\pgfusepath{draw}
}


\pgfcircdeclarelogicport{nor}{
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}\pgf@circ@res@right}
		{0pt}}	
	
	\pgfusepath{draw}
	
	\pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}\pgf@circ@res@right
	\pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/circle width}\pgf@circ@res@right
		
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}	

	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}	
		
	\pgfpathellipse
		{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{0pt}{.5\pgf@circ@res@step}}
		
	\pgfusepath{draw}
}




\pgfcircdeclarelogicport{or}{

	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}\pgf@circ@res@right}
		{0pt}}	
	
	\pgfusepath{draw}
	\pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}\pgf@circ@res@right
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}	

	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}	
	\pgfusepath{draw}
}


\pgfcircdeclarelogicport{xor}{

	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}\pgf@circ@res@right}
		{0pt}}	
	
	\pgfusepath{draw}
	\pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}\pgf@circ@res@right
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}	

	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}	
		
	\def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/distance}\pgf@circ@res@right+}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}
	
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}	
				
	\pgfusepath{draw}
}



\pgfcircdeclarelogicport{xnor}{

	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input height}\pgf@circ@res@up}}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{(\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input skip})*\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/input height}\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}\pgf@circ@res@right}
		{0pt}}	
	
	\pgfusepath{draw}
	\pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}\pgf@circ@res@right
	\pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/circle width}\pgf@circ@res@right

	\pgfsetlinewidth{2\pgflinewidth}
	\pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/aaa}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}	

	\pgfpathcurveto
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@res@other-\pgf@circ@res@step}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ddd}\pgf@circ@res@left}{\pgf@circ@res@up}}
		{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}	
		
	\def\pgf@circ@temp{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/distance}\pgf@circ@res@right+}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{\pgf@circ@res@up}}
	
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@up}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@up}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{0pt}}
	\pgfpathcurveto
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/bbb}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/ccc}\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@temp\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/aaa}\pgf@circ@res@left}{.95*\pgf@circ@res@down}}
		{\pgfpoint{\pgf@circ@temp-\pgf@circ@res@other}{.95*\pgf@circ@res@down}}	
		
		
	\pgfpathellipse
		{\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{.5\pgf@circ@res@step}{0pt}}
		{\pgfpoint{0pt}{.5\pgf@circ@res@step}}
				
	\pgfusepath{draw}
}


\pgfdeclareshape{american not port}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{in}{
		\northwest
		\pgf@y=0pt
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  \anchor{center}{
	  	\pgfpointorigin
	  }
	  \anchor{east}{
	  	\left
	  	\pgf@x=-.8\pgf@x  
	  }
	  \anchor{west}{
	  	\left
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
		\pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right
						
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfusepath{draw}
		\pgfpathellipse
			{\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
			{\pgfpoint{.5\pgf@circ@res@other}{0pt}}
			{\pgfpoint{0pt}{.5\pgf@circ@res@other}}
		\pgfusepath{draw}
	\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	
		\pgfusepath{draw}
	  
	  }
	}

\pgfdeclareshape{invschmitt}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{in}{
		\northwest
		\pgf@y=0pt
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  \anchor{center}{
	  	\pgfpointorigin
	  }
	  \anchor{east}{
	  	\left
	  	\pgf@x=-.8\pgf@x  
	  }
	  \anchor{west}{
	  	\left
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
		\pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right
						
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathclose
		\pgfusepath{draw}
		\pgfpathellipse
			{\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
			{\pgfpoint{.5\pgf@circ@res@other}{0pt}}
			{\pgfpoint{0pt}{.5\pgf@circ@res@other}}
				\pgfsetfillcolor{white}
		\pgfusepath{draw,fill}
	\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
				\pgfusepath{draw}
		%draw inner shape
		
		\pgfsetlinewidth{2\pgflinewidth}
		
		\pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfusepath{draw}
	  
	  }
	}

\pgfdeclareshape{schmitt}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{in}{
		\northwest
		\pgf@y=0pt
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  \anchor{center}{
	  	\pgfpointorigin
	  }
	  \anchor{east}{
	  	\left
	  	\pgf@x=-.8\pgf@x  
	  }
	  \anchor{west}{
	  	\left
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
		\pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right
						
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathclose
		\pgfusepath{draw}
	\endpgfscope
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
		\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right-\pgf@circ@res@other}{0pt}}
				\pgfusepath{draw}
		%draw inner shape
		
		\pgfsetlinewidth{2\pgflinewidth}
		
		\pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
		\pgfusepath{draw}
	  
	  }
	}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% #1 - name
% #2 - text inside
% #3 - number of inputs
% #4 - is it a not

\long\def\pgfcircdeclareeurologicport#1#2#3#4{
	\pgfdeclareshape{european #1 port}
	{
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }	  
	  \anchor{in}{
		\inOne
	  }
	  \anchor{in 1}{
		\inOne
	  }
	  \anchor{in 2}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
  	  \anchor{center}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-.8\pgf@x  
	  }
	  \anchor{east}{
	  	\left
	  	\pgf@x=-.8\pgf@x  
	  }
	  \anchor{west}{
	  	\left
	  }
	  \anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  \anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	  }
	  \anchor{north west}{
		\northwest
	  }
	  \anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	  }	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			\def\pgf@temp{1}
			\def\pgf@circ@temp{#3}
			\ifx\pgftemp\pgf@circ@temp % one input
				\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfpathlineto{
					\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}{0pt}}
			\else % two inputs
				\pgfpathmoveto{
					\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/input height}\pgf@circ@res@up}}
				\pgfpathlineto{
					\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/input height}\pgf@circ@res@up}}
					%
				\pgfpathmoveto{
					\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/input height}\pgf@circ@res@down}}
				\pgfpathlineto{
					\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/input height}\pgf@circ@res@down}}
			\fi%
			%
			%
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
			\pgfpathlineto{
				\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{0pt}}
			%
			\edef\pgf@temp{not}
			\edef\pgf@circ@temp{#4}
			\ifx\pgf@temp\pgf@circ@temp % is a not
				\pgfpathmoveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/not width}\pgf@circ@res@right}{0pt}}
				\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/not height}\pgf@circ@res@up}}
			\fi
			%
			\pgfusepath{draw}
			%
			\pgfpathmoveto{\pgfpointorigin}
			\pgftext{#2}
			%
			%
			%
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfpathrectanglecorners
				{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}{\pgf@circ@res@up}}
				{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{\pgf@circ@res@down}}
			\pgfusepath{draw}
%
%
	  }
	}
}



\pgfcircdeclareeurologicport{and}{$\&$}{2}{}
\pgfcircdeclareeurologicport{or}{$\ge 1$}{2}{}
\pgfcircdeclareeurologicport{xor}{$=1$}{2}{}
\pgfcircdeclareeurologicport{not}{$1$}{1}{not}
\pgfcircdeclareeurologicport{nand}{$\&$}{2}{not}
\pgfcircdeclareeurologicport{nor}{$\ge 1$}{2}{not}
\pgfcircdeclareeurologicport{xnor}{$=1$}{2}{not}

\long\def\pgfcircdeclaretransistor#1#2#3{
	\pgfdeclareshape{#1}
	{
	\anchor{center}{
		 \pgfpointorigin
	 }
	\savedanchor\northeast{% upper right
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=0pt
	}
	\savedanchor\left{%center left
	  	\pgf@y=0pt
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/width}\pgf@circ@Rlen
	}
	\anchor{text}{
	 \northeast
	 \pgf@y=.7\pgf@y
	 \pgf@x= \pgf@circ@Rlen
	 \pgf@x=0.1\pgf@x
	}
	\anchor{pathstart}{ % south
		  	\northeast
			\pgf@y=-\pgf@y
	}
	\anchor{pathend}{
		  	\northeast
	}  
	\anchor{north}{
			\northeast
			\pgf@circ@res@step=\pgf@y
			\left
			\pgf@y=\pgf@circ@res@step
			\pgf@x=.5\pgf@x
		}  
	 \anchor{west}{
			\left
	 }
	 \anchor{east}{
		  	\northeast
			\pgf@y=0pt
	 }  
	\anchor{south}{
			\northeast
			\pgf@circ@res@step=\pgf@y
			\left
			\pgf@y=-\pgf@circ@res@step
			\pgf@x=.5\pgf@x
	}
	\anchor{south west}{
			\northeast
			\pgf@circ@res@step=\pgf@y
			\left
			\pgf@y=-\pgf@circ@res@step
	}
	\anchor{north east}{
		\northeast
	}
	\anchor{north west}{
			\northeast
			\pgf@circ@res@step=\pgf@y
			\left
			\pgf@y=\pgf@circ@res@step
	}
	\anchor{south east}{
		\northeast
		\pgf@y=-\pgf@y
	}
	\anchor{B}{
			 \northeast
	         \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
	         \left
	         \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
	}
	\anchor{base}{
			 \northeast
	         \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
	         \left
	         \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
	}
		\anchor{G}{
	         \northeast
	         \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
	         \left
	         \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
		}
		\anchor{gate}{
	         \northeast
	         \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
	         \left
	         \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
		}	
	 \anchor{nobase}{
	 		 	\left
	 		 	\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@x
	 }
	 	\anchor{nogate}{
	 		\left
	 		\pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@x
	 	}	
	 	\anchor{E}{
	 		\northeast
	 		\pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{emitter}{
	 		\northeast
	 		\pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{C}{
	 		\northeast
	 		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{collector}{
	 		\northeast
	 		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{S}{
	 		\northeast
	 		\pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{source}{
	 		\northeast
	 		\pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{D}{
	 		\northeast
	 		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}
	 	\anchor{drain}{
	 		\northeast
	 		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
	 	}	
	  #2
	  \backgroundpath{
	  	\pgftransformationadjustments		
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			%
			\ifnum \pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction} > 0
				\pgf@circuit@trans@ntypetrue
			\else
				\pgf@circuit@trans@ntypefalse
			\fi
			\northeast
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = \pgf@x
			\left
			\pgf@circ@res@left = \pgf@x
			%
			#3
			% BODY DIODE
			\ifpgf@circuit@fet@bodydiode
			\drawbodydiode{#1}
			\fi
	  %
	  }
	}
}

\long\def\drawbodydiode#1{
        \pgfscope
	         \pgftransformshift{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\pgf@circ@res@up+\pgf@circ@res@down}}
	        \pgftransformrotate{90}
			\pgftransformscale{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode scale}}
			\ifpgf@circuit@fulldiode
				\pgfnode{fulldiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
			\else
				\pgfnode{emptydiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
			\fi
		\endpgfscope
		%Draw upper connection to body diode
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
						{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}
						{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
			 	\pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{east}}
		\pgfusepath{draw}
		\pgfscope
	        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}
        	       {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
   	       	\pgftransformscale{0.5}
        \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
      \endpgfscope{}
   		%Draw lower connection to body diode
	   \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
	        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
			 	\pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{west}}
		\pgfusepath{draw}
		\pgfscope
      \pgftransformshift{\pgfpoint{\pgf@circ@res@right}		        	       {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
  	       		\pgftransformscale{0.5}
      \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
    \endpgfscope
}

\long\def\declarebpt#1{
	\pgfcircdeclaretransistor{#1}{}{
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@up}}
		\pgfusepath{draw}
	
		\pgfscope
		\pgfpathmoveto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
		\pgfsetlinewidth{2\pgflinewidth}
		\pgfusepath{draw}
		\endpgfscope
		
		\pgfpathmoveto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}		
		\pgfusepath{draw}
		%draw arrow depending on type of transiytor
	 	\pgfscope
	 	\pgfslopedattimetrue
	 	\pgfallowupsidedownattimetrue
	 	\pgfresetnontranslationattimefalse
		\ifpgf@circuit@trans@ntype
		 	\pgftransformlineattime{.5}{%
		 		\pgfpoint%
		 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
		 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@down}%
		 	}{%
		 		\pgfpoint{\pgf@circ@res@right}%
		 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}%
		 	}
		\else
		 	\pgftransformlineattime{.5}{%
		 		\pgfpoint{\pgf@circ@res@right}%
		 				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}%
		 		}{%
		 		\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
		 				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@up}%
		 		}
		\fi
		\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
		\endpgfscope
	
		\ifpgf@circuit@bpt@drawphoto
					\pgfscope
					\pgfsetarrowsstart{latex'}
					\pgfpathmoveto{\pgfpointadd{\pgfpoint
										{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
										{\pgf@circ@res@up+\pgf@circ@res@down}}
										{\pgfpoint{0.05\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
					\pgfpathlineto{\pgfpointadd{\pgfpoint
										{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
										{\pgf@circ@res@up+\pgf@circ@res@down}}
										{\pgfpoint{0.5\pgf@circ@res@left}{0.3\pgf@circ@res@up}}}
					\pgfusepath{draw}
					\pgfpathmoveto{\pgfpointadd{\pgfpoint
										{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
										{\pgf@circ@res@up+\pgf@circ@res@down}}
										{\pgfpoint{0.05\pgf@circ@res@left}{-0.1\pgf@circ@res@up}}}
					\pgfpathlineto{\pgfpointadd{\pgfpoint
										{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
										{\pgf@circ@res@up+\pgf@circ@res@down}}
										{\pgfpoint{0.5\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
					\pgfusepath{draw}
					\endpgfscope
		\else
		\ifpgf@circuit@bpt@drawbase
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
				{\pgf@circ@res@up+\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
			\pgfusepath{draw}
		\fi
		\fi
	}
}

\declarebpt{npn}
\declarebpt{pnp}

\long\def\declareigbt#1{
\pgfcircdeclaretransistor{#1}{}
{
	%draw upper connection
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@up}}
	\pgfusepath{draw}

	%draw thicker gate lines
	\pgfscope
	\pgfpathmoveto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
	\pgfpathmoveto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
	\pgfsetlinewidth{2\pgflinewidth}
	\pgfusepath{draw}
	\endpgfscope
	%draw lower connection		
	\pgfpathmoveto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}		
	\pgfusepath{draw}
	%draw arrow depending on type of transiytor
 	\pgfscope
 	\pgfslopedattimetrue
 	\pgfallowupsidedownattimetrue
 	\pgfresetnontranslationattimefalse
	\ifpgf@circuit@trans@ntype
	 	\pgftransformlineattime{.5}{%
	 		\pgfpoint%
	 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
	 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@down}%
	 	}{%
	 		\pgfpoint{\pgf@circ@res@right}%
	 			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}%
	 	}
	\else
	 	\pgftransformlineattime{.5}{%
	 		\pgfpoint{\pgf@circ@res@right}%
	 				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}%
	 		}{%
	 		\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
	 				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@up}%
	 		}
	\fi
	\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
	\endpgfscope
	%draw gate
	\ifpgf@circuit@trans@ntype	
		\pgfpathmoveto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}				
	\else
		\pgfpathmoveto{\pgfpoint
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
			{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@up}}			
	\fi
	\pgfusepath{draw}
}
}

\declareigbt{pigbt}
\declareigbt{nigbt}
\declareigbt{Lnigbt}
\declareigbt{Lpigbt}


\pgfcircdeclaretransistor{nmos}{}{%
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}

			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
			\pgfusepath{draw}
			
			\pgfscope
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base height}\pgf@circ@res@down}}
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
			\endpgfscope
		\ifpgf@circuit@mos@arrows
			\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgfresetnontranslationattimefalse
			\pgftransformlineattime{.6}{%
				\pgfpoint%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}%
			}{%
				\pgfpoint
					{\pgf@circ@res@right}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}%
			}
			\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
			\endpgfscope
		\fi

		\ifpgf@circuit@bpt@drawgate			
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
				{\pgf@circ@res@up+\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
			\pgfusepath{draw}
		\fi
}


\pgfcircdeclaretransistor{pmos}{}{%
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
			\pgfusepath{draw}

		\ifpgf@circuit@mos@arrows
			\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgfresetnontranslationattimefalse
			\pgftransformlineattime{.4}{%
				\pgfpoint%
					{\pgf@circ@res@right}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}%
			}{%
				\pgfpoint
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}%
			}
			\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
			\endpgfscope
		\fi

			\pgfscope
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base height}\pgf@circ@res@down}}
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
			\endpgfscope
			
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}		


			\pgfusepath{draw}		
			\ifpgf@circuit@bpt@drawgate
				\pgfpathmoveto{\pgfpoint
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
					{\pgf@circ@res@up+\pgf@circ@res@down}}
				\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
				\pgfusepath{draw}
			\fi
			\pgfpathcircle{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left - \pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
				{\pgf@circ@res@up+\pgf@circ@res@down}}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
			\ifpgf@circuit@pmos@emptycircle
				\pgfsetfillcolor{white}
			\fi
			\pgfusepath{draw,fill}		
}

\long\def\drawfetcore#1{
	\pgftransformationadjustments
		%top connection
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
		\pgfusepath{draw}
		\pgfscope
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
		\ifpgf@circuit@trans@depletiontype
		      \pgfpathlineto{\pgfpoint
		        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
		        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
		\else

      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up*0.45}}
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up*0.25}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down*0.25}}
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nfet/base height}\pgf@circ@res@down*0.45}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
        \fi
      \pgfsetlinewidth{2\pgflinewidth}
		\pgfusepath{draw}
		\endpgfscope
		%Bulk connection line
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
      
      %bottom connection
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
       {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}    
      \pgfusepath{draw}
     
     %draw thick gate line 
    \pgfscope
    \pgfpathmoveto{\pgfpoint
      {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
      {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint
      {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
      {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfsetlinewidth{2\pgflinewidth}
    \pgfusepath{draw}
    \endpgfscope
    
      \pgfscope
          \pgfslopedattimetrue 
          \pgfallowupsidedownattimetrue
          \pgfresetnontranslationattimefalse
          
          \pgftransformlineattime{.6}{%
            \pgfpoint
              {\pgf@circ@res@right}%
              {\pgf@circ@res@up+\pgf@circ@res@down}%
          }{%
            \pgfpoint%
              {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
              {\pgf@circ@res@up+\pgf@circ@res@down}%
          }
          	  \ifpgf@circuit@trans@ntype
          	  \else
          	  \pgftransformrotate{180}
          	  \fi
          \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
          \endpgfscope
      
      	% GATE CONNECTION
      	\ifpgf@circuit@bpt@drawgate
			\ifpgf@circuit@trans@ntype
		      	\pgfpathmoveto{\pgfpoint
		      		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
		      		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
		      	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
	      	\else
		      	\pgfpathmoveto{\pgfpoint
		      		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
		      		{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
		      	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}      	
	      	\fi
      	\pgfusepath{draw}
      	\fi

}

\long\def\pgfdeclaretransistorwrapperaddbulk#1#2#3
{\pgfcircdeclaretransistor{#1}{
	\anchor{bulk}{\left\pgf@x=0pt}
 	\anchor{B}{\left\pgf@x=0pt}%override Base anchor from npn&igbt
	 #2
	 }
	 {#3}
}


\pgfdeclaretransistorwrapperaddbulk{nfet}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{nfet}
}


\pgfdeclaretransistorwrapperaddbulk{pfet}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{pfet}
}

% N-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfete}{}{%	
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{nigfete}
	     
      % SOURCE CONNECTION
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}    
      \pgfusepath{draw}
      
      % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
      \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
          \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
        \pgfnode{circ}{center}{}{}{}
      \endpgfscope{}
      \fi
}




% N-CHANNEL IGFET ENHANCEMENT TYPE with Bulk connector
\pgfdeclaretransistorwrapperaddbulk{nigfetebulk}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{nigfetebulk}
    % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
      \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
          \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfetebulk/gate height}\pgf@circ@res@down}}
        \pgfnode{circ}{center}{}{}{}
      \endpgfscope{}
      \fi
}



% N-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfetd}{}{%
	\pgf@circuit@trans@depletiontypetrue
	\drawfetcore{nigfetd}

      % SOURCE CONNECTION
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}    
      \pgfusepath{draw}
             
      % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
      \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
          \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
        \pgfnode{circ}{center}{}{}{}
      \endpgfscope{}
      \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfete}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{pigfete}
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    
      % SOURCE CONNECTION
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}    
      \pgfusepath{draw}
      
      
      % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
      \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
          \pgfkeysvalueof{/tikz/circuitikz/tripoles/pigfete/gate height}\pgf@circ@res@up}}
        \pgfnode{circ}{center}{}{}{}
      \endpgfscope
      \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE with bulk connector
\pgfdeclaretransistorwrapperaddbulk{pigfetebulk}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{pigfetebulk}
}


% P-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfetd}{}{%
	\pgf@circuit@trans@depletiontypetrue
	\drawfetcore{pigfetd}
  
      % SOURCE CONNECTION
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}    
      \pgfusepath{draw}
      
            
      % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
      \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
          \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@up}}
        \pgfnode{circ}{center}{}{}{}
      \endpgfscope{}
      \fi
}

\pgfcircdeclaretransistor{njfet}{}{%
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@up}}

			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}		
			\pgfusepath{draw}
			
			\pgfscope
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height}\pgf@circ@res@down}}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
			\endpgfscope
			
			\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgfresetnontranslationattimefalse
			\pgftransformlineattime{.6}{%
				\pgfpoint{\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}%
			}{%
				\pgfpoint
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}%
			}
			\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
			\endpgfscope
	
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
			\pgfusepath{draw}
}


\pgfcircdeclaretransistor{pjfet}{}{%
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}

			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}		
			\pgfusepath{draw}
			
			\pgfscope
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height}\pgf@circ@res@down}}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
			\endpgfscope
			
			\pgfscope             
			\pgfslopedattimetrue 
			\pgfallowupsidedownattimetrue
			\pgfresetnontranslationattimefalse
			\pgftransformlineattime{.4}{%
				\pgfpoint%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
			}{%
				\pgfpoint{\pgf@circ@res@left}%
					{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
			}
			\pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
			\endpgfscope

					
			\pgfpathmoveto{\pgfpoint
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
				{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
			\pgfusepath{draw}
}


\pgfdeclaretransistorwrapperaddbulk{isfet}{}{%
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
      % DRAIN CONNECTION 
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@up}}
      % DRAIN
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@up}}
      \pgfusepath{draw}
      
      % GATE, DEPLETION TYPE
      \pgfscope %% added
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base height}\pgf@circ@res@up}}
      \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base height}\pgf@circ@res@down}}
      \pgfsetlinewidth{2\pgflinewidth} %% added
      \pgfusepath{draw} %% added
      \endpgfscope %% added
      
      % BULK
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
       \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+.5\pgflinewidth}
         {\pgf@circ@res@up+\pgf@circ@res@down}}

      % SOURCE
      \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@down}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
         {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@down}}
      % SOURCE CONNECTION
      \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
      \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}    
      \pgfusepath{draw}
      
      % GATE
      %\pgfscope
      %\pgfpathmoveto{\pgfpoint
       % {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate width}\pgf@circ@res@left}
       % {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@up}}
      %\pgfpathlineto{\pgfpoint
       % {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate width}\pgf@circ@res@left}
       % {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@down}}
      %\pgfsetlinewidth{2\pgflinewidth}
      %\pgfusepath{draw}
      %\endpgfscope
      
            
      % SOLDER DOT at source-bulk connection
      \ifpgf@circuit@fet@solderdot
	      \pgfscope
	        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
	          \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
	        \pgfnode{circ}{center}{}{}{}
	      \endpgfscope{}
      \fi
      % ARROW
      \pgfscope
      \pgfslopedattimetrue 
      \pgfallowupsidedownattimetrue
      \pgfresetnontranslationattimefalse
      \pgftransformlineattime{.6}{%
        \pgfpoint
          {\pgf@circ@res@right}%
          {\pgf@circ@res@up+\pgf@circ@res@down}%
      }{%
        \pgfpoint%
          {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}%
          {\pgf@circ@res@up+\pgf@circ@res@down}%
      }
      \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
      \endpgfscope
      \pgfusepath{draw}
      
      % Wavy lines
      	\pgfscope
			\pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves y sep}\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfusepath{draw}

			\pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{0cm}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfusepath{draw}

			\pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves y sep}\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
			\pgfusepath{draw}
		\endpgfscope

}


%% Black thyristor

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{G}{
		\northeast
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}{\ctikzvalof{tripoles/thyristor/height 2}}{fullthyristor}{\ctikzvalof{tripoles/thyristor/height}}{\ctikzvalof{tripoles/thyristor/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
	\pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@other}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
				
		\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} 
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfusepath{draw,fill}
		
		\pgfsetlinewidth{\pgfstartlinewidth}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{\pgfstartlinewidth}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	
	\pgfusepath{draw}
	
}

%% Empty thyristor

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{G}{
		\northeast
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}{\ctikzvalof{tripoles/thyristor/height 2}}{emptythyristor}{\ctikzvalof{tripoles/thyristor/height}}{\ctikzvalof{tripoles/thyristor/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
	\pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

	\pgfscope
		\pgftransformxshift{\pgf@circ@res@other}
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
				
		\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} 
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfusepath{draw}
		
		\pgfsetlinewidth{\pgfstartlinewidth}
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
		\pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
		\pgfusepath{draw}
	\endpgfscope
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{\pgfstartlinewidth}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	
	\pgfusepath{draw}
	
}

%% Empty triac

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{G}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}{\ctikzvalof{tripoles/triac/height}}{emptytriac}{\ctikzvalof{tripoles/triac/height}}{\ctikzvalof{tripoles/triac/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
	\pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	
	\pgfusepath{draw}
	
	\pgfsetlinewidth{\pgfstartlinewidth}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	
	\pgfusepath{draw}
	
}

%% Empty triac

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{G}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}{\ctikzvalof{tripoles/triac/height}}{fulltriac}{\ctikzvalof{tripoles/triac/height}}{\ctikzvalof{tripoles/triac/width}}{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

	\pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
	\pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	
	\pgfusepath{draw,fill}
	
	\pgfsetlinewidth{\pgfstartlinewidth}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	
	\pgfusepath{draw}
	
}







\pgfcircdeclarebipole{
	\anchor{out 1}{
		\northeast
		\pgf@y=0cm
	}
	\anchor{out 2}{
		\northeast
		\pgf@y=.8\pgf@y
	}
}{\ctikzvalof{tripoles/toggleswitch/height 2}}{toggleswitch}{\ctikzvalof{tripoles/toggleswitch/height}}{\ctikzvalof{tripoles/toggleswitch/width}}{

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
	\pgfpathlineto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
	\pgfusepath{draw}
	\pgfscope
	\pgfpathmoveto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{.5\pgf@circ@res@up}}
	\pgfusepath{draw}
	\endpgfscope
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.8\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.8\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.15\pgf@circ@res@up}}
	\pgfusepath{draw}
	
	
	\pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfusepath{draw}
	
	\pgfsetdash{{.08\pgf@circ@res@up}{.04\pgf@circ@res@up}{.7\pgf@circ@res@up}{.04\pgf@circ@res@up}{.8\pgf@circ@res@up}}{0cm}
	\pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0}{.8\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{.2\pgf@circ@res@left}{.6\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0}{.4\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0}{.2\pgf@circ@res@up}}
	\pgfusepath{draw}
	\pgfsetdash{}{0cm}
}










\pgfdeclareshape{op amp}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	  }
	  \anchor{north}{
		\northwest
		\pgf@x=0pt
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{leftedge}
	  {\left
		  \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }	  
	  \anchor{-}{
		\inOne
	  }
	  \anchor{+}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\up{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
	    \pgfpointlineattime{
			\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/up pos}}{
			\pgfpoint{
				\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
				{\pgf@circ@res@up}}
			{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	  }
	  \anchor{up}{
		\up
	  }
	  \anchor{down}{
		\up
		\pgf@y=-\pgf@y
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  	\anchor{west}{
		  	\left
    	  }
		  \anchor{east}{
		  	\left
		  	\pgf@x=-\pgf@x
		  }  
	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
			
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $-$}
	

	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $+$}
		
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	\pgfsetrectcap
	\pgfusepath{draw}

						
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
		\pgfpathclose
		\pgfusepath{draw}
	\endpgfscope
		
		
	  
	  }
	}

%op amp shape as in european standard en 60617
\pgfdeclareshape{en amp}
{
	\anchor{center}{\pgfpointorigin}
	\savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	}
	\anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
	\savedanchor\left{%
	  	\pgf@y=0pt
	}
	\anchor{leftedge}
	{
		\left
	 	\pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/port width}\pgf@x
	}
	\savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	}	  
	\anchor{-}{
		\inOne
	}
	\anchor{+}{
		\inOne
		\pgf@y=-\pgf@y
	}
	\anchor{up}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{down}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{west}{
		\left
	}
	\anchor{east}{
	  	\left
		\pgf@x=-\pgf@x
	}
	\backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@up}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/font} $-$}
	
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@down}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/font} $+$}
		
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	\pgfsetrectcap
	\pgfusepath{draw}
				
	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgfpathmoveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathclose
		\pgfusepath{draw}
	\endpgfscope

	\pgftext[base,y=-3ex,at=\pgfpoint{.3\pgf@circ@res@left}{\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/font2} $\triangleright$}
	\pgftext[base,y=-3ex,at=\pgfpoint{.3\pgf@circ@res@right}{\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/en amp/font2} $\infty$}
	  }
}

%%Transkonduktanzverstärker
\pgfdeclareshape{gm amp}
	{
	  \anchor{center}{\pgfpointorigin}
	  \savedanchor\northwest{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }
	  \anchor{south}{
		\northwest
		\pgf@y=-\pgf@y
	  }
	  \anchor{north}{
		\northwest
	  }
	  \savedanchor\left{%
	  	\pgf@y=0pt
	  }
	  \anchor{leftedge}
	  {\left
  	  	\pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
	  }
	  \savedanchor\inOne{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
	  }	  
	  \anchor{-}{
		\inOne
	  }
	  \anchor{+}{
		\inOne
		\pgf@y=-\pgf@y
	  }
	  \savedanchor\up{%
		\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
		\pgf@y=.5\pgf@y
		\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
		\pgf@x=.5\pgf@x
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
	    \pgfpointlineattime{
			\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/up pos}}{
			\pgfpoint{
				\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
				{\pgf@circ@res@up}}
			{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
	  }
	  \anchor{up}{
		\up
	  }
	  \anchor{down}{
		\up
		\pgf@y=-\pgf@y
	  }
	  \anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	  }
	  	\anchor{west}{
		  	\left
    	  }
		  \anchor{east}{
		  	\left
		  	\pgf@x=-\pgf@x
		  }  
	  
	  \backgroundpath{			
			\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
						
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x
			\pgf@circ@res@left = \pgf@x
			
	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $-$}
	

	\pgfpathmoveto{\pgfpoint
		{\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}}
	\pgfpathlineto{\pgfpoint
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
		{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}}
	\pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} $+$}
		
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{.3\pgf@circ@res@right}{0pt}} %
		\pgfsetrectcap
	\pgfusepath{draw}

	\pgfscope
		\pgfsetlinewidth{2\pgflinewidth}
		\pgftransformxshift{.7\pgf@circ@res@left}
		\pgf@circ@res@step=\pgf@circ@res@right
		\advance\pgf@circ@res@step by -\pgf@circ@res@left
		\pgf@circ@res@step=.7\pgf@circ@res@step
		%Umrandung:
		\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}} %geändert startpunkt neu am ausgangsstrich
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}%vom Ausgang nach oben
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}} %neu ecke links oben nach rechts oben
		\pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} %bei deneigängen runter 
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}%ecke links unten nach rechts unten
		\pgfpathclose
		\pgfusepath{draw}
	\endpgfscope
  
	  }
	}	



%% Potentiometer
\pgfcircdeclarebipole{
	\anchor{wiper}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}
	\anchor{W}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}	
}{\ctikzvalof{bipoles/potentiometer/height 2}}{potentiometer}{\ctikzvalof{bipoles/potentiometer/height}}{\ctikzvalof{bipoles/potentiometer/width}}{
\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
\pgftransformationadjustments
\pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
\divide \pgf@circ@res@step by 12

\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}

\pgf@circ@res@other = \pgf@circ@res@left
\advance\pgf@circ@res@other by \pgf@circ@res@step 
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
\advance\pgf@circ@res@other by 2\pgf@circ@res@step 
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
\advance\pgf@circ@res@other by 2\pgf@circ@res@step
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
\advance\pgf@circ@res@other by 2\pgf@circ@res@step
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
\advance\pgf@circ@res@other by 2\pgf@circ@res@step
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
\advance\pgf@circ@res@other by 2\pgf@circ@res@step
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
\advance\pgf@circ@res@other by \pgf@circ@res@step
\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
\pgfsetbeveljoin
\pgfusepath{draw}

\pgfscope
	%\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfsetarrowsend{latex'}
	\pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
	\pgfusepath{draw}
\endpgfscope
}





%% Generic tunable 

\pgfcircdeclarebipole{
	\anchor{wiper}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}
}{\ctikzvalof{bipoles/generic potentiometer/height 2}}{genericpotentiometer}{\ctikzvalof{bipoles/generic potentiometer/height}}{\ctikzvalof{bipoles/generic potentiometer/width}}{

		\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
		\divide \pgf@circ@res@step by 14

		\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
					
		\pgfusepath{draw} 
		
		\pgfscope
		%\pgfsetlinewidth{\pgfstartlinewidth}
		\pgfsetarrowsend{latex'}
		\pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
		\pgfusepath{draw}
		\endpgfscope
}


\pgfdeclareshape{mixer}
{
	\savedanchor\northwest{
		\ifpgf@circuit@boxed
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\else	
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/mixer/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/mixer/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\fi
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{left}{%
		\northwest
		\pgf@y=0pt
	}
	\anchor{1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{3}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{4}{
		\northwest
		\pgf@y=\pgf@y
		\pgf@x=0pt
	}
	\anchor{in 1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{in1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{in}{
		\northwest
		\pgf@y=0pt
	}	  
	\anchor{in 2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{in2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{center}{
		\pgf@y=0pt
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x  
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	}
	\anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	}
	\anchor{north west}{
		\northwest
	}
	\anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	}
	\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
		\pgf@circ@res@step=\ctikzvalof{tripoles/mixer/width}\pgf@circ@Rlen
			
		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			
			% draw outer box
			\ifpgf@circuit@boxed
				\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
			\fi
			
			% draw outer circle
			\ifpgf@circuit@boxed
				\pgf@circ@res@step=.7\pgf@circ@res@step
				\pgfsetdash{}{0pt}	% draw solid circle if boxed
			\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\fi
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
			\pgfusepath{draw}
			
			% draw inner stuff
			\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathmoveto{\pgfpointpolar{135}{0.5\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpointpolar{-45}{0.5\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathmoveto{\pgfpointpolar{45}{0.5\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpointpolar{-135}{0.5\pgf@circ@res@step}}
			\pgfusepath{draw}
			
		\endpgfscope
	}
}

\pgfdeclareshape{adder}
{
	\savedanchor\northwest{
		\ifpgf@circuit@boxed
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\else	
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/adder/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/adder/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\fi
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{left}{%
		\northwest
		\pgf@y=0pt
	}
	\anchor{1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{3}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{4}{
		\northwest
		\pgf@y=\pgf@y
		\pgf@x=0pt
	}
	\anchor{in 1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{in1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{in}{
		\northwest
		\pgf@y=0pt
	}	  
	\anchor{in 2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{in2}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{out}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{center}{
		\pgf@y=0pt
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x  
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	}
	\anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	}
	\anchor{north west}{
		\northwest
	}
	\anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	}
	\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
		\pgf@circ@res@step=\ctikzvalof{tripoles/adder/width}\pgf@circ@Rlen
			
		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			
			% draw outer box
			\ifpgf@circuit@boxed
				\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
			\fi
			
			% draw outer circle
			\ifpgf@circuit@boxed
				\pgf@circ@res@step=.7\pgf@circ@res@step{}
				\pgfsetdash{}{0pt}	% draw solid circle if boxed
			\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\fi
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
			\pgfusepath{draw}
			
			% draw inner stuff
			\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
			\pgfsetlinewidth{\pgfstartlinewidth}
			
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathmoveto{\pgfpointpolar{0}{0.3\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpointpolar{180}{0.3\pgf@circ@res@step}}
			\pgfpathmoveto{\pgfpointorigin}
			\pgfpathmoveto{\pgfpointpolar{90}{0.3\pgf@circ@res@step}}
			\pgfpathlineto{\pgfpointpolar{270}{0.3\pgf@circ@res@step}}
			\pgfsetlinewidth{2\pgflinewidth}
			\pgfusepath{draw}
			
		\endpgfscope				  
	}
}

\pgfdeclareshape{oscillator}
{
	\savedanchor\northwest{
		\ifpgf@circuit@boxed
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
		\else	
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/oscillator/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/oscillator/width}\pgf@circ@Rlen
		\fi
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{north}{
		\northwest
		\pgf@x=.5\pgf@x
	}
	\anchor{south}{
		\northwest
		\pgf@x=.5\pgf@x
		\pgf@y=-\pgf@y
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=0pt
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{text}{
		\pgf@x=-2\pgf@x
		\advance \pgf@x by -.5\wd\pgfnodeparttextbox
		\advance \pgf@y by -1.5\ht\pgfnodeparttextbox
	}
	\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
			
		\pgf@circ@res@step=\ctikzvalof{tripoles/oscillator/width}\pgf@circ@Rlen{}
			
		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			
			\pgftransformxshift{-0.5\pgf@circ@res@step} % The oscillator is shifted to the left, so a connection comes out of the anchor "east"
			
			% draw outer box
			\ifpgf@circuit@boxed{}
				\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
			\fi
			
			% draw outer circle
			\ifpgf@circuit@boxed
				\pgf@circ@res@step=.7\pgf@circ@res@step{}
				\pgfsetdash{}{0pt}	% draw solid circle if boxed
			\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\fi
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
			\pgfusepath{draw}
			
			% draw inner sine waves
			\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
			\pgfsetlinewidth{\pgfstartlinewidth}
			\pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
			\pgfpathmoveto{\pgfpoint{-0.3\pgf@circ@res@step}{0\pgf@circ@res@step}}
			\pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}
			\pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
			\pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
			\pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}
		
			\pgfusepath{draw}
			
		\endpgfscope				  
	}
}

\pgfdeclareshape{circulator}
{
	\savedanchor\northwest{
		\ifpgf@circuit@boxed
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\else	
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/circulator/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/circulator/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\fi
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{left}{%
		\northwest
	  	\pgf@y=0pt
	}
	\anchor{1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{2}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{3}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x  
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	}
	\anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	}
	\anchor{north west}{
		\northwest
	}
	\anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	}
	\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
		\pgf@circ@res@step=\ctikzvalof{tripoles/circulator/width}\pgf@circ@Rlen
			
		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			
			% draw outer box
			\ifpgf@circuit@boxed
				\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
			\fi
			
			% draw outer circle
			\ifpgf@circuit@boxed{}
				\pgf@circ@res@step=.7\pgf@circ@res@step{}
				\pgfsetdash{}{0pt}	% draw solid circle if boxed
			\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\fi
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
			\pgfusepath{draw}
			
			% inner arrow
			\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
			\pgfsetlinewidth{\pgfstartlinewidth}
			
			\pgfsetarrowsend{latex}
			\pgfpathmoveto{\pgfpoint{-0.25\pgf@circ@res@step}{0}}
			\pgfpatharc{180}{-90} {0.25\pgf@circ@res@step}
			\pgfpathlineto{\pgfpoint{-5pt}{-0.2\pgf@circ@res@step}}
			\pgfusepath{draw}
			
		\endpgfscope				  
	}
}


% Wilkinson divider
\pgfdeclareshape{wilkinson}{
		\anchor{center}{
			\northwest
			\pgf@x=0pt
			\pgf@y=0pt
		}
		\savedanchor\northwest{%
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/wilkinson/height}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x= \pgf@circ@Rlen
			\pgf@x=.5\pgf@x
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/wilkinson/width}\pgf@x
			}
		\anchor{north}{
			\northwest
			\pgf@x=0pt
		}
		\anchor{south}{
			\northwest
			\pgf@x=0pt
			\pgf@y=-\pgf@y
		}
		\anchor{west}{
			\northwest
			\pgf@y=0pt
		}
		\anchor{east}{
			\northwest
			\pgf@y=0pt
			\pgf@x=-\pgf@x
		}
		\anchor{south west}{
			\northwest
			\pgf@y=-\pgf@y
		}
		\anchor{north east}{
			\northwest
			\pgf@x=-\pgf@x
		}
			\anchor{north west}{
			\northwest
		}
		\anchor{south east}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=-\pgf@y
		}
		\anchor{in}{
			\northwest
			\pgf@y=0pt
		}
		\anchor{out1}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=-0.5\pgf@y
		}
		\anchor{out2}{
			\northwest
			\pgf@x=-\pgf@x
			\pgf@y=0.5\pgf@y
		}
		\anchor{text}{
			\northwest
			\advance \pgf@y by 0.5\ht\pgfnodeparttextbox
			\pgf@x=-.5\wd\pgfnodeparttextbox
		}
		\backgroundpath{			
				\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}	
			
				\northwest
				\pgf@circ@res@up = \pgf@y 
				\pgf@circ@res@down = -\pgf@y
				\pgf@circ@res@right = -\pgf@x
				\pgf@circ@res@left = \pgf@x
			
				\pgfstartlinewidth=\pgflinewidth

				% draw outer box
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
				\pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
				\pgfusepath{draw}
				
				% draw inner stuff
				\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
				\pgfsetarrows{-} %never draw arrows
				\pgfsetlinewidth{\pgfstartlinewidth}
				\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
				\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
				\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}				
				
				\pgfusepath{draw}
				
				\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
				% draw inner resisitor - european or american style is recognised
				{
					\pgftransformshift{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
					\pgftransformrotate{90}
					
					% calculate size of resistor
					\ifpgf@circuit@europeanresistor
						\pgfmathparse{\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/generic/width} / 2}
						\pgftransformscale{\pgfmathresult}
						\pgfnode{genericshape}{center}{}{pgf@generic}{\pgfusepath{fill}}
					\else
						\pgfmathparse{\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/resistor/width} / 2}
						\pgftransformscale{\pgfmathresult}
						\pgfnode{resistorshape}{center}{}{pgf@resistor}{\pgfusepath{fill}}
					\fi
				}
				
				\pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.25\pgf@circ@res@up}}
				
				\pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.25\pgf@circ@res@down}}
				\pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
				\pgfusepath{draw}

		}
}

% electromechanical device (motor/generator)
\pgfdeclareshape{elmech}
{
	\savedanchor\northwest{
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/elmech/height}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/elmech/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
	}
	\anchor{center}{
		\pgfpointorigin
	}
	  \anchor{text}{
		\pgfpointorigin
		\advance \pgf@x by -.5\wd\pgfnodeparttextbox
		\advance \pgf@y by -.5\ht\pgfnodeparttextbox
	}
	\anchor{left}{%
		\northwest
		\pgf@y=0pt
	}
	\anchor{right}{%
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{top}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{pathstart}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{pathend}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{bottom}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{center}{
		\pgf@y=0pt
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
		\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
		\pgf@circ@res@step=\ctikzvalof{tripoles/elmech/width}\pgf@circ@Rlen
		\pgf@circ@res@up=\ctikzvalof{tripoles/elmech/height}\pgf@circ@Rlen
		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			% draw outer box
		%	\ifpgf@circuit@boxed
		%		\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
		%	\fi
			% draw outer circle
			%\ifpgf@circuit@boxed
			%	\pgf@circ@res@step=.7\pgf@circ@res@step
			%	\pgfsetdash{}{0pt}	% draw solid circle if boxed
			%\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			%\fi
			\pgfpathrectangle{\pgfpoint{-.25\pgf@circ@res@step}{-.5\pgf@circ@res@up}}{\pgfpoint{.5\pgf@circ@res@step}{\pgf@circ@res@up}}
			\pgfsetfillcolor{black}
			\pgfusepath{draw,fill}
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
			\pgfsetfillcolor{white}
			\pgfusepath{draw,fill}
		\endpgfscope
	}
}

\pgfdeclareshape{magnetron}
{
	\savedanchor\northwest{
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/magnetron/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/magnetron/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{anode}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{cathode1}{
		\northwest
		\pgf@circ@res@step=\pgf@y
		\pgfmathparse{cos(105)}
		\pgf@x=\pgfmathresult\pgf@circ@res@step
		\pgfmathparse{sin(105)}
		\pgf@y=\pgfmathresult\pgf@circ@res@step
		%\pgfpointorigin
		%\pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
	}
	\anchor{cathode2}{
		\northwest
		\pgf@circ@res@step=\pgf@y
		\pgfmathparse{cos(75)}
		\pgf@x=\pgfmathresult\pgf@circ@res@step
		\pgfmathparse{sin(75)}
		\pgf@y=\pgfmathresult\pgf@circ@res@step
		%\pgfpointorigin
		%\pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
	}
	  \anchor{text}{
		\pgfpointorigin
		\advance \pgf@x by -.5\wd\pgfnodeparttextbox
		\advance \pgf@y by -.5\ht\pgfnodeparttextbox
	}
	\anchor{left}{%
		\northwest
		\pgf@y=0pt
	}
	\anchor{right}{%
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{top}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{pathstart}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{pathend}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{bottom}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{center}{
		\pgf@y=0pt
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
		\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
		\pgf@circ@res@step=\ctikzvalof{tripoles/magnetron/width}\pgf@circ@Rlen
			\northwest
			\pgf@circ@res@up = \pgf@y 
			\pgf@circ@res@down = -\pgf@y
			\pgf@circ@res@right = -\pgf@x  
			\pgf@circ@res@left = \pgf@x
			\pgfmathsetlength{\pgf@circ@res@other}{sin(15)*\pgf@circ@res@up}

		\pgfscope
			\pgfstartlinewidth=\pgflinewidth
			% draw outer box
		%	\ifpgf@circuit@boxed
		%		\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
		%	\fi
			% draw outer circle
			%\ifpgf@circuit@boxed
			%	\pgf@circ@res@step=.7\pgf@circ@res@step
			%	\pgfsetdash{}{0pt}	% draw solid circle if boxed
			%\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			%\fi
			%create outer circle
			\pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@right}
			\pgfsetfillcolor{white}
			\pgfusepath{draw}
			%create chambers
			 \foreach \angle in {45,135,225,315}{
						\pgfpathmoveto{ \pgfpointpolar{\angle}{0.6\pgf@circ@res@right}}
						\pgfpathlineto{ \pgfpointpolar{\angle}{\pgf@circ@res@right}}
					}
			\pgfsetroundcap
			\pgfusepath{draw}
			\pgfscope
			%draw connection from outside
			%anode
				\pgfsetlinewidth{\pgfstartlinewidth}
				\pgfpathmoveto{\pgfpoint{0\pgf@circ@res@left}{\pgf@circ@res@down}}
				\pgfpathlineto{\pgfpoint{0\pgf@circ@res@right}{.5\pgf@circ@res@down}}
				%cathodes
				\pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@up}}
				\pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
				\pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@up}}
				\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
				\pgfsetbuttcap
				\pgfusepath{draw}
			\endpgfscope
			%create cathode
			\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{0}{.15\pgf@circ@res@up}}
			\pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
						\pgfusepath{draw}
			%create anode
			\pgfpathmoveto{\pgfpoint{0.3\pgf@circ@res@left}{.5\pgf@circ@res@down}}
			\pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{.5\pgf@circ@res@down}}
			
			\pgfsetbuttcap
			\pgfusepath{draw}
		\endpgfscope
	}
}

\endinput


==> circuitikz/tex/pgfcircutils.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%\def\pgf@circ@handleSI#1{%
 % \pgf@circ@siunitx@resfalse
%  
 % \edef\len{\stringlength[e]{#1}}
  %\testmatchingchar[e]{#1}{\len}{>}%
  %\ifmatchingchar%
  %  \ifnum\findchars{#1}{<}=0
	%  \def\pgf@circ@handleSI@val{\substring{#1}{1}{\findchars{#1}{<}-1}}
	  %\def\pgf@circ@handleSI@unit{\substring{#1}{\findchars{#1}{<}-1}+1}{\stringlength{#1}}
	  %\pgf@circ@siunitx@restrue
%	\else
%	\fi
  %\else 
  %\fi
%}

\def\pgf@circ@handleSI#1{
	\noexpandarg
        	\def\pgf@temp{}
	\StrBetween{#1}{<}{>}[\pgf@circ@handleSI@unit]
	\StrLen{\pgf@circ@handleSI@unit}[\pgf@circ@handleSI@unit@len]

	\ifnum\pgf@circ@handleSI@unit@len=0  
	  \pgf@circ@siunitx@resfalse  
	\else  
	  \IfEndWith{#1}{>}{
	  	\pgf@circ@siunitx@restrue 
		\noexpandarg
	  	\StrBefore{#1}{<}[\pgf@circ@handleSI@val]		
                %\typeout{si |#1|}
	  }{
	  	\pgf@circ@siunitx@resfalse 
                %\typeout{no si |#1|}
	  }
	\fi
}

\def\pgf@circ@ifkeyempty#1{
	\pgfextra{
		\ctikzset{#1/.get=\pgf@circ@temp}
		\edef\pgf@temp{}
	}
	\ifx\pgf@circ@temp\pgf@temp
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%    Math routines

\def\pgf@circ@stripdecimals#1.#2\pgf@nil{#1}


\endinput

==> circuitikz/tex/pgfcircvoltage.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Voltage management


\ctikzset{v^>/.style = {
		v = #1,
		\circuitikzbasekey/bipole/voltage/direction = forward,
		\circuitikzbasekey/bipole/voltage/position = above
	}
}

\ctikzset{v^</.style = {
		v = #1,
		\circuitikzbasekey/bipole/voltage/direction = backward,
		\circuitikzbasekey/bipole/voltage/position = above
	}
}

\ctikzset{v_>/.style = {
		v = #1,
		\circuitikzbasekey/bipole/voltage/direction = forward,
		\circuitikzbasekey/bipole/voltage/position = below
	} 
}

\ctikzset{v_</.style = {
		v = #1,
		\circuitikzbasekey/bipole/voltage/direction = backward,
		\circuitikzbasekey/bipole/voltage/position = below
	}
}

\ctikzset{v_/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position = below} }
\ctikzset{v^/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position  = above} }
\ctikzset{v>/.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = forward} }
\ctikzset{v</.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = backward} }

% Default position varies whether the component is a voltage source
% or not
\ctikzset{v/.code = {
			\ifpgf@circuit@bipole@isvoltage
				\pgfkeys{\circuitikzbasekey/bipole/voltage/position=above,
					\circuitikzbasekey/bipole/voltage/direction=forward}
			\else
				\ifpgf@circ@oldvoltagedirection
				\pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
					\circuitikzbasekey/bipole/voltage/direction=backward}
				\else
				\pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
					\circuitikzbasekey/bipole/voltage/direction=forward}
				\fi
			\fi
			\ifpgf@circ@oldvoltagedirection\else
			\ifpgf@circuit@bipole@iscurrent
			\ifpgf@circuit@bipole@current@backward
					\pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
					\circuitikzbasekey/bipole/voltage/direction=forward}
			\else
					\pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
					\circuitikzbasekey/bipole/voltage/direction=backward}
			\fi\fi\fi
	\pgfkeys{/tikz/circuitikz/bipole/voltage/label/name=#1}
	\ctikzsetvalof{bipole/voltage/label/unit}{}
	\ifpgf@circ@siunitx 
		\pgf@circ@handleSI{#1}
		\ifpgf@circ@siunitx@res
			\edef\pgf@temp{\pgf@circ@handleSI@val}
			\pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/name}{\pgf@temp}
			\edef\pgf@temp{\pgf@circ@handleSI@unit}
			\pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/unit}{\pgf@temp}
		\else
		\fi
	\else
	\fi
	}
}




%% Output routine for generic bipoles

\def\pgf@circ@drawvoltagegeneric{
	\pgfextra{
			\edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/straight label distance}
			\pgfkeysifdefined{\pgf@temp}
				{ 
					\edef\partheight{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/straight label distance}}
					\edef\tmpdistfromline{(\partheight\pgf@circ@Rlen)}
				}
				{
				\pgfkeysifdefined{/tikz/circuitikz/bipoles/voltage/straight label distance}
					{
						\edef\partheight{\ctikzvalof{bipoles/voltage/straight label distance}}
						\edef\tmpdistfromline{(\partheight\pgf@circ@Rlen)}
					}
					{%calculate default value from part height
						\edef\partheight{0.5*\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/height}}
						\edef\tmpdistfromline{(\partheight\pgf@circ@Rlen+0.2\pgf@circ@Rlen)}
					}
				}
		\ifnum \ctikzvalof{mirror value}=-1
			\ifpgf@circuit@bipole@inverted
				\ifpgf@circuit@bipole@voltage@straight
					\def\distfromline{\tmpdistfromline}
				\else
					\def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
				\fi
			\else
				\ifpgf@circuit@bipole@voltage@straight
					\def\distfromline{-\tmpdistfromline}
				\else
					\def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
				\fi
			\fi
		\else
			\ifpgf@circuit@bipole@inverted
				\ifpgf@circuit@bipole@voltage@straight
					\def\distfromline{-\tmpdistfromline}
				\else
					\def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
				\fi
			\else
				\ifpgf@circuit@bipole@voltage@straight
					\def\distfromline{\tmpdistfromline}
				\else
					\def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
				\fi
			\fi
		\fi
		\ifpgf@circuit@bipole@voltage@below
			\def\pgf@circ@voltage@angle{90}
		\else
			\def\pgf@circ@voltage@angle{-90}
		\fi
		\edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/distance from node}
		\pgfkeysifdefined{\pgf@temp}
			{ \edef\distacefromnode{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/distance from node}} }
			{ \edef\distacefromnode{\ctikzvalof{voltage/distance from node}} }
		\edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/bump b}
		\pgfkeysifdefined{\pgf@temp}
			{ \edef\bumpb{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/bump b}} }
			{ \edef\bumpb{\ctikzvalof{voltage/bump b}} }
	}
	% %\pgf@circ@Rlen/16 is equal to the length of the currarrow
	coordinate (pgfcirc@midtmp) at ($(\tikztostart) ! \pgf@circ@Rlen/16 ! (anchorstartnode)$) %absolute move, minimum space is length of arrowhead
	coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distacefromnode ! (anchorstartnode)$)

	coordinate (pgfcirc@Vfrom) at ($(pgfcirc@midtmp) ! -\distfromline ! \pgf@circ@voltage@angle:(anchorstartnode)$)
	coordinate (pgfcirc@midtmp) at ($(\tikztotarget) ! \pgf@circ@Rlen/16 ! (anchorendnode)$)%absolute move, minimum space is length of arrowhead
	coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distacefromnode ! (anchorendnode)$)

	coordinate (pgfcirc@Vto) at ($(pgfcirc@midtmp) ! \distfromline ! \pgf@circ@voltage@angle : (anchorendnode)$)

	\ifpgf@circuit@bipole@voltage@below
		coordinate (pgfcirc@Vcont1) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-110)$)
		coordinate (pgfcirc@Vcont2) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-70)$)
	\else
		coordinate (pgfcirc@Vcont1) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.110)$)
		coordinate (pgfcirc@Vcont2) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.70)$)
	\fi

	\ifpgf@circuit@europeanvoltage
		\ifpgf@circuit@bipole@voltage@straight
			\ifpgf@circuit@bipole@voltage@backward
				(pgfcirc@Vto) --(pgfcirc@Vfrom) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
			\else
				(pgfcirc@Vfrom) --(pgfcirc@Vto) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
			\fi
		\else
			\ifpgf@circuit@bipole@voltage@backward
				(pgfcirc@Vto) .. controls (pgfcirc@Vcont2)  and (pgfcirc@Vcont1) ..
					node[currarrow, sloped,  allow upside down, pos=1] {}
				(pgfcirc@Vfrom)
			\else
				(pgfcirc@Vfrom) .. controls (pgfcirc@Vcont1)  and (pgfcirc@Vcont2) ..
					node[currarrow, sloped,  allow upside down, pos=1] {}
				(pgfcirc@Vto)
			\fi
		\fi
	\else
		\ifpgf@circuit@bipole@voltage@backward
			\ifpgf@circ@oldvoltagedirection
				(pgfcirc@Vfrom) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{\scriptsize$+$}
				(pgfcirc@Vto) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{$-$}
			\else
				(pgfcirc@Vfrom) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{\scriptsize$-$}
				(pgfcirc@Vto) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{$+$}
			\fi
		\else
			\ifpgf@circ@oldvoltagedirection
				(pgfcirc@Vfrom) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{\scriptsize$-$}
				(pgfcirc@Vto) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{$+$}
			\else
				(pgfcirc@Vfrom) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{\scriptsize$+$}
				(pgfcirc@Vto) node[inner sep=0, anchor=\pgf@circ@bipole@voltage@label@anchor]{$-$}
			\fi
		\fi
	\fi
}

%% Output routine for voltage sources
\def\pgf@circ@drawvoltagegenerator{
	\ifpgf@circuit@bipole@voltage@below
		coordinate (pgfcirc@Vfrom) at ($(\ctikzvalof{bipole/name}.center) ! \ctikzvalof{voltage/bump a} ! (\ctikzvalof{bipole/name}.-120)$)
		coordinate (pgfcirc@Vto) at ($(\ctikzvalof{bipole/name}.center) ! \ctikzvalof{voltage/bump a} ! (\ctikzvalof{bipole/name}.-60)$)
	\else
		coordinate (pgfcirc@Vfrom) at ($ (\ctikzvalof{bipole/name}.center) ! \ctikzvalof{voltage/bump a} ! (\ctikzvalof{bipole/name}.120)$)
		coordinate (pgfcirc@Vto) at ($ (\ctikzvalof{bipole/name}.center) ! \ctikzvalof{voltage/bump a} ! (\ctikzvalof{bipole/name}.60)$)
	\fi
	\ifpgf@circuit@europeanvoltage
		\ifpgf@circuit@bipole@voltage@backward
			(pgfcirc@Vto)  -- node[currarrow, sloped,  allow upside down, pos=1] {} (pgfcirc@Vfrom)
		\else
			(pgfcirc@Vfrom)  -- node[currarrow, sloped,  allow upside down, pos=1] {} (pgfcirc@Vto)
		\fi
	\else% american voltage
		\ifpgf@circuit@bipole@voltageoutsideofsymbol
		% if it is a battery, must put + and -
			\ifpgf@circuit@bipole@voltage@backward
				(pgfcirc@Vfrom)  node {$-$}  (pgfcirc@Vto) node {$+$}
			\else
				(pgfcirc@Vfrom)  node {$+$}  (pgfcirc@Vto) node {$-$}
			\fi
		\fi
	\fi
}

%% Output routine
\def\pgf@circ@drawvoltage{% node name 
%\pgf@circ@direction
	\pgfextra{
		\edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
		\ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
			\ifpgf@circuit@bipole@voltage@below
				\def\pgf@circ@bipole@voltage@label@anchor{north west}
			\else \def\pgf@circ@bipole@voltage@label@anchor{south east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
			\ifpgf@circuit@bipole@voltage@below
				\def\pgf@circ@bipole@voltage@label@anchor{west}
			\else \def\pgf@circ@bipole@voltage@label@anchor{east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
			\ifpgf@circuit@bipole@voltage@below
				 \def\pgf@circ@bipole@voltage@label@anchor{south west}
			\else \def\pgf@circ@bipole@voltage@label@anchor{north east}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
			\ifpgf@circuit@bipole@voltage@below
				  \def\pgf@circ@bipole@voltage@label@anchor{south}
			\else\def\pgf@circ@bipole@voltage@label@anchor{north}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
			\ifpgf@circuit@bipole@voltage@below
				 \def\pgf@circ@bipole@voltage@label@anchor{south east}
			\else\def\pgf@circ@bipole@voltage@label@anchor{north west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
			\ifpgf@circuit@bipole@voltage@below
				 \def\pgf@circ@bipole@voltage@label@anchor{east}
			\else \def\pgf@circ@bipole@voltage@label@anchor{west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
			\ifpgf@circuit@bipole@voltage@below
				  \def\pgf@circ@bipole@voltage@label@anchor{north east}
			\else\def\pgf@circ@bipole@voltage@label@anchor{south west}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >-1 \ifnum\pgfcircmathresult <5
			\ifpgf@circuit@bipole@voltage@below
				 \def\pgf@circ@bipole@voltage@label@anchor{north}
			\else\def\pgf@circ@bipole@voltage@label@anchor{south}
			\fi
		\fi\fi
		\ifnum\pgfcircmathresult >355 \ifnum\pgfcircmathresult <361
			\ifpgf@circuit@bipole@voltage@below
				  \def\pgf@circ@bipole@voltage@label@anchor{north}
			\else\def\pgf@circ@bipole@voltage@label@anchor{south}
			\fi
		\fi\fi

		\ifnum \ctikzvalof{mirror value}=-1
			\ifpgf@circuit@bipole@voltage@below
				\pgf@circuit@bipole@voltage@belowfalse
			\else
				\pgf@circuit@bipole@voltage@belowtrue
			\fi
		\fi

		\ifpgf@circuit@bipole@inverted
			\ifpgf@circuit@bipole@voltage@below
				\pgf@circuit@bipole@voltage@belowfalse
			\else
				\pgf@circuit@bipole@voltage@belowtrue
			\fi
		\fi

		\ifpgf@circuit@bipole@voltage@below
			\def\pgf@circ@bipole@voltage@label@where{-90}
		\else
			\def\pgf@circ@bipole@voltage@label@where{90}
		\fi


		\edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/european label distance}
		\pgfkeysifdefined{\pgf@temp}
			{ \edef\eudist{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/european label distance}} }
			{ \edef\eudist{\ctikzvalof{voltage/european label distance}} }

	\pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
	}%end pgfextra

		\ifpgf@circuit@bipole@isvoltage
			\pgf@circ@drawvoltagegenerator
		\else
			\pgf@circ@drawvoltagegeneric
		\fi

	%	(\ctikzvalof{bipole/name}.\pgf@circ@bipole@voltage@label@where) %Zeile sinnlos!?
		\ifpgf@circuit@bipole@voltage@straight
			coordinate (Vlab) at ($(pgfcirc@Vto)!0.5!(pgfcirc@Vfrom) $)
			node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt]
					  at (Vlab) { \pgf@circ@finallabels{voltage/label} }
		\else
		coordinate (Vlab) at ($(\ctikzvalof{bipole/name}.center) !
			\ifpgf@circuit@europeanvoltage
				\eudist
			\else
				\ctikzvalof{voltage/american label distance}
			\fi !
			(\ctikzvalof{bipole/name}.\pgf@circ@bipole@voltage@label@where)$)
		node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt] at (Vlab) { \pgf@circ@finallabels{voltage/label} }
		\fi
}%end drawvoltages
\endinput


==> circuitikz/tex/t-circuitikz.tex <==
\def\pgfcircversion{0.8.3}
\def\pgfcircversiondate{2017/05/28}
\writestatus{loading}{\pgfcircversiondate{} The CircuiTikz circuit drawing package version \pgfcircversion}

\usemodule[tikz]

\startmodule[circuitikz]
\usetikzlibrary[calc]
\usetikzlibrary[arrows]

\unprotect

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfcirc.defines.tex
\input pgfcircutils.tex

\input pgfcircshapes.tex
\input pgfcircmonopoles.tex
\input pgfcircbipoles.tex
\input pgfcirctripoles.tex
\input pgfcircquadpoles.tex

\input pgfcirclabel.tex
\input pgfcircvoltage.tex
\input pgfcirccurrent.tex
\input pgfcircflow.tex

% defaults

\setupmodule
   [current=european,
    voltage=european,
    resistor=american,
    inductor=cute,
    logic=american,
    siunitx=true,
    arrowmos=false]

\processaction
   [\currentmoduleparameter{voltage}]
   [european=>\ctikzset{voltage=european},
    american=>\ctikzset{voltage=american}]

\processaction
   [\currentmoduleparameter{current}]
   [european=>\ctikzset{ current=european},
    american=>\ctikzset{ current=american}]

\processaction
   [\currentmoduleparameter{label}]
   [straight=>\ctikzset{label/align = straight},
    align=>\ctikzset{label/align = rotate},
    smart=>\ctikzset{label/align = smart}]

\processaction
   [\currentmoduleparameter{resistor}]
   [european=>\ctikzset{ resistor=european},
    american=>\ctikzset{ resistor=american}]

\processaction
   [\currentmoduleparameter{inductor}]
   [european=>\ctikzset{ inductor=european},
    american=>\ctikzset{ inductor=american},
    cute=>\ctikzset{ inductor=cute}]

\processaction
   [\currentmoduleparameter{diode}]
   [full=>\ctikzset{ diode=full},
    empty=>\ctikzset{ diode=empty}]

\processaction
   [\currentmoduleparameter{logic}]
   [european=>\ctikzset{ logic ports=european},
    american=>\ctikzset{ logic ports=american}]

\processaction
   [\currentmoduleparameter{siunitx}]
   [true=>\def\SI#1#2{#1\,#2}
    \def\ampere{\rm{A}}
    \def\volt{\rm{V}}
    \def\ohm{\Omega}
    \def\siemens{\rm{S}}
    \def\farad{\rm{F}}
    \def\henry{\rm{H}}
    \def\second{\rm{s}}
    \def\coulomb{\rm{C}}
    \def\siemens{\rm{S}}
    \def\radians{\rm{rad}}
    \def\milli{\rm{m}}
    \def\micro{\mu}
    \def\nano{\rm{n}}
    \def\pico{\rm{p}}
    \def\kilo{\rm{k}}
    \def\mega{\rm{M}}
    \def\giga{\rm{G}}
    \def\tera{\rm{T}},
    false=>]
%   \s!default=>\pgf@circ@siunitxtrue,

\processaction
   [\currentmoduleparameter{arrowmos}]
   [true=>\pgf@circuit@mos@arrowstrue,
    false=>\pgf@circuit@mos@arrowsfalse]
%   \s!default=>\pgf@circuit@mos@arrowstrue,


\ifpgf@circ@siunitx
 % nothing! siunitx and xstrings don't work in context
\fi


% Context specific

\ctikzset{tripoles/op amp/font/.initial=\switchtobodyfont[small]}

\input pgfcircpath.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

% define the environment
\long\def\startcircuitikz#1\stopcircuitikz{\starttikzpicture#1\stoptikzpicture}

\protect

\stopmodule

\endinput


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

